Robust Linear Regression: Phase-Transitions and Precise Tradeoffs for General Norms

In this paper, we investigate the impact of test-time adversarial attacks on linear regression models and determine the optimal level of robustness that any model can reach while maintaining a given level of standard predictive performance (accuracy). Through quantitative estimates, we uncover fundamental tradeoffs between adversarial robustness and accuracy in different regimes. We obtain a precise characterization which distinguishes between regimes where robustness is achievable without hurting standard accuracy and regimes where a tradeoff might be unavoidable. Our findings are empirically confirmed with simple experiments that represent a variety of settings. This work applies to feature covariance matrices and attack norms of any nature, and extends beyond previous works in this area.

==> abstract.tex <==
\begin{abstract}
We study the robustness (to input perturbations) of high-dimensional kernel regression as a function of all relevant variables, namely: the choice of kernel, the amount of explicit $L_2$-regularization, the aspect ratio $n / d$, the covariance structure of the features, the signal-to-noise ratio of the training dataset, and the shape of the prior on the parameters of the ground-truth model. Our focus is on the setting where both the sample size $n$ and the input-dimension $d$ are large but proportionate. Our analysis puts to light a number of interesting phenomena. For example, in the case of kernels which arise as infinite-width limits of neural networks if different linearized regimes, we obtain a complete classification of activation functions as either: (1) genuinely robust (e.g., absolute value), or (2) genuinely nonrobust (e.g., ReLU), in this specific regime.  We also uncover novel tradeoffs between generalization error and robustness. Our analysis also allows us to give precise answers to otherwise difficult questions like: What is better for robustness, more data or more features ?
\end{abstract}

==> analysis.tex <==
\section{Proofs of main results}
\label{sec:proofs}
In this section, we provide proofs for our theoretical results. Low-level technical details will be deferred to appropriate sections in the appendix. 

% Thus, the (non)robustness of the kernel ridge regressor depends on the data only via its empirical covariance matrix $XX^\top$,  by means of two intermediate random matrices
% \begin{itemize}
%     \item The kernel gram matrix $G=h(XX^\top)$.
%     \item The matrix $B$, which measures the amount to which the kernel function $h$ distorts the empirical covariance structure of the training data $XX^\top$.
% \end{itemize}

% \paragraph{A (non)robustness kernel.}
% Notice that the matrix $ D$ appearing in Lemma \ref{lm:kridgerob} can be succinctly written as $d_{ij} = (1/d^2) \Delta_h( x_i, x_j)$, where $ \Delta_h$ is the kernel on $\sphere$ defined by
% \begin{eqnarray}
%  \Delta_h(   a,   b) := (   a^\top    b)\mathbb E_{ x \sim P}[h'( x^\top a/d)h'( x^\top b/d)].
% \end{eqnarray}
% Thus, $B$ is the gram matrix for this kernel.
% In particular, if $P$ is isotropic, then
% \begin{eqnarray}
%  \Delta_h(   a,   b) := h_{ \Delta_h}(   a^\top    b) = (   a^\top    b)\phi_{h',P}(   a^\top    b),
% \end{eqnarray}

% an inner-product kernel, where $\phi_{h,P}:[-1,1] \to \mathbb R$ is the dual of kernel function $h$ w.r.t the distribution $P$, defined in \eqref{eq:phigP}.
% % , and $\phi_{g,P}'$ is its derivative.
% In this case $ D=h_{ \Delta_h}(XX^\top)$, a function of the empirical covariance matrix $XX^\top$ alone. As a consequence, the matrix $R$ defined in \eqref{eq:R} depends on the data only via its empirical covariance matrix $XX^\top$: it is a nonlinear distortion thereof.

% \input{linear.tex}

% where $m_\gamma$ is the Stieltjes transform of $\mu_{\mathrm{MP}(\gamma)}$, the Marchenko-Pastur density with para7    Proofsmeter $\gamma$. 

% For a proof of the lemma, we will need the following auxiliary lemma.

% \subsection{Warmup: law of robustness for regularized linear model}
% We start off by computing the nonrobustness measure $\mathfrak{S}(f)^2$ for regularized linear regression. We will later extend the result to the more interesting case of nonlinear kernel methods.

% Recall the definition of the curvature coefficients $\alpha(\cdot)$, $\beta(\cdot)$, $\gamma(\cdot)$, and $\kappa(\cdot)$ from \eqref{eq:curvcoefs}. 
% The theorem is proved in the Appendix.
% The result is established using tools from random matrix theory.

% \paragraph{A link with generalization error.}
% One can show that the generalization error of model $\widehat{f}_{h,\lambda}$, defined by
% \begin{eqnarray}
% \varepsilon(\widehat{f}_{h,\lambda}) := \mathbb E_{(x_{n+1},y_{n+1}) \sim P_{\text{data}}}[(y_{n+1}-\widehat{f}_{h,\lambda}(x_{n+1}))^2],
% \end{eqnarray}
% is given by the following formula
% \begin{eqnarray}
%  \varepsilon(\widehat{f}_{h,\lambda}) = \zeta^2 \cdot \dfrac{1}{n}\trace( Q\widetilde{g}^{-2}) + o_{n,\mathbb P}(1).
% \end{eqnarray}
% Comparing with the formula in Lemma \ref{lm:nonrobkernel} gives the following result which lower-bounds nonrobustness in terms of generalization error.
% \begin{restatable}{cor}{}
% Under the conditions of Lemma \ref{lm:nonrobkernel}, the following inequality holds in the limit $n,d \to \infty$ with $d/n \to \gamma \in (0,\infty)$
% \begin{eqnarray}
% d^{-1}\mathfrak{S}(\widehat{f}_{h,\lambda})^2 \ge \alpha(h')\cdot \varepsilon(\widehat{f}_{h,\lambda}) + o_{n,\mathbb P}(1).
% \end{eqnarray}
% \end{restatable}

% \paragraph{An important special case.}
% \subsection{An explicit formula}


% Define another extended-value function $ s_{\mathrm{MP}}^+:(0,\infty) \to [0,\infty]$ by
% \begin{eqnarray}
% s_{\mathrm{MP}}^+(\gamma) := \frac{1}{|1-\gamma|}.
% \end{eqnarray}

% \subsection{Law of robustness for kernel methods}
% We now extend the previous lemma to a large class of kernel methods (including polynomial and exponential kernel methods).
% We will establish in Theorem \ref{thm:master} that for such kernel methods, the normalized nonrobustness measure $d^{-1}\mathfrak S(\widehat{f}_{h,\lambda})^2$ converges to $\zeta^2 s_{\mathrm{MP}}(\overline{\lambda}_h,1/\gamma)$ in probability, wher $\overline{\lambda}_h$ is the total regularization defined in \eqref{eq:impreg}.
% Thus, in view of Lemma \ref{lm:linear}, such a model is robustness-equivalent to a linear model with regularization $\overline{\lambda}_h$. 

\subsection{Proof of Theorem \ref{thm:main}}
\label{subsec:proofgeneral}
% We start with a proof of Lemma \ref{lm:kridgerob}
% \begin{proof}[Proof of Lemma \ref{lm:kridgerob}]
% Let $c_i$ be the $i$th component of the dual weights vector $  c : = ( G+\lambda  I_n)^\top  y \in \mathbb R^n$ in the definition of the KRR model $\widehat{f}_{h,\lambda}$ \eqref{eq:kridge}. By direct computation, we have $\nabla_{ x} \widehat{f}_{h,\lambda}( x) = (1/d)\sum_{i=1}^n c_ih'( x^\top  x_i/d) x_i$, and so for $ x \sim P$, one has
% \begin{eqnarray*}
% \begin{split}
% \mathfrak S(\widehat{f}_{h,\lambda};P)^2 &:= \mathbb E_{ x} \|\nabla_{ x} \widehat{f}_{h,\lambda}( x)\|^2 
% = (1/d^2)\mathbb E_{ x} \sum_{i=1}^n\sum_{\ell=1}^n c_ic_\ell  x_i^\top  x_\ell h'( x^\top  x_i/d)h'( x^\top  x_\ell/d)\\
% &= (1/d^2)\sum_{i=1}^n\sum_{\ell=1}^n c_ic_\ell  x_i^\top  x_\ell \mathbb E_{ x}[h'( x^\top  x_i/d)h'( x^\top  x_\ell/d)] = (1/d)  c^\top (Q \circ M)   c\\
% &=  y^\top ( G+\lambda  I_n)^{-1}  (Q \circ M) ( G + \lambda  I_n)^{-1} y= (1/d) \cdot (y^\top  R  y),\end{split}
% \end{eqnarray*}
% as claimed.
% \end{proof}

We will need the following lemma which is proved in the appendix.
% We now consider the case of a general nonlinear kernel function $h$.
%  Given a continuous function $g:[-1,1] \to \mathbb R$, define an associated function $u_g(\cdot;d):[-1,1] \to \mathbb R$ by
% \begin{eqnarray}
% u_g(t;d) := \mathbb E[g(z_1)g(tz_1 + \sqrt{1-t^2}z_2)],
% \label{eq:ug}
% \end{eqnarray}
% where $z=(z_1,\ldots,z_d) \sim \unif(\sphere)$.
% Note that by rotational-invariance of $\unif(\sphere)$, the following identity holds for all $a,b \in \mathbb R^d$
% \begin{eqnarray}
% \mathbb E[g(z^\top x)g(z^\top x')] = u_g(x^\top x';d).
% \end{eqnarray}

% \subsection{Tools}
\begin{restatable}{lm}{viewpoint}
Suppose Conditions \ref{cond:smooth} and \ref{cond:gausslike} are in order. For fixed $\lambda > -\lambda_h$, consider the $n \times n$ random psd matrices $G=h(Q)+\lambda I_n$ and $D := Q \circ M$, where $M$ is $n \times n$ random psd matrix with entries
\begin{eqnarray}
\begin{split}
M_{ij} := \mathbb E_{x \sim P}[h'( x^\top  x_i/d)h'( x^\top  x_j/d)],\,\forall i,j \in [n].
\end{split}
\end{eqnarray}
Also consider $n \times n$ random psd matrices $G_1:=G_0 + (h(0)+\trace(\Sigma^2/d^2))1_n1_n^\top$ with $G_0:= h'(0)Q +(\lambda+\lambda_h) I_n$
Finally, let $A$ be an $n \times n$ possibly random matrix such that $\|A\|_\star = o(n^{\min(c_0,1)})$ w.h.p, where $c_0>0$ is the absolute constant in the previous lemma. Then, for sufficiently large $n \asymp d$, it holds w.h.p over $X$ and $A$ that
\begin{eqnarray}
\begin{split}
% |\trace( A G^{-1}  B  G^{-1})-\trace( A G_0^{-1} B_0  G_0^{-1})| &= o_n(1),\\
\trace(A G^{-1}  (Q \circ M)  G^{-1}) = h'(0)^2\trace(AG_1^{-1} Q G_1^{-1}) + o_n(1).
\end{split}
\end{eqnarray}
\label{lm:viewpoint}
\end{restatable}
% The proof Lemma \ref{lm:viewpoint} requires the following auxiliary lemma which is proved in the appendix.
\begin{proof}[Proof of Theorem \ref{thm:main}]
We know from Lemma \ref{lm:kridgerob} that $\mathfrak{S}(\widehat{f}_{h,\lambda})^2= c^\top R c/d$, where $ c= G^{-1}  y$, $ R := G^{-1}  (Q \circ M)  G^{-1}$ with $ Q := (1/d) X X^\top$ and $M$ as defined in the lemma. It suffices to invoke Lemma \ref{lm:viewpoint} with $A=zz^\top$ where $z:=y/\sqrt{d} \in \mathbb R^n$; this is valid since $\|A\|_\star = \|z\|^2 = \|y\|^2/d = o(d^\delta)$ w.h.p by hypothesis. Defining $S : = h'(0)^2Q$ and $G_0:=Q + \overline{\lambda}_h I_n$, we get
\begin{eqnarray}
\begin{split}
\mathfrak{S}(\widehat{f}_{h,\lambda})^2 &= z^\top G^{-1} (Q \circ M)G^{-1}z = \trace(zz^\top G^{-1} (Q \circ M)G^{-1})\\
&= \trace(zz^\top G_1^{-1}SG_1^{-1}) + o_{n,\mathbb P}(1) =  z^\top G_1^{-1}S G_1^{-1}z+o_{n,\mathbb P}(1).%\\
%&= z^\top G_0^{-1}SG_0^{-1} z + o_{n,\mathbb P}(1).
\end{split}
\label{eq:oneliner}
\end{eqnarray}
% The last step in the above display is because $G_1 = G_0 + h(0)1_n1_n^\top$ and so by \eqref{eq:turbo5} and \eqref{eq:turbo6} it holds w.h.p over $X$ that (\mytodo{Pending a proof!})
% \begin{align}
% |z^\top G_1^{-1} S G_1^{-1}z - z^\top G_0^{-1} S G_0^{-1} z| = o_{n,\mathbb P}(1).
% \end{align}
Now, when $h'(0) = 0$, we have $S := h'(0)^2 Q=0$ and so \eqref{eq:oneliner} gives $\mathfrak{S}(\widehat{f}_{h,\lambda})^2=o_{n,\mathbb P}(1)$ w.h.p over $X$ and $y$ as claimed. Otherwise, with $\overline{\lambda}_h>0$ and defined in \eqref{eq:totalreg} and $\alpha_h \ge 0$ as defined in Theorem \ref{thm:main}, have
$G_1^{-1} = h'(0)^{-1}(Q+\overline{\lambda}_h I_n + \alpha_h 1_n1_n^\top) = h'(0)^{-1}H_1^{-1}$
\begin{eqnarray}
\begin{split}
G_1^{-1} S G_1^{-1} &:= H_1^{-1} Q H_1^{-1},
\end{split}
\end{eqnarray}
which completes the proof of the theorem upon combining with \eqref{eq:oneliner}.
\end{proof}

\subsection{Proof of Theorem \ref{thm:master}, Theorem \ref{thm:linearsignal}, and their corollaries}
\label{subsec:prooflinear}
% Suppose the weights vector of the linear response model $w_\star$ is a random (and independent of the training data) from an isotropic distribution on $\mathbb R^d$ with covariance matrix $(r_\star^2/d) I_d$. In particular, this means that on average, the squared $\ell_2$ norm of $w_\star$ is $r_\star^2$.
% Let $\lambda_1 \ge \ldots \ge \lambda_n$ be the eigenvalues of the rescaled sample covariance matrix $ Q:=(1/d) X X^\top$.
% \begin{restatable}[Nonasymptotic estimate of nonrobustness of KRR]{thm}{}
% Suppose Conditions abc and xyz are in order. For any fixed regularization parameter $\lambda > -\lambda_h$, we have the following (with $\overline{\lambda}_h := \lambda_h + \lambda$)

% \textbf{(A) Covariance-oriented case.} If $h'(0) = 0$, then $\mathbb E_{\varepsilon,w_\star}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2] = o_{n,\mathbb P}(1)$.

% \textbf{(B) Distorted case.} If $h'(0) > 0$, then
% \begin{eqnarray}
% \begin{split}
% \mathbb E_{\varepsilon,w_\star}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2 \mid  X] &=  \zeta^2\cdot \frac{1}{d} \sum_{i=1}^n \dfrac{\lambda_i}{(\lambda_i + \overline{\lambda}_h/h'(0))^2} + r_\star^2 \cdot \frac{1}{d}\sum_{i=1}^n \dfrac{\lambda_i^2}{(\lambda_i + \overline{\lambda}_h/h'(0))^2} + o_{n,\mathbb P}(1).
% \end{split}
% \label{eq:lsd}
% \end{eqnarray}
% \end{restatable}
\begin{proof}[Proof of Theorem \ref{thm:linearsignal}]
We know from Theorem \ref{thm:main} that $\mathfrak{S}(\widehat{f}_{h,\lambda})^2= c^\top Qc/d + o_n(1)$ w.h.p over the training dataset $\mathcal D_n \equiv (X,y)$, where $ c= H_1^{-1}y$, $H_1 := H_0 + \alpha_h 1_n1_n^\top$ (where $\alpha_h$ is as defined in Theorem \ref{thm:main}), $H_0 := Q+\overline{\lambda}_h I_n$, and $Q:=XX^\top /d$. Taking expectations w.r.t $(\varepsilon,w_\star)$ and noting that $X$, $\varepsilon$, and $w_\star$ are independent (and $\mathbb E[\varepsilon] = 0$), we obtain
\begin{eqnarray}
\begin{split}
\mathbb E_{\varepsilon,w_\star}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2] &= \zeta^2\cdot d^{-1}\trace( H_1^{-1} Q H_1^{-1}) +  d^{-1}\mathbb E_{w_\star}[w_\star^\top  X^\top  H_1^{-1}  Q H_1^{-1} X w_\star] + o_{n,\mathbb P}(1)\\
&= \zeta^2\cdot d^{-1}\trace( H_1^{-1}  Q H_1^{-1}) + r_\star^2 \cdot d^{-1}\trace(\phi(\Sigma) X^\top  H_1^{-1} Q H_1^{-1} X/d)+o_{n,\mathbb P}(1)\\
&= \zeta^2\cdot\trace(Q H_1^{-2}/d) + r_\star^2 \cdot \trace(\phi(\Sigma)Q^2 H_1^{-2}/d)+o_{n,\mathbb P}(1)\\
&= \zeta^2\cdot \trace(Q H_0^{-2}/d) + r_\star^2 \cdot \trace(\phi(\Sigma)Q^2 H_0^{-2}/d)+o_{n,\mathbb P}(1)\\
&= \zeta^2\cdot \frac{n}{d}\cdot \widetilde{V}_n(\overline{\lambda}_h)(\overline{\lambda}_h) + r_\star^2\cdot \frac{n}{d}\cdot \widetilde{B}(\overline{\lambda}_h)+o_{n,\mathbb P}(1)\\
&= r_\star^2  \widetilde{B}_n(\overline{\lambda}_h) + \zeta^2\widetilde{V}_n(\overline{\lambda}_h) + o_{n,\mathbb P}(1),
\end{split}
\label{eq:truck}
\end{eqnarray}
where the second line is thanks to a classical formula on the expectation of a quadratic form; the fourth line follows from Lemma \ref{lm:shermann-morrison}; and the last two lines follow from the definition of the functions $\widetilde{V}_n$ and $\widetilde{B}_n$ defined in \eqref{eq:Vn} and \eqref{eq:Bntilde} respectively.
% This establishes \eqref{eq:linearformula} upon dividing through by $r_\star^2$.
It then suffices to divide through \eqref{eq:truck} by $r_\star^2$ from letting $n,d \to \infty$ with $d/n \to \gamma$ on both sides of \eqref{eq:truck}, and invoking \eqref{eq:Vtilde} and \eqref{eq:Btilde}.

The proof of parts (B1) and (B2) of the theorem follow from the decomposition \eqref{eq:Sdecomp}, combined with the definition of $\widetilde{B}_\mu$ and $\widetilde{V}_\mu$.

The proof of part (B3) follows from the decomposition \eqref{eq:Sdecomp} combined with \cite[Corollary 3]{Hastie2019}.
% \emph{Part (A).}
% We deduce from \eqref{eq:truck} that if $h'(0) = 0$, then $\mathbb E_{\varepsilon,w_\star}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2 \mid X] = o_{n,\mathbb P}(1)$ and $S(h,\gamma,\zeta^2,\lambda)=0$.
% \emph{Part (B).} The formula \eqref{eq:linearformula} follows from \eqref{eq:truck} and definition of the $\lambda_i$'s. Formula \eqref{eq:lsd} is a direct consequence of \eqref{eq:linearformula} and the $\widehat{\mu}_n \to \mu$ (weakly) by hypothesis.
% Finally, if $P$ is isotropic log-concave, it is a classical results of RMT that $\widehat{\mu}_n$ converges weakly to $\mu_{\mathrm{MP}(\rho)}$, the Marchenko-Pastur distribution with shape parameter $\rho:=1/\gamma$. The extreme cases \eqref{eq:extremecases} are a direct consequence of well-known elementary properties of functions $s_{\mu_{\mathrm{MP}(\gamma)}}^{(k)}$.
\end{proof}

% \begin{proof}[Proof of Corollary \ref{cor:extremecases}]
% Follows directly from the second part of Theorem \ref{thm:linearsignal}, the definition of the functions $t\mapsto\widetilde{B}(\gamma,t)$ and $t \mapsto V(\gamma,\mathrm{SNR},t)$ via \eqref{eq:compbias} and \eqref{eq:biasvariance} respectively via the functions $t \mapsto s_{\mu}(t)$ defined in \eqref{eq:smu} with $\mu=\mu_{\mathrm{MP}(\gamma)}$, and their elementary properties (see Lemma \eqref{lm:slimits}).
% \end{proof}

\begin{proof}[Proof of Theorem \ref{thm:master}]
Let $z := (f_\star(x_1),\ldots,f_\star(x_n)) \in \mathbb R^n$. Analogous the beginning of the proof of Theorem \ref{thm:linearsignal}, we establish
\begin{eqnarray}
\begin{split}
\mathbb E_{\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2 \mid X] &= \zeta^2\cdot \trace( G^{-1} (Q \circ M) G^{-1}) +  z^\top  G^{-1}  (Q \circ M)  G^{-1} z\\
&\ge \zeta^2\cdot \trace( G^{-1} (Q \circ M) G^{-1}).%\\
% &= \zeta^2 \cdot \trace(h'(0)^2  Q (h'(0) Q + \overline{\lambda}_h  I_n)^{-2}).
\end{split}
\label{eq:bigtruck}
\end{eqnarray}
Invoking Theorem \ref{thm:linearsignal} with $r_\star = 0$ completes the proof.
\end{proof}
% \begin{restatable}[Analytic formula for robustness profile of KRR]{cor}{}
% Suppose $ Q$ admits a limiting eigenvalue distribution $\mathcal D$ (in a weak sense).
%  Then, under the same conditions as the previous theorem, we have the following analytic formula for the robustness profile 
% \begin{eqnarray}
% S(h,\gamma,\zeta^2,\lambda) = \rho \cdot \begin{cases}
% \zeta^2\cdot s_{\mathcal D}^{(1)}(\overline{\lambda}_h/h'(0))+r_\star^2 \cdot s_{\mathcal D}^{(2)}(\overline{\lambda}_h/h'(0)),&\mbox{ if }h'(0)>0,\\
% 0,&\mbox{ else.}
% \end{cases}
% \end{eqnarray}
% where $\rho := 1/\gamma$ and the functions $s_{\mathcal D}^{(1)},s_{\mathcal D}^{(2)}:(0,\infty) \to [0,\infty]$ are defined by 
% \begin{eqnarray}
% s_{\mathcal D}^{(k)}(t) := \int_{\mathbb R}\frac{\tau^k}{(\tau + t)^2}\,\dv \mathcal D(\tau).
% \end{eqnarray}
% \end{restatable}
% In particular, if the distribution of the features $P$ is log-concave isotropic, then the celebrated Marchenko-Pastur theorem tells us that $\mathcal D$ has density w.r.t Lebesgue is given by
% \begin{eqnarray}
% \label{eq:lsdbased}
% \frac{\dv \mathcal D(\tau)}{\dv \tau} = \begin{cases} (1-\rho)_+\delta_0(\tau)+ \dfrac{\sqrt{(c_+-\tau)(\tau-c_-)}}{2\pi\rho \tau},&\mbox{ for }\tau \in [c_-,c_+],\\
% 0,&\mbox{ else,}
% \end{cases}
% \end{eqnarray}
% where $\rho := 1/\gamma$ and $c_\pm := (1 \pm \sqrt{\rho})^2$.
% Thus, in this case, $\mathcal D$ and therefore the functions $s_{\mathcal D}^{(k)}$ appearing in \eqref{eq:lsdbased}, only depends on the shape parameter $\gamma$.

% \begin{proof}[Proof of Corollary]
% Follows from previous theorem and the fact that $\widehat{\mathcal D}_n \to \mathcal D$ (weakly) by assumption.
% \end{proof}

% \paragraph{Comparison with generalization error.}
% It is clear that if $h'(0) = 0$, then $\widehat{f}_{h,\lambda}$ is generalization-equivale
% nt to the null model, more precisely $\mathbb E_{\varepsilon,w_\star}[e(\widehat{f}_{h,\lambda})] = r_\star^2 + o_{n,\mathbb P}(1)$. Otherwise, let $t := \overline{\lambda}_h/h'(0)$. . One computes
% \begin{eqnarray*}
% \begin{split}
% \mathbb E_{\varepsilon,w_\star}[e(\widehat{f}_{h,\lambda}) \mid X] &= \zeta^2 \cdot \trace( B_0 G_0^{-2}) + t^2\cdot \mathbb E_{w_\star}[\|\Sigma^{1/2}( Q+t I_n)^{-1} w_\star \|_2^2 \mid X] + o_{n,\mathbb P}(1)\\
% &= \zeta^2 \cdot \trace((1/d^2) X\Sigma X^\top( Q+t I_n)^{-2}) + r_\star^2 t^2 \cdot \trace(\Sigma( Q+t I_n)^{-2}) + o_{n,\mathbb P}(1)\\
% &= \zeta^2 \cdot d^{-1}\trace(\widetilde{Q}( Q+t I_n)^{-2}) + r_\star^2 t^2\cdot d^{-1}\trace(( Q+t I_n)^{-2}\Sigma) + o_{n,\mathbb P}(1)
% \end{split}
% \end{eqnarray*}

% \begin{restatable}{rmk}{}
% In Section \ref{sec:signalplusnoise}, we will consider extensions that go beyond the noise-only reponse model \eqref{eq:noiseonly}.

% \subsection{Generic lower-bound: Proof of Theorem \ref{thm:master}}
% We will need the following auxiliary lemma which is of independent interest.

% % \begin{restatable}{lm}{nonrobkernel}
% % Consider kernel ridge regression \eqref{eq:kridge} with training data generated according to the noise-only model \eqref{eq:noiseonly}, and
% % suppose the kernel function $h$ verifies the Conditions \ref{cond:smooth}(B) and \ref{cond:smooth}(C).
% % % Let $\gamma \in (0,\infty)$ and define constants $0 \le R_1 \le R_2 $ by
% % % \begin{eqnarray}
% % % \begin{split}
% % % R_1 &:=\max(\kappa(h'),\alpha(h')(1-\sqrt{\gamma})_+^2,\beta(h')(1-\sqrt{\gamma})_+^4),\\
% % % R_2 &:=\kappa(h')+\alpha(h')(1+\sqrt{\gamma})^2+\beta(h')(1+\sqrt{\gamma})^4.
% % % \end{split}
% % % \end{eqnarray}
% % % where $\kappa(g) := \zeta_0(h^2)-\zeta_1(h)^2\ge 0$
% % Fix a ridge regularization parameter $\lambda > -\lambda_h$, where $\lambda_h$ is the implicit regularization induced by $h$, and defined in \eqref{eq:impreg}. Then, in the limit $n,d \to \infty$ with $n/d \to \gamma \in (0,\infty)$, it holds that
% % \begin{eqnarray}
% % \begin{split}
% % n^{-1}\mathfrak{S}(\widehat{f}_{h,\lambda})^2 - \zeta^2 \cdot n^{-1} \trace( D_0 G_0^{-2}) \overset{p}{\to} 0,
% % \end{split}
% % \end{eqnarray}
% % where $ D_0, G_0$ are $n \times n$ random psd matrices given by
% % \begin{eqnarray}
% % \begin{split}
% %  D_0 &:= h'(0)^2  Q,\\
% %  Q &:=  X X^\top,\\
% %  G_0 &:= h(0) \ones_n\ones_n^\top + h'(0)  Q + (\lambda+\lambda_h)  I_n.
% % %\ A &:=  Q \circ  I_n = \diag(\|x_1\|^2,\ldots,\|x_n\|^2).
% % \end{split}
% % \label{eq:matrices}
% % \end{eqnarray}
% % % Moreover, the above lower-bound is tight: it is attained when $\beta(h')=0$, e.g as as in
% % % \begin{itemize}
% % % \item Odd-degree polynomial kernel regression.
% % % \item Infinite-width two-layer neural networks with absolute-value activation function.
% % % \end{itemize}
% % \label{lm:nonrobkernel}
% % \end{restatable}
% \begin{proof}
% We know from Lemma \ref{lm:kridgerob} that $\mathfrak{S}(\widehat{f}_{h,\lambda})^2= c^\top R  c$, where $ c=( G+\lambda  I_n)^{-1} \varepsilon$, $ R:= B \circ  Q$
% where  $D:=  B \circ  Q$, with $ Q :=  X X^\top$ and $B$ is the $n \times n$ psd matrix with entries given by $b_{i,\ell} := \mathbb E_{ x}[h'( x^\top  x_i)h'( x^\top  x_\ell)]$. We deduce from \cite[Lemma 7.6]{Dobriban2018} that
% \begin{eqnarray}
% \begin{split}
% n^{-1}\mathfrak{S}(\widehat{f}_{h,\lambda})^2 - \zeta^2 \cdot n^{-1}\trace( D( G+\lambda  I_n)^{-2})=o_{n,\mathbb P}(1)
% \end{split}
% \label{eq:randomquad}
% \end{eqnarray}

% The remainder of the proof is split between separate steps.

% \paragraph{-- Step 1: Linearizing $D :=  B \circ  Q$.} Thanks to Lemma \eqref{lm:approxsphericalmatrix}, we know that in the limit $n,d \to \infty$ with $n/d \to \gamma \in (0,\infty)$, it holds that
% \begin{eqnarray}
% \| B\circ  Q- D_0\|=o_{n,\mathbb P}(1),
% \label{eq:Bapprox}
% \end{eqnarray}
% where $ D_0:=h'(0)^2  Q$.
% % where in the last step, we have used the following facts 
% % \begin{itemize}
% % \item[--] Each $\|x_i\|^2/d$ has exponential concentration around its mean value of $1$.
% % \item[--] $\lambda_{\min}(C \circ C) \ge \lambda_{\min}(C)^2$, by the \emph{Shur Product Theorem}.
% % \item[--] $\lambda_{\min}(C) \overset{a.s}{\to} (1-\sqrt{\gamma})_+^2$, thanks to a result of Bai-Yin.
% % \end{itemize}

% % \begin{eqnarray}
% % \begin{split}
% % n^{-1}\lambda_{\min}(( X X^\top) \circ B) \gtrsim n^{-1}\lambda_{\min}(( X X^\top) \circ  B_0) &\gtrsim \kappa(h)^2 \lambda_{\min}( X X^\top/d)\\
% % &\overset{a.s}{\to} \kappa(h)^2(1-\sqrt{\gamma})^2,
% % \end{split}
% % \end{eqnarray}
% % where the last step is an application of the \emph{Bai-Yin Theorem}. We deduce that
% % \begin{eqnarray}
% % \mathfrak{S}(f_\lambda)^2 \gtrsim \kappa(h)^2(1-\sqrt{\gamma})^2\| c\|^2,
% % \end{eqnarray}
% % in probability.

% % \begin{eqnarray*}
% % \begin{split}
% % \mathbb E_y[n^{-1}\mathfrak S(f_\lambda)^2] &= n^{-1}\mathbb E_y[ c^\top (( X X^\top) \circ B)  c)]\\
% % &= n^{-1} \mathbb E_y[y^\top  G^{-1}(( X X^\top) \circ B)  G^{-1} y]\\
% % &= \zeta^2 n^{-1}\trace( G^{-2}B) = \zeta^2 n^{-1}\trace( G_0^{-2}  B_0) + o_{n,\mathbb P}(1)\\
% % &\ge \zeta^2\zeta_3(h)^2 \frac{1}{d}\sum_i \frac{\lambda_i( X X^\top)}{\lambda+\nu(h)+\lambda_i(h'(0)  X X^\top + h(0) \ones_n\ones_n^\top)} + o_{n,\mathbb P}(1),
% % \end{split}
% % \end{eqnarray*}

% % \paragraph{-- Step 1: Upper-bounding $\lambda_{\max}( B \circ C)$.}
% % Analogously to the lower-bound for $\lambda_{\min}( B \circ C)$, one computes
% % \begin{eqnarray*}
% % \begin{split}
% %     \lambda_{\max}( B \circ C) &= \| B \circ C\|_{op} \le \kappa(h')\|C \circ  I_n\|_{op} + \alpha(h')\|C\|_{op}+\beta(h')\|C \circ C\|_{op} \\
% %     &\ge \kappa(h') + \alpha(h')(1+\sqrt{\gamma})^2 + \beta(h')(1+\sqrt{\gamma})^4 + o_{n,\mathbb P}(1).
% % \end{split}
% % \end{eqnarray*}
% \paragraph{-- Step 2 : Linearizing the (nonlinear) gram matrix $ G$.}
% Since $ G = h( Q)$, \cite[Theorem 2.3]{elkaroui2010} gives
% $$
% \|( G+\lambda  I_n)- G_0\|_{op} = o_{n,\mathbb P}(1),
% $$
% where $ G_0$ is as defined in \eqref{eq:matrices}.
% Finally, invoking Lemma \ref{lm:crucial} gives $n^{-1}\trace( D( G+\lambda  I_n)^{-2}) = n^{-1}\trace( D_0 G_0^{-2})+o_{n,\mathbb P}(1)$. Combining with \eqref{eq:randomquad} then gives
% \begin{eqnarray}
% \begin{split}
% n^{-1} \mathfrak{S}(\widehat{f}_{h,\lambda})^2 &= \zeta^2 n^{-1} \trace( D_0 G_0^{-2}) + o_{n,\mathbb P}(1),
% \end{split}
% \label{eq:meanvariance}
% \end{eqnarray}
% as claimed.
% %  Direct computation gives
% %  \begin{eqnarray*}
% %  \begin{split}
% %  n^{-1}\mathbb E_y \| c\|^2 &= n^{-1} \mathbb E_y [y^\top ( G/n + \lambda  I_n)^{-2} y] = \zeta^2 n^{-1} \trace(( G + \lambda  I_n)^{-2})\\
% %  &= \zeta^2\frac{1}{d}\sum_{i=1}^n\dfrac{1}{(\lambda+\nu(h)+\lambda_i(h'(0) X X^\top/d + h(0) \ones_n\ones_n^\top))^2}+o_{n,\mathbb P}(1)\\
% %  &= \zeta^2 \cdot \robdim_h(\lambda;\gamma)+o_{n,\mathbb P}(1),
% %  \end{split}
% %  \end{eqnarray*}
% % where in the last step we have used Lemma \ref{lm:sMP} and the fact that a finite-rank psd perturbation does not affect the limiting spectral density of a psd random matrix (thanks to eigenvalue interlacing).
% %  Similarly, we compute $\var_y(n^{-1}\| c\|^2) = n^{-1} \zeta^4\cdot n^{-1}\trace(( G+\lambda  I_n)^{-4})=\mathcal O_{n,\mathbb P}(1/d)=o_{n,\mathbb P}(1)$. We deduce that $n^{-1}\| c\|^2 = \zeta^2 \robdim_h(\lambda;\gamma)+o_{n,\mathbb P}(1)$,
% %  and the result follows from \eqref{eq:poincare}.
% \end{proof}

% \begin{proof}[Proof of Theorem \ref{thm:master}]
% Let $z := f_\star( X) = (f_\star(x_1),\ldots,f_\star(x_n)) \in \mathbb R^n$, so that $y = z + \varepsilon$. % , and let $\widehat{f}_{h,\lambda}^{\text{noise}}$ be the model obtained by fitting only on the noise vector $\varepsilon$.

% \paragraph{-- Decomposition.} Thanks to Lemma \ref{lm:kridgerob}, we have the decomposition
% \begin{eqnarray}
% \begin{split}
% \mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2] &= \mathbb E_{ X,\varepsilon}[y^\top R y] = \mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon + z^\top R z^\top + 2\varepsilon^\top R z]\\
% &=\underbrace{\mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon]}_{\text{contribution of noise}} + \underbrace{\mathbb E_ X[f_\star( X)^\top R f_\star( X)]}_{\text{contribution of signal}},
% \end{split}
% \label{eq:split}
% \end{eqnarray}
% where $ R$ is the random $n \times n$ psd matrix given in \eqref{eq:R}, and we have used the fact that $ X$ and $\varepsilon$ are independent with $\mathbb E[\varepsilon] = 0$ in the second line.
% Combining \eqref{eq:split} with Lemma \ref{lm:kridgerob}, we deduce that
% \begin{eqnarray}
% \mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2] \ge \mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon]=\mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}^{\text{noise}}_{h,\lambda})^2],
% \label{eq:splitineq}
% \end{eqnarray}
% where $\widehat{f}^{\text{noise}}_{h,\lambda}$ is the model obtained by fitting only on the noise-only response model \eqref{eq:noiseonly}.

% % It then remains to compute the asymptotics of $\mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon]$.

% \paragraph{-- Controlling contribution of noise-only response model.}
% Now, from Lemma \ref{lm:nonrobkernel} 
% %and the fact that $\alpha(h') = \gamma(h') = h'(0)^2$ and $\beta(h') = 0$ thanks to Lemma \ref{lm:curvcoefs} (which is applicable here, since $h \in \mathcal C^2$ at $0$ by Condition \ref{cond:smooth}(A)),
% we have the asymptotic expansion
% \begin{eqnarray}
%  n^{-1} \mathfrak{S}(\widehat{f}^{\text{noise}}_{h,\lambda})^2 =  \zeta^2 \cdot n^{-1}\mbox{trace}(h'(0)^2  X X^\top  G_0^{-2}) + o_{n,\mathbb P}(1),
% \end{eqnarray}
% where $ G_0:= h(0)\ones_n\ones_n^\top + h'(0) X X^\top + \overline{\lambda}_h  I_n \succ 0$. Further, we may ignore the rank-1 term to obtain (after some rearrangements)
% \begin{eqnarray}
% \begin{split}
% n^{-1}\mathfrak{S}(\widehat{f}^{\text{noise}}_{h,\lambda})^2 &= \zeta^2 \cdot \frac{1}{n}\sum_{i=1}^n \frac{\lambda_i( X X^\top)}{(\lambda_i( X X^\top) + \overline{\lambda}_h/h'(0))^2} + o_{n,\mathbb P}(1)\\
% &=\zeta^2 \cdot \int_{\mathbb R}\frac{\tau}{(\tau+\overline{\lambda}_h/h'(0))^2}d\mu_{\mathrm{MP}(\rho)}(\tau) + o_{n,\mathbb P}(1)\\
% & = \zeta^2 s_{\mathrm{MP}}(\overline{\lambda}_h/h'(0),1/\gamma)+o_{n,\mathbb P}(1),
% \end{split}
% \label{eq:mpcalc}
% \end{eqnarray}
% where $\mu_{\mathrm{MP}(\rho)}$ is the Marchenko-Pastur density with parameter $\rho := 1/\gamma$. In the second step of the above display,  the classical Marchenko-Pastur theory has been used to argue that in the limit \eqref{eq:proportionate},
% $$
% \dfrac{1}{n}\sum_{i=1}^n \dfrac{\lambda_i( X X^\top)}{(\lambda_i( X X^\top) + t)^2} \overset{a.s}{\to}  \int_{\mathbb R}\dfrac{\tau}{(\tau+t)^2}d\mu_{\mathrm{\mathrm{MP}}(\rho)}(\tau) =: s_{\mathrm{MP}}(t,1/\gamma).
% $$
% Combining \eqref{eq:splitineq} with \eqref{eq:mpcalc} yields the first part of the result, namely the lower-bound \eqref{eq:master}

% \paragraph{-- Under-regularized regime.}
% The second part of the result, namely \eqref{eq:chinda}, follows from taking limits on both sides of \eqref{eq:master} and invoking Lemma \ref{lm:slimits}. 
% \end{proof}

% \subsection{Exact formulae for linear response model: Proof of Theorem \ref{thm:linearsignal}}
% We now turn to the proof of Theorem \ref{thm:linearsignal}, linear the exact formule in the case of the linar data model \eqref{eq:linearf}.
% \begin{proof}[Proof of Theorem \ref{thm:linearsignal}]
% % \linearsignal*
% % \begin{proof}
% Setting $z := f_\star( X) =  X w_\star \in \mathbb R^n$, we know from \eqref{eq:split} that
% $$
% \mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2]= \mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda}^{\text{noise}})^2] + \mathbb E_ X[z^\top R z]=\mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda}^{\text{noise}})^2] + \mathbb E_ X[w_\star^\top  X^\top R  X w_\star],
% $$
% where $ R$ is the $n \times n$ random psd matrix given in \eqref{eq:R}.
% The asymptotic limit of the first term in the rightmost side of the above decomposition is given by \eqref{eq:mpcalc} in the proof of Theorem \ref{thm:master}. We only need to analyze the second term. To this end, we note that thanks to Lemma \ref{lm:crucial} with $A_0 = (1/d) X w_\star w_\star^\top  X^\top$), one has
% \begin{eqnarray}
% \begin{split}
% \mathbb E_ X[n^{-1} w_\star  X^\top R  X w_\star] &= \mathbb E_ X[n^{-1}w_\star^\top  X^\top ( G+\lambda  I_n)^{-1}( B \circ  X X^\top)( G+\lambda  I_n)^{-1}  X w_\star]\\
% &= \mathbb E_ X[n^{-1}w_\star^\top  X^\top  G_0^{-1} D_0  G_0^{-1} X w_\star] + o_{n}(1),
% \end{split}
% \end{eqnarray}
% where $ D_0 := h'(0) X X^\top$ and $ G_0 := h(0)\ones_n\ones_n^\top + h'(0)  X X^\top + (\lambda+\lambda_h) I_n$, and $B$ is as defined in \eqref{eq:R}.

% Next, because of rotational-invariance of the distribution on the rows $x_i$ of $ X$, we may rotate $w_\star$ to be parallel to, any coordinate axis $j$, so that
% \begin{eqnarray}
% \begin{split}
% \mathbb E_ X[n^{-1} w_\star  X^\top  G_0^{-1} D_0 G_0^{-1}  X w_\star] &= \|w_\star\|^2 \cdot \mathbb E_ X[n^{-1} ( X^\top  G_0^{-1} D_0 G_0^{-1}  X)_{j,j}]\\
% &=  \frac{\|w_\star\|^2}{d}\cdot \mathbb E_ X[n^{-1}\trace( X^\top  G_0^{-1} D_0  G_0^{-1} X)]\\
% &= \frac{\|w_\star\|^2}{d}\cdot \mathbb E_ X\left[\dfrac{1}{n}\sum_{i=1}^n\dfrac{\lambda_i( X X^\top)^2}{(\lambda_i( X X^\top)+\overline{\lambda}_h/h'(0))^2}\right] + o_{n}(1)\\
% &\to r_\star^2 \tilde{s}_{\mathrm{MP}}(\overline{\lambda}_h/h'(0),\gamma).
% \end{split}
% \end{eqnarray}
% \end{proof}

\subsection{Proofs of results for neural networks}
% \subsubsection{Infinite-width neural networks}
\begin{proof}[Proof of Corollary \ref{cor:nn}]
In case $\sigma$ is thrice-continuously differentiable, so are $h_\sigma^\rf$ and $h_\sigma^\ntk$ and so the result follows directly from Theorem \ref{thm:master}. For the nonsmooth cases, we focus on the ReLU activation, as the others follow a completely analogous argument. So, consider the infinite-width limit of a two-layer neural network with ReLU activation function $\sigma(z) := \max(z,0)$. The corresponding inner-product kernel function is given by (see appendix for derivation)
\begin{eqnarray}
h(t) = \frac{t\arccos(-t) + \sqrt{1-t^2}}{2\pi},\, t \in [-1,1].
\label{eq:arccos}
\end{eqnarray}
This kernel function (usually referred to as the \textit{arc-cosine kernel} in the literature) arises from considering the infinite-width limit of a two-layer neural network with ReLU activation function defined by $\sigma(z) := \max(z,0)$ (see \cite{inductivebietti}, for example). It is clear that the kernel function \eqref{eq:arccos} is $\mathcal C^\infty$ on $(-1,1)$, with $h'(t) \equiv \arccos(-t)/(2\pi)$. Moreover, one computes $h(0)=\theta_0(\sigma)= 1/(2\pi)$, $h'(0)=\theta_2(\sigma) = 1/4 >0$, $h(1)=\theta_1(\sigma)=1/2$ and the  implicit regularization as
$\lambda_{h} := h(1)-h(0)-h'(0) = 1/2-1/(2\pi)-1/4
= 1/4-1/(2\pi) \approx 0.091 >0$.
Thus, this kernel function satisfies the conditions of Theorem \ref{thm:master}, and we obtain the conclusion of Corollary \ref{cor:nn} in the case of the ReLU activation function.
\end{proof}

% \subsubsection{Finite-width neural networks}
% \begin{proof}[Proof of Theorem \ref{thm:RFrobprofilebounds}]
% Under Condition \ref{cond:peche}, \cite[Theorem 6]{Mei2019} predicts that in the limit \eqref{eq:doubleproportionate}
% \begin{eqnarray}
%  \mathbb E_{W, X,\varepsilon}|\theta_\star(\sigma)\|\widehat{v}_{\rf,N,\lambda}\|_2^2-(\zeta^2 + r_\star^2)\alpha| = o_{d}(1),
% \end{eqnarray}

% where $\alpha \in (0,\infty]$ is as in the statement of Theorem \ref{thm:RFrobprofilebounds}.
% % Let $\widetilde{\sigma'}:[-1,1] \to \mathbb R$ be a function defined by
% % \begin{eqnarray}
% % \widetilde{\sigma'}(z) := \begin{cases} (\sigma'(z^+)+\sigma'(z^-))/2,&\mbox{ if }z\text{ is a jump-discontinuity of }\sigma',\\
% % \sigma'(z),&\mbox{ else.}
% % \end{cases}
% % \end{eqnarray}
% Combining the previous display with \eqref{eq:sandwich} gives and taking expectations over $W$, $ X$, and $\varepsilon$, and letting $N,n,d \to \infty$ as in \eqref{eq:doubleproportionate} while recalling the definition of $S_\rf(\gamma_1,\gamma_2,\zeta^2,\lambda)$ in \eqref{eq:RFrobprofile}, we get
% \begin{eqnarray}
% \lim_{\substack{N,d \to \infty\\d/N \to \gamma_2}}\mathbb E_{W}[\lambda_{\min}( B_{\rf,N}/d)] \le \frac{\theta_\star(\sigma)S_\rf(\gamma_1,\gamma_2,\zeta^2,\lambda)}{(\zeta^2 + r_\star^2)\alpha} \le \lim_{\substack{N,d \to \infty\\d/N \to \gamma_2}}\mathbb E_W[\lambda_{\max}( B_{\rf,N}/d)].
%  \label{eq:rfmd}
% \end{eqnarray}

% It remains to bound the spectrum of the matrix $(1/d)B_{\rf,N}$. By Lemma \ref{lm:approxsphericalmatrix}, we know that in the limit $N,d \to \infty$ with $d/N \to \gamma_2$, it holds that
%  \begin{eqnarray}
% \|(1/d)B_{\rf,N} - \theta_2(\sigma) (WW^\top/d)\|_{op} \overset{p}{\to} 0.
%  \end{eqnarray}
% Thanks to a result of Bai-Yin, the limiting extreme eigenvalues of $WW^\top/d$ are $(1 \pm \sqrt{1/\gamma_2})^2$ a.s, and so we deduce that
% \begin{eqnarray}
% \begin{split}
% \mathbb E_W[\lambda_{\min}( B_{\rf,N}/d)] &\to \theta_2(\sigma)(1-\sqrt{1/\gamma_2})^2,\\
% \mathbb E_W[\lambda_{\max}( B_{\rf,N}/d)] &\to \theta_2(\sigma)(1+\sqrt{1/\gamma_2})^2.
% \end{split}
% \end{eqnarray}
% This completes the proof upon combining with \eqref{eq:rfmd}.
% \end{proof}

% \subsection{Idea of Proof of Theorem \ref{thm:master}}
% Let us outline the key ideas in the proof of Theorem \ref{thm:master}; detailed proof of is proved in the appendix. At a high-level, the proof of the theorem parallels that of the case of linear kernels, namely Lemma \ref{lm:linear}, except that now the random matrix $ R$ matrix defined in \eqref{eq:R} is a nonlinear function of the data.
% % \paragraph{-- Step 1: Reduction of $\mathfrak {S}(\widehat{f}_{h,\lambda})^2$ to a random quadratic form.}

% \paragraph{-- Step 1: Decomposition.}
% Since the vector of labels in the training data is $y = f_\star( X) + \varepsilon=(f_\star(x_1)+\varepsilon_1,\ldots,f_\star(x_n)+\varepsilon_n) \in \mathbb R^n$, we have the following decomposition thanks to Lemma \ref{lm:kridgerob}
% \begin{eqnarray}
% \begin{split}
% d^{-1}\mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2] &:= d^{-1}\mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2] = d^{-1}\mathbb E_{ X,\varepsilon}[y^\top R y]\\
% &= d^{-1}\mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon + f_\star( X)^\top R f_\star( X)^\top + 2\varepsilon^\top R f_\star( X)] \\
% &=\underbrace{d^{-1}\mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon]}_{\text{contribution of label-noise}} + \quad\underbrace{d^{-1}\mathbb E_ X[f_\star( X)^\top R f_\star( X)]}_{\text{contribution of signal}},
% \end{split}
% \label{eq:split0}
% \end{eqnarray}
% where $ R$ is the random $n \times n$ psd matrix given in \eqref{eq:R}, and we have used the fact that $ X$ and $\varepsilon$ are independent with $\mathbb E[\varepsilon] = 0$ in the second line.
% Combining \eqref{eq:split0} with Lemma \ref{lm:kridgerob}, we deduce that
% \begin{eqnarray}
% S(h,\gamma,\zeta^2,\lambda) \ge \lim_{n,d \to \infty,\,d/n \to \gamma}d^{-1}\mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon]=\lim_{n,d \to \infty,\,d/n \to \gamma}\mathbb E_ X[d^{-1}\trace(R)].
% \end{eqnarray}
% % where $\widehat{f}^{\text{noise}}_{h,\lambda}$ is the model obtained by fitting only on the noise-only response model \eqref{eq:noiseonly}.


% \paragraph{-- Step 2: Contribution of label-noise.}
% By the previous step, we see that in the presence of label-noise, one can obtain a lower-bound for the robustness profile $S(h,\gamma,\zeta^2,\lambda)$ by analyzing $\mathbb E_ X[d^{-1}\trace(R)]$. In the Lemma \ref{lm:approxsphericalmatrix} and \ref{lm:nonrobkernel}, we use random matrix theory (RMT) to obtain a spectrally-consistent linearization of the matrices $ B \circ ( X X^\top)$ and $ G$ (the kernel gram matrix) appearing in the definition of the $ R$, namely
% \begin{eqnarray}
% \begin{split}
% \| B \circ ( X X^\top) - h'(0)^2  X X^\top\|_{op} = o_{n,\mathbb P}(1),\\
% \| G-(h(0)\ones_n\ones_n^\top + h'(0) X X^\top + \lambda_h  I_n)\|_{op} = o_{n,\mathbb P}(1),
% \end{split}
% \end{eqnarray}
% in the limit \eqref{eq:proportionate}. These linearizations allow us to (after some algebra) estimate $\mathbb E_ X[d^{-1}\trace(R)]$ by the RHS of \eqref{eq:master}, with vanishing error.

% The other parts of the claim follow from properties of the function $s_{\mathrm{MP}}$ defined in \eqref{eq:sMP}, established in the appendix.

% \subsection{Idea of Proof of Theorem \ref{thm:master}}
% Let us outline the key ideas in the proof of Theorem \ref{thm:master}; detailed proof of is proved in the appendix. At a high-level, the proof of the theorem parallels that of the case of linear kernels, namely Lemma \ref{lm:linear}, except that now the random matrix $ R$ matrix defined in \eqref{eq:R} is a nonlinear function of the data.
% % \paragraph{-- Step 1: Reduction of $\mathfrak {S}(\widehat{f}_{h,\lambda})^2$ to a random quadratic form.}

% \paragraph{-- Step 1: Decomposition.}
% Since the vector of labels in the training data is $y = f_\star( X) + \varepsilon=(f_\star(x_1)+\varepsilon_1,\ldots,f_\star(x_n)+\varepsilon_n) \in \mathbb R^n$, we have the following decomposition thanks to Lemma \ref{lm:kridgerob}
% \begin{eqnarray}
% \begin{split}
% d^{-1}\mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2] &:= d^{-1}\mathbb E_{ X,\varepsilon}[\mathfrak{S}(\widehat{f}_{h,\lambda})^2] = d^{-1}\mathbb E_{ X,\varepsilon}[y^\top R y]\\
% &= d^{-1}\mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon + f_\star( X)^\top R f_\star( X)^\top + 2\varepsilon^\top R f_\star( X)] \\
% &=\underbrace{d^{-1}\mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon]}_{\text{contribution of label-noise}} + \quad\underbrace{d^{-1}\mathbb E_ X[f_\star( X)^\top R f_\star( X)]}_{\text{contribution of signal}},
% \end{split}
% \label{eq:split0}
% \end{eqnarray}
% where $ R$ is the random $n \times n$ psd matrix given in \eqref{eq:R}, and we have used the fact that $ X$ and $\varepsilon$ are independent with $\mathbb E[\varepsilon] = 0$ in the second line.
% Combining \eqref{eq:split0} with Lemma \ref{lm:kridgerob}, we deduce that
% \begin{eqnarray}
% S(h,\gamma,\zeta^2,\lambda) \ge \lim_{n,d \to \infty,\,d/n \to \gamma}d^{-1}\mathbb E_{ X,\varepsilon}[\varepsilon^\top R \varepsilon]=\lim_{n,d \to \infty,\,d/n \to \gamma}\mathbb E_ X[d^{-1}\trace(R)].
% \end{eqnarray}
% % where $\widehat{f}^{\text{noise}}_{h,\lambda}$ is the model obtained by fitting only on the noise-only response model \eqref{eq:noiseonly}.


% \paragraph{-- Step 2: Contribution of label-noise.}
% By the previous step, we see that in the presence of label-noise, one can obtain a lower-bound for the robustness profile $S(h,\gamma,\zeta^2,\lambda)$ by analyzing $\mathbb E_ X[d^{-1}\trace(R)]$. In the Lemma \ref{lm:approxsphericalmatrix} and \ref{lm:nonrobkernel}, we use random matrix theory (RMT) to obtain a spectrally-consistent linearization of the matrices $ B \circ ( X X^\top)$ and $ G$ (the kernel gram matrix) appearing in the definition of the $ R$, namely
% \begin{eqnarray}
% \begin{split}
% \| B \circ ( X X^\top) - h'(0)^2  X X^\top\|_{op} = o_{n,\mathbb P}(1),\\
% \| G-(h(0)\ones_n\ones_n^\top + h'(0) X X^\top + \lambda_h  I_n)\|_{op} = o_{n,\mathbb P}(1),
% \end{split}
% \end{eqnarray}
% in the limit \eqref{eq:proportionate}. These linearizations allow us to (after some algebra) estimate $\mathbb E_ X[d^{-1}\trace(R)]$ by the RHS of \eqref{eq:master}, with vanishing error.

% The other parts of the claim follow from properties of the function $s_{\mathrm{MP}}$ defined in \eqref{eq:sMP}, established in the appendix.

% The rest of the analysis will be more or less about using tools from random matrix theory to analyze the trace of the random matrix $ R$ appearing in \eqref{eq:kridgerob}.

% \subsection{Upper-bound for general nonlinear kernel}
% \lorem

% \lorem


% \paragraph{Comparison to ground-truth model $f_\star$.} One may ask how the robustness of unregularized kernel regressor $\widehat{f}_{h,0}$ compares to that of the linear ground-truth model $f_\star$ defined in \eqref{eq:linearf}. To answer this question, note that $d^{-1}\mathfrak{S}(f_\star)^2 = \|w_\star\|^2/d \to r_\star^2 \ge \dfrac{r_\star^2}{\underline{\gamma}}$, with equality iff $\gamma = 1$ (square design matrix). Thus, for kernel functions verying Condition \ref{cond:smooth} and $h'(0)>0$, we see from Theorem \ref{thm:linearsignal}(A) that 
% \begin{itemize}
% \item[--]\textbf{Under-parametrized.} If $\gamma \ge 1$ (i.e more data than parameters), then the unregularized kernel regressor $\widehat{f}_{h,0}$ is less robust than $f_\star$ in the presence of label noise.
% \item[--]\textbf{Evenly-parametrized.} If $\gamma=1$ (i.e as much data as parameters), then $\widehat{f}_{h,0}$ is as robust as the ground-truth model $f_\star$ in the noiseless regime where $\zeta=0$.
% \item[--]\textbf{Over-parametrized.} If $\gamma < 1$ (i.e more parameters than data), then in the noiseless regime, % $d^{-1}\mathfrak{S}(\widehat{f}_{h,0})^2$ is less than $f_\star$ on average (over randomness in the design matrix $ X$), in other words, in this noiseless regime,
% $\widehat{f}_{h,0}$ is more robust than the ground-truth model!
% \end{itemize}

% \paragraph{More data hurts robustness!} The arguments in the previous paragraph lead us to the conclusion that, (at least for kernel methods), more data hurts robustness, as the method is likely to memorize the label noise during training, at the expense of smoothness. This answers  Question \ref{question:morewhat}, for kernel methods with kernel function $h$ verifying Condition \ref{cond:smooth} and $h'(0)>0$.

% \lorem

% For certain kernel methods (e.g polynomial and exponential kernel methods), we will establish that
% \begin{eqnarray}
% d^{-1}\trace( D_0\widetilde{g}^{-2}) = \Theta_{n,\mathbb P}(1),
% \end{eqnarray}
% % in the limit $n,d \to \infty$  with $d/n \to \gamma$ and the regularization parameter $\lambda$ held fixed,
% which immediately implies that $\mathfrak S(\widehat{f}_{h,\lambda})^2 \sim n$ (w.h.p), i.e the nonrobustness varies as the sample size $n$ (w.h.p).


==> continuity.tex <==
\subsection{Statistical Considerations}
\textcolor{red}{TODO: This sub-section needs cleanup and double-checking. Maybe remove it altogether!}
\begin{restatable}{prop}{}
(A) For any attack strength $r \ge 0$ and $w_0 \in \mathbb R^d$, the adversarial risk $w \mapsto E(w,r)$ is a continuous function. (B) For any attack strength $r \ge 0$ and accuracy tolerance $\epsilon \ge 0$, $E_{opt}(r,\epsilon)$ defined in \eqref{eq:Eopteps} is a continuous function of the generative model $w_0$ and covariance matrix $\Sigma$.
\end{restatable}
The above result has some important statistical implications which we now outline.

\begin{restatable}[Chasing the Wrong Model ?]{cor}{}
$\widehat w_n$ is a consistent estimator of $w_0$ in the sense that $\|\widehat w_n - w_0\|_2 \to 0$ in some sense, then for any $r \ge 0$, it holds that $E(\widehat w_n,r) \to E(w_0,r)$. % in the same sense. 
\end{restatable}
Thus, such an estimator inherits the robustness profile of $w_0$.

\paragraph{Two-Stage Estimators.}
In \cite{Xing2021,MeyerAndDohmatob2023}), two-stage estimators for computing the robust-optimal model $w_{opt}(r)$ were proposed, corresponding to $\epsilon=1$. The following result generalizes the analysis to any level of accuracy tolerance $\epsilon$.
\begin{restatable}{cor}{}
Let $\widehat w_0$ and $\widehat \Sigma$ be consistent estimators\footnote{The assumed consistency of $\widehat \Sigma_n$ is w.r.t operator-norm, i.e we are assuming that $\|\widehat \Sigma_n - \Sigma\|_{op} \to 0$.} of the generative model $w_0$ and covariance matrix $\Sigma$.
% (e.g from training data) to obtain consistent estimators$\widehat w_n$ and $\widehat \Sigma_n$.
Let $r,\epsilon \ge 0$ be given.
In the definition of $E(w,r)$, plug-in the above estimators in the place of $w_0$ and $\Sigma$, and minimize it over $w \in \mathcal W_\epsilon$ to obtain a model $\widehat w_{opt,n}(r,\epsilon)$.
Then, $E(\widehat w_{opt,n}(r,\epsilon),r) \to E(w_{opt}(r,\epsilon),r) = E_{opt}(r,\epsilon)$.
\end{restatable}


==> contributions.tex <==
\section{General Results}
\label{sec:main}
\subsection{Preliminaries}
\paragraph{An Important Auxiliary Function.} Define the auxiliary function $\gamma:\mathbb R_+ \to \mathbb R_+$ by
\begin{eqnarray}
\gamma(r) := \inf_{w \in \mathbb R^d} K(w,r),\text{ where } K(w,r):= \|w-w_0\|_\Sigma + r\|w\|_\star.
\end{eqnarray}
Note that apart from the explicit on $r$, the scalar $\gamma(r)$ implicitly depends on attack norm $\|\cdot\|$, the feature covariance matrix $\Sigma$, and the generative model $w_0$.
\begin{restatable}{rmk}{}
The function $\gamma$ can be seen as a kind of "modolus of smoothness" of the generative model $w_0$ w.r.t the covariance structure of the features. This connection can be put on rigorous footing. Indeed, let consider the space of linear $\mathcal F_{lin}$ is the linear function space defined by $\mathcal F_{lin} := \{f_w \mid w \in \mathbb R^d\}$, with $f_w(x):=x^\top w$. Then, $\gamma(r)$ is nothing but Peetre's K-functional between the following Banach spaces:
\begin{itemize}
\item $\mathcal F_{lin}$ equipped with the norm $\|f_w\| := \|w\|_\Sigma$, and
\item  $\mathcal F_{lin}$ equipped with the norm $\|f_w\| := r\|w\|_\star$.
\end{itemize}
\end{restatable}

Note that one always has
\begin{eqnarray}
\label{eq:gammatrivial}
\begin{split}
\gamma(r) &\le \min(K(w_0,r),K(0,r))\\
&= \min(r\|w_0\|_\star,\|w_0\|_\Sigma)\\
&\le \|w_0\|_\Sigma.
\end{split}
\end{eqnarray}
Note that the above upper bound immediately implies that $\gamma$ is a bounded function. In general this upper-bound can be greatly improved. For any $r \ge 0$, consider the subset $S(r)$ of $\mathbb R^d$ defined by
\begin{eqnarray}
    S(r) := \{w \in \mathbb R^d \mid \|w\|_\star \le r,\, \|w\|_{\Sigma^{-1}} \le 1\}.
\end{eqnarray}
The following elementary lemma was established in Scetborn and Dohmatob (AISTATS 2023).
\begin{restatable}{lm}{}
\label{lm:gamma}
For any $r \ge 0$, we have the identity
\begin{eqnarray}
\gamma(r) = \sup_{z \in S(r)}z^\top w_0,
\end{eqnarray}
that is $\gamma(r)$ is the support function of the set $S(r)$, evaluated at the point $w_0$.

Moreover, we have the bounds
\begin{eqnarray}
\label{eq:gammasandwich}
    \min(1,r/r_1) \le \frac{\gamma(r)}{\|w_0\|_\Sigma} \le \min(1,r/r_0).
\end{eqnarray}
\end{restatable}
Note that the RHS of \eqref{eq:gammasandwich} is just a restatement of \eqref{eq:gammatrivial}. \textcolor{red}{TODO: The LHS is less trivial. Provide a proof here!}

% \paragraph{Relation to Gaussian Width.} The following lemma will be crucial in the sequel.
% \begin{restatable}{lm}{}
% Let $r \ge 0$ and let $\omega(S(r))$ be the Gaussian width of the set $S(r)$. Then, for $w_0 \sim N(0,I_d)$, it holds w.p $1-\delta(r)$ that $\gamma(r) \asymp \omega(S(r))$, where $\delta(r):=  e^{-\omega(S(r))^2/(2\min(r,1/\lambda_{min}(\Sigma))^2)}$.
% \label{lm:gaussianwidth}
% \end{restatable}
% \begin{proof}
%     First observe that thanks to Lemma \ref{lm:gamma}, we have
%     \begin{eqnarray}
%     \mathbb E \left[\gamma(r)\right] = \mathbb E \left[\sup_{z \in S(r)}z^\top w_0\right] =: \omega(S(r)),
%     \end{eqnarray}
% where the expectations are w.r.t $w_0 \sim N(0,I_d)$.

% Next, observe that the function $G(w) := \sup_{z \in S(r)} z^\top w$ is $\min(r,1/\lambda_{min}(\Sigma))$-Lipschitz w.r.t to the Euclidean-norm The result then follows from the concentration of Lipschitz functions \cite{boucheron2013}.
% \end{proof}

\subsection{A Two-Sided Oracle Bound: Reduction to Scalar Convex Optimization}
We start with the following two-sided oracle bound which will be our main workhorse for the sequel.
\begin{restatable}{prop}{gammaoracle}
\label{prop:oracleexact}
For an attack of strength $r \ge 0$ w.r.t any norm $\|\cdot\|$, and excess ordinary risk level $\epsilon > 0$, it holds that
\begin{eqnarray}
    E_{opt}(r,\epsilon)^2 \asymp \sigma^2 + h(r,\epsilon)^2,
\end{eqnarray}
where $h(r,\epsilon) := \sup_{\lambda \ge 0} (1+\lambda)\gamma(\frac{r}{1+\lambda})-\lambda\epsilon\|w_0\|_\Sigma$.

In particular, it holds that
\begin{eqnarray}
    E_{opt}(r) \asymp \sigma^2 + \gamma(r)^2.
\end{eqnarray}
\label{prop:gammaoracle}
\end{restatable}
Thus, the name of the game is to estimate the quantity $h(r,\epsilon)$, as a function of the attack strength $r$ and the excess risk level $\epsilon$. The good thing here is that unlike our ultimate target $E_{opt}(r,\epsilon)$ which is defined as an optimization problem over a nontrivial subset of $\mathbb R^d$, the auxiliary function $h$ is defined a scalar optimization problem over the half-line $\mathbb R_+$.

The prove of Proposition \ref{prop:oracleexact}, given Appendix abc, is based on \emph{Lagrangian Strong Duality}, in the form of \emph{Slater's Theorem}. 

% The proof of the proposition is given in the Appendix, and relies on \emph{Lagragian Strong Duality} which is allowed because of the convexity of the problem and the fact that constraint set has non-empty interior (in fact, it contains $w_0$).
% Also, it is convenient that the impact of the noise level $\sigma$ is separated from the impact of the other problem parameters, namely the attack strength $r$ and the excess risk level $\epsilon$. 



\section{Results for Euclidean-Norm Attacks under Spectral Conditions}
\label{sec:precise}
Let $\Sigma=\sum_{k=1}^d \lambda_k \phi_k\phi_k^\top$ be the singular-value decomposition of the feature covariance matrix $\Sigma$, with eigenvalues $\lambda_1 \ge \ldots \ge \lambda_d$.
Let $c_k=\phi_k^\top w_0$ be the coefficient of the generative model $w_0$ in $k$th eigen-direction of $\sigma$, i.e
\begin{eqnarray}
    w_0 = \sum_{k=1}^d c_k \phi_k.
\end{eqnarray}

In this section we will only consider Euclidean-norm attacks. We will give exact non-asymptotic estimates for $E(r,\epsilon)$ under different laws for the spectral decay of the feature covariance matrix $\Sigma$. 

\subsection{Structure of Optima}
\begin{restatable}{prop}{lagrangian}
\label{prop:lagrangian}
For any $r,\epsilon \ge 0$, it holds that
\begin{eqnarray}
    E_{opt}(r,\epsilon) \asymp \sup_{\lambda \ge 0}(1+\lambda)\newgamma(r/\sqrt{1+\lambda}) - \epsilon^2\|w_0\|_\Sigma^2\lambda,
\end{eqnarray}
where $\newgamma(t) := \min_w \|w-w_0\|_\Sigma^2 + t^2\|w\|_\star^2$.
\end{restatable}
\begin{restatable}{thm}{ridge}
\label{thm:ridge}
$E_{opt}(r,\epsilon) \asymp E(w(\lambda),r)$,
where 
\begin{eqnarray}
w(\lambda) = (\Sigma + r(\lambda)^2 I_d)^{-1}\Sigma w_0,
\end{eqnarray}
$t = r(\lambda) := r/\sqrt{1+\lambda}$ maximizes the 1D function $H:(0,r^2] \to \mathbb R$ defined by
\begin{eqnarray}
    H(t) := \sum_k \frac{\lambda_k c_k^2}{\lambda_k + t} - \frac{\epsilon^2\|w_0\|_\Sigma^2}{t} =  \sum_k \frac{\lambda_k c_k^2}{\lambda_k + t} - \frac{\epsilon^2}{t}\sum_k \lambda_k c_k^2.
\end{eqnarray}
\end{restatable}
Note that $w(\lambda)$ given in the theorem is a ridge. Such a result has also been derived in \cite{Xing2021} using a different approach. The advantage here is that the ridge parameter $t=r(\lambda)^2$ is the solution of a simple 1D optimization problem.

\begin{restatable}{rmk}{}
Is $c_k^2=1$ for all $k$, then $H(t)+\epsilon d/t = \sum_k \lambda_k/(\lambda_k + t)$ reduces to the level-$t$ effective dimension of the feature covariance matrix $\Sigma$, seen as a linear kernel-integral operator.
\end{restatable}

\begin{proof}
From Proposition \ref{prop:lagrangian}, we know that
$$
E_{opt}(r,\epsilon) \asymp \sigma^2 + \sup_{\lambda \ge 0}\inf_w (1+\lambda)\|w-w_0\|_\Sigma^2 + r^2\|w\|_2^2.
$$
Of course, the RHS is minimized when $w=w(\lambda):=(\Sigma + r(\lambda)^2 I_d)^{-1}\Sigma w_0$. This proves the first part of the claim.

For the second part, one computes
\begin{align*}
E(w(\lambda)) &=\|w(\lambda)-w_0\|_\Sigma^2 = r(\lambda)^4 \|(\Sigma+r(\lambda)^2I_d)^{-1}w_0\|_{\Sigma}^2 = r(\lambda)^4 \sum_k \frac{\lambda_k c_k^2}{(\lambda_k + r(\lambda)^2)^2},\\ \|w(\lambda)\|_2^2 &= \|(\Sigma+r(\lambda)^2 I_d)^{-1}\Sigma w_0\|_2^2 = \sum_k \frac{\lambda_k^2 c_k^2}{(\lambda_k + r(\lambda)^2)^2},\\
E(w(\lambda),r(\lambda)) &= \|w(\lambda)-w_0\|_\Sigma^2 + r(\lambda)^2 \|w(\lambda)\|_2^2 = \ldots = r(\lambda)^2 \sum_k \frac{\lambda_k c_k^2}{\lambda_k + r(\lambda)^2}.
\end{align*}
Thus, noting that $(1+\lambda)r(\lambda)^2 = r^2$, we see that optimal value of $\lambda$ can be gotten by solving the following 1D concave maximization problem
\begin{align}
E_{opt}(r,\epsilon) &\asymp \sigma^2 + \epsilon^2\|w_0\|_\Sigma^2 + r^2 \cdot \max_{0 \le t \le r^2} H(t),
\end{align}
where, we have used the convenient change of variable $t=r(\lambda)^2 = r^2/(1+\lambda) \in [0,r^2]$.
\end{proof}



% \input{oldpolynomial.tex}

\subsection{The Case Weak-Strong Features}
Consider the case where the eigenvalues $(\lambda_k)_k$ of the feature covariance matrix are given by
\begin{eqnarray}
    \lambda_k =  \begin{cases}
        1,&\mbox{ if }1 \le k \le d_1,\\
        b^2,&\mbox{ if } d_1 + 1 \le k \le d,
    \end{cases}
\end{eqnarray}
where $b \in [0,1]$ and $d_1 \in [1,d-1]$ is an integer. The first $d_1$ eigen-directions of the covariance matrix $\Sigma$ are referred to as \emph{strong features}, while the remaining eigen-directions are referred to as \emph{weak features}. Further, define
\begin{eqnarray}
    d_2 := d-d_1 \in [1,d-1].
\end{eqnarray}
The special case where $b \ll 1$ will is important, as the remaiing $d_2$ eigen-directions of $\Sigma$ can be see as corresponding to spurious correlations. If in addition $d_1 = o(d)$, the situation is then analogous to that considered in \cite{tsipras18}, Albeit in binary classification.

Note for $x \sim N(0,\Sigma)$ it holds w.p that $\|x\|_2 \asymp \sqrt{d_1}+b\sqrt{d_2}$.

Define $u,v,c \ge 0$ by
\begin{eqnarray}
\begin{split}
    u &:= \sqrt{\sum_{j=1}^{d_1} c_j^2},\, v :=\sqrt{\sum_{j=d_1+1}^d c_j^2},\, R :=\|w_0\|_\Sigma = u+bv.    
\end{split}
\end{eqnarray}

\begin{restatable}{lm}{}
For a Euclidean-norm attack with strength $r \ge 0$, it holds that \begin{eqnarray}
\gamma(r) \asymp \min(1,r)u + \min(b,r)v.
\end{eqnarray}
\end{restatable}

\begin{restatable}{thm}{weakstrong}
\label{thm:weakstrong}
For Euclidean attack of strength $r \ge 0$ and for any excess risk level $\epsilon \ge 0$, 
\begin{eqnarray}
E_{opt}(r,\epsilon) \asymp \sigma^2 + h_0(r,\epsilon)^2,
\end{eqnarray}
where:

-- \textbf{ Below Threshold.} If $\epsilon \le \epsilon_\star := vb/R$,
then
\begin{eqnarray}
   h_0(r,\epsilon) =
   \begin{cases}
    (u+v)r,&\mbox{ if }0 \le r \le b,\\
(u+v-R\epsilon/b)r + R\epsilon,&\mbox{ if }b \le r \le 1,\\
    (u+vb-R\epsilon)r,&\mbox{ if }r \ge 1.
    \end{cases}
\end{eqnarray}

-- \textbf{Above Threshold.} If $\epsilon \ge \epsilon_\star$,
then
\begin{eqnarray}
    h_0(r,\epsilon) = \min(1,r)u + \min(b,r)v \asymp \gamma(r).
\end{eqnarray}
\end{restatable}
Thus, if $vb/R = o(1)$, i.e if $b = o(u/v)$, so that $\epsilon_\star=\Omega(1)$, then there is no cross-over / phase-transition. We shall see a few special cases.

% Now, if $c_k=1$ for all $k$, then $u=\sqrt{d_1}$ and $v=\sqrt{d_2}$, and so
% $$
% \epsilon_\star = \dfrac{vb}{R} = \dfrac{b\sqrt{d_2}}{\sqrt{d_1}+b\sqrt{d_2}} = \dfrac{b\sqrt{1-\rho}}{\sqrt\rho + b\sqrt{1-\rho}}.
% $$

% Thus, in order for $\epsilon_\star^2=\Omega(1)$, we need $b\sqrt{1-\rho} = \Omega(\sqrt\rho)$, i.e
% \begin{eqnarray}
% b^2 = \Omega(\frac{\rho}{1-\rho}).
% \end{eqnarray}
% Likewise, in order for $\epsilon_\star^2=o(1)$, we need $b\sqrt{1-\rho} = o(\sqrt\rho)$, i.e
% \begin{eqnarray}
% b^2 = o(\frac{\rho}{1-\rho}).
% \end{eqnarray}

\subsection{Phase-Transition in the Case of Only a Few Strong Features}
We now show an instance of the problem where there is indeed phase-transition. Consider a weak-strong feature setting with
\begin{eqnarray}
d_1=1,\, b^2 = 1/d,\,c_k^2=1\forall k \in [d],
\label{eq:fewstrong}
\end{eqnarray}
We will show that there is a catastrophic tradeoff between accuracy and robustness.
This scenario is homologous to the one considered in \cite{tsipras18}, albeit for binary classification and $\ell_\infty$-norm attacks. Observe that $u:=1$, $v=\sqrt d_2 = \sqrt{d-d_2}  \asymp\sqrt d$, and $R=u+bv \asymp 1 + 1 = 2$. Thus, $\epsilon_\star:=vb/R = 1$.  Taking $b \le r =o(1)$ and $\epsilon \in [0, \epsilon_\star]$, we are in \textbf{Case 1} exclusively,
\begin{eqnarray}
\begin{split}
h(r,\epsilon) \asymp (u+v-R\epsilon/b)r + R\epsilon \asymp (1-\epsilon)r\sqrt{d} + \epsilon\sqrt d.
\end{split}
\end{eqnarray}
Combining with  Proposition \ref{prop:oracleexact}, we conclude that 
\begin{eqnarray}
E_{opt}(r,\epsilon) \gtrsim \sigma^2 +  h(r,\epsilon)^2 \gtrsim \sigma^2 +  (1-\epsilon)^2 r^2 d
\end{eqnarray}
Noting that $\gamma(r) \asymp \min(1,r) + \min(b,r)\sqrt{d} \asymp r + b\sqrt d$, invoking Proposition \ref{prop:oracleexact}, it is easy to see in comparison that w.p over $w_0$,
\begin{eqnarray}
 E_{opt}(r) \asymp \sigma^2 + \gamma(r)^2 \asymp \sigma^2 + (r+b\sqrt d)^2 \asymp \sigma^2 + r^2+b^2 d \lesssim \sigma^2 + 1 + r^2.
\end{eqnarray}
Putting things together, we obtain the following result in this setting.
\begin{restatable}{cor}{}
Consider the weak-strong features regime with parameters as in \eqref{eq:fewstrong}. Consider Euclidean-norm attack with strength $r$ such that 
\begin{eqnarray}
r \ge b,\, r \to 0,\, r\sqrt d \to \infty,
\end{eqnarray}
and consider an excess ordinary risk level $\epsilon \in [0,1)$ fixed. Then,
\begin{align}
E_{opt}(r) &= O(1),\\
E_{opt}(r,\epsilon) &\gtrsim (1-\epsilon)^2 r^2 d \to \infty.
\end{align}
\end{restatable}
That is, even though robust models exist for this imperceptible attack, such models cannot have be accurate.

Note that in order to satisfy the conditions on the attack strength in the corollary, it suffices to take  $r =\sqrt{\log(d)/d}$. Importantly, we can show that this phenomenon disappears if the marginal variance $b^2$ of the weak features is of order $o(1/d)$.

\subsection{Phase-Transition in the Case of Many Strong Features}
Now consider the following weak-strong feature settings
\begin{align}
    d_1 &\asymp d,\, b^2 = O(1/d),\,c_k^2 = 1\forall k \in [d]\label{eq:manystrong1},\\
    d_1 &\asymp d,\, b^2 = \Theta(1),\,c_k^2 = 1\forall k \in [d]\label{eq:manystrong2}.
\end{align}
In the first case \eqref{eq:manystrong1}, it is easy to compute \begin{eqnarray}
u=\sqrt{d_1} \asymp \sqrt d,\, v=\sqrt{d_2} \lesssim \sqrt d,\,R=u+vb \ge u \asymp\sqrt d,\,\epsilon_\star := vb/R \lesssim 1/\sqrt d =o(1),
\end{eqnarray}
and thus there is really no tradeoff needed, thanks to Theorem \ref{thm:weakstrong}. In the second case \eqref{eq:manystrong2}, one has
\begin{eqnarray}
u \asymp \sqrt d,\,v \asymp \sqrt d,\,R=u+bv \asymp \sqrt{d},\,\epsilon_\star := vb/R = \Theta(1).
\end{eqnarray}
This second case \eqref{eq:manystrong2} essentially is an instance of the setting of isotropic features considered in Section xyz. We have
\begin{restatable}{cor}{}
Consider the setting \eqref{eq:manystrong2}, with Euclidean-norm attack of strength $r \ge 0$, where
\begin{eqnarray}
    r = O(1),\, r\sqrt d \to \infty.
\end{eqnarray}
For any $\epsilon \in [0,\epsilon_\star)$, where $\epsilon_\star= \Theta(1)$ is given in the preceding paragraph, it holds that
\begin{align}
    E_{opt}(r) &\asymp \sigma^2 + r^2 = O(1),\\
    E_{opt}(r,\epsilon) &\gtrsim \sigma^2 + r^2 d \to \infty.
\end{align}
\end{restatable}

If $\epsilon \ge \epsilon_\star$, then $E_{opt}(r,\epsilon) \asymp E_{opt}(r)$ for any $r \ge 0$.

\subsection{No Phase-Transition in the Case of Polynomial Spectral Decay}
\label{subsec:polynomial2}
Now, consider the polynomial spectral decay setting where
\begin{eqnarray}
\lambda_k = k^{-\beta},\text{ for all }k \in [d]\text{ and for some }\beta \in (1,\infty)
\end{eqnarray}
For simplicity, suppose the generative model $w_0$ has the same energy along every spectral direction of the feature covariance matrix, i.e
\begin{eqnarray}
c_k^2=1,\text{ for all } k \in [d].
\end{eqnarray}

We have the following result which shows the absence of phrase-transition in this setting.
\begin{restatable}{thm}{powerlaw}
\label{thm:powerlaw}
For any $r \ge d^{-\beta}$ and $\epsilon \ge 0$, and define $\epsilon_\star := (1/\beta)r^{2(1-1/\beta)}$.
The following hold:

-- If $0 \le \epsilon \le \epsilon_\star$, then
\begin{eqnarray}
    E_{opt}(r,\epsilon) \asymp E_{opt}(w_0,r) \asymp \sigma^2 + r^2 d.
\end{eqnarray}

-- If $\epsilon \ge \epsilon_\star$, then
\begin{eqnarray}
    E_{opt}(r,\epsilon) \asymp E_{opt}(r) \asymp \sigma^2 + \epsilon^2 + r^{2(1-1/\beta)}.
\end{eqnarray}
\end{restatable}

% \input{exponential-decay.tex}

%\input{infnorm-attacks.tex}

\section{Statistical Consequences}
\label{sec:consequences}

\section{Concluding Remarks}
\lorem 

\lorem

==> convex-analysis.tex <==
\begin{proposition}
Let $f,g:\mathbb R^d \to \mathbb R$ be functions such that
\begin{itemize}
\item $g$ has at least one minimizer $a \in \mathbb R^d$.
\item For every $t \ge 0$, the function $L_t := f + t g$ has a minimizer $x(t) \in \mathbb R^d$. In particular, this means that $f$ has at least one minimizer. Define $x(\infty)=a$.
\item The equation $g(x(t)) = 0$ has a solution in $t_{opt} \in [0,\infty]$
\end{itemize}
Then, it holds that
\begin{eqnarray}
    f(x(t_{opt})) = \inf_{g(x) \le 0} f(x).
\end{eqnarray}
\end{proposition}

\begin{proof}
It is clear that
\begin{eqnarray}
f(x(t)) = \min_{g(x) \le g(x(t))} f(x)
\end{eqnarray}
Indeed, let $x \in \mathbb R^d$ such that $g(x) \le g(x(t))$. By definition of $x(t)$, we have
$$
f(x(t)) + t g(x(t)) = L_t(x(t)) \le L_t(x) = f(x) + t g(x),
$$
and it follows that $f(x(t)) \le f(x) + t (g(x)-g(x(t)))  \le f(x)$.

Now, let $f_{opt} := \inf_{g(x)\le 0}f(x)$. For any $t \ge 0$, observe that
\begin{itemize}
\item[--] If $g(x(t)) \le 0$, then
$$
f(x(t)) = \inf_{g(x) \le g(x(t))} f(x) \ge \inf_{g(x) \le 0}f(x) =: f_{opt},
$$
i.e $f(x(t)) \ge f_{opt}$.
\item[--] Analogously, if $g(x(t)) \ge 0$, then 
$$
f(x(t)) = \inf_{g(x) \le g(x(t))} f(x) \le \inf_{g(x) \le 0}f(x) =: f_{opt},
$$
$f(x(t)) \le f_{opt}$.
\end{itemize}
We conclude that $f_{opt} = f(x(t_{opt}))$,
where $t_{opt}$ is as in the proposition.
\end{proof}

\subsection{Proof of Proposition \ref{prop:lagrangian}}
The proof follows from the previous proposition with the choise of functions defined by $f(w) = f_r(w) := K(w,r)$ and $g(w) = f_r(w) := \|w-w_0\|_\Sigma^2-\epsilon^2 \|w_0\|_\Sigma^2$; with the identification $\lambda = r^2/(1+t)$ and $w(\lambda) = x(t)$, and  the fact that the function $G$ defined in \eqref{eq:F} is decreasing in $t$, and so the equation $g(x(t)) = 0$, i.e $G(\lambda) = \epsilon^2 \|w_0\|_\Sigma^2$ has a unique solution $\lambda_{opt}(r,\epsilon) \in [0,r]$.

==> experimental_setup.tex <==
\section{Experimental Details}
\label{sec:expe}

\subsection{Role of Over-Parametrization (Figure \ref{fig:overparam})}
\label{subsec:overparamexp}
For this experiment, the input-dimension is fixed at $d=1000$, and the covariance matrix of the features is $\Sigma=I_d$. The generative model $w_0$ is sampled from $N(0,I_d)$. For each sample size $n$ ranging over the set $\{10, 20, \ldots,100\} \cup \{100,200,300,\ldots,1000\}$, we generate an iid training dataset $\mathcal D_n$ of size $n$ from the distribution \eqref{eq:generator} with label-noise std $\sigma=0.1$, and compute the ordinary least-squares (OLS) estimator $\widehat w_n^{OLS}$; we then use Lemma \ref{lm:analytic} to analytically compute its adversarial risk $E^{\|\cdot\|_2}(\widehat w_n^{OLS},r)$ w.r.t Euclidean-norm attack for different values of the attack strength $r$. This experiment is run 5 times to produce error bars.
% For the lower-bound (green curve), we use \eqref{eq:nflt} with $\epsilon$ taken as the RHS of \eqref{eq:hastie}.
% The results are shown in Figure \ref{fig:overparam}.

\subsection{Failure of Lasso-type Estimators (Figure \ref{fig:lasso})}
For this experiment, the sample size is fixed to $n=1000$ and the input-dimension $d$ sweeps the range from $10$ through $610$ in steps of $20$. The sparsity $s$ of the generative model $w_0$ is set to the floor of $\sqrt{d}$. The label-noise std $\sigma$ varies in $\{0, 0.1, 1\}$. For each tuple of these parameters, the generative model $w_0$ is sampled from $N(0,I_d)$, and the last $d-s$ components set to zero. Then an iid training dataset $\mathcal D_n$ is generated from the distribution \eqref{eq:generator}. The scikit-learn package is used to fine tune a Lasso estimator $\widehat w_n^{Lasso}$ (by optimizing cross-validated standard risk). The adversarial risk $E^{\|\cdot\|_\infty}(\widehat w_n^{Lasso},r)$ w.r.t $\ell_\infty$-norm attack with $r=\sqrt{\log(d)/s}$ is computed analytically via Lemma \ref{lm:analytic}.

\subsection{Failure of OLS and GD (Figure \ref{fig:all})}
For this experiment, the sample size is set to $n=200$ and the input-dimension is set to $d=20$. We consider both Euclidean / $\ell_2$-norm and $\ell_\infty$-norm attacks. We generate an iid training dataset $\mathcal D_n$ of size $n$ from the distribution \eqref{eq:generator} with label-noise std $\sigma=0.1$, and compute the ordinary least-squares (OLS) estimator $\widehat w_n^{OLS}$, and compute its standard and adversarial risk as in Appendix \ref{subsec:overparamexp}. The OPT estimator shown for reference in the figure (3rd and 4th subplots from left to right) corresponds to the estimator which attains the optimum $E_{opt}^{\|\cdot\|}(r)$. In the case of Euclidean-norm attacks, this estimator is computing using the algorithm proposed in \cite{Xing2021}.

==> experiments.tex <==
\begin{figure*}[t]
    \centering
        \hspace{-0.15in}
\subfigure[Linear kernel]{\includegraphics[width=0.5\textwidth]{Linear_c2=0.1_zeta=1_reg=1e-05_results.pkl.pdf}\label{fig:toto}}
     	\hspace{-0.05in}
\subfigure[Exponential kernel]{\includegraphics[width=0.5\textwidth]{Exponential_c2=0.1_zeta=1_reg=1e-05_results.pkl.pdf}\label{fig:titi}}

\hfill
        \hspace{-0.15in}
\subfigure[Infinite-width ReLU NN (RF regime)]{\includegraphics[width=0.5\textwidth]{ReLURF_c2=0.1_zeta=1_reg=1e-05_results.pkl.pdf}\label{fig:titi}}
     	\hspace{-0.05in}
\subfigure[Infinite-width absval NN (RF regime)]{\includegraphics[width=0.5\textwidth]{AbsValRF_c2=0.1_zeta=1_reg=1e-05_results.pkl.pdf}\label{fig:titi}}
        \vspace{-.3cm}
                      \caption{Curves of normalized generalization $\widetilde{\varepsilon}$ and normalized robustness profile $\widetilde{S}$ versus aspect ratio $\gamma=d/n$, for unregularized kernel regression ($\lambda = 10^{-5}$) with target data from weak / strong features regime. For this experiment, we have $d=300$, $d_1=50$, $\rho_1=4$ and $\rho_2=0.1$. Solid curves correspond to theoretical values, while error-bars correspond to actual experiments (over 5 independent replications). We all show horizontal asymptotes at $0$ and $1$. The vertical lines correspond to interpolation thresholds at $n=d_1$ and $n=d_2$, for the linear model. Notice the match between empirical results and our theoretical estimates.}
    \label{fig:weakstrong}
\end{figure*}

\vspace{-.5cm}
\section{A toy experiment: weak / strong features regime}
%We run a simple experiment on simulated data to empirically verify our theoretical results.

\subsection{Experimental setup}
Inspired by \cite{RosacoSource2021}, we consider a scenario where the distribution of features is $N(0,\Sigma)$ and the covariance matrix $\Sigma$ of the features has $d_1 \in (0,d)$ "strong" eigen-directions and $d_2:=d-d_1 \in (0,d)$ "weak" eigen-directions. Thus, $\Sigma$ can be decomposed as $\Sigma = \rho_1 U_1U_1^\top + \rho_2 U_2 U_2^\top$, where $\rho_1$ is the variance of the strong features and $\rho_2<\rho_1$ is the variance of the weak features; $U_1$ is a $d \times d_1$ matrix whose columns correspond to the strong eigen-directions and $U_2$ is a $d \times d_2$ matrix whose columns correspond to the weak eigen-directions, and the union of the columns of $U_1$ and of $U_2$ forms an orthonormal basis for the entire feature space $\mathbb R^d$.
% \vspace{-.5cm}
\begin{figure*}[!h]
    \centering
        \hspace{-0.15in}
\subfigure[Linear kernel]{\includegraphics[width=0.25\textwidth]{Linear_c2=2_results.pkl.pdf}\label{fig:toto}}
        \hspace{-0.1in}
        \subfigure[Exponential kernel]{\includegraphics[width=0.25\textwidth]{Exponential_c2=2_results.pkl.pdf}\label{fig:titi}}
        \hspace{-0.1in}
\subfigure[Inf--width ReLU NN]{\includegraphics[width=0.25\textwidth]{ReLURF_c2=2_results.pkl.pdf}\label{fig:titi}}
        \hspace{-0.1in}
\subfigure[Inf--width absval]{\includegraphics[width=0.25\textwidth]{AbsValRF_c2=2_results.pkl.pdf}\label{fig:titi}}
        \vspace{-.3cm}
    \caption{Curves of normalized generalization $\widetilde{\varepsilon}$ and normalized robustness profile $\widetilde{S}$ for unregularized kernel regression with target data from the isotropic features regime. Solid curves correspond to our theoretical, while error-bars correspond to actual experiments (over 5 independent replications). Notice the match between empirical results and our theoretical estimates.
    We also show horizontal asymptotes at $0$ and $1$. The vertical line corresponds to the interpolation threshold $n=d$, for the linear model. The curves for the absolute activation function are flat: generalization error is at $1$ and robustness profile is at $0$, as predicted by Corollary \ref{cor:nn}.}
    \label{fig:strongstrong}
\end{figure*}
We run a small experiment in which, for the source condition $\phi$ in \eqref{eq:prior}, we consider two cases: (1) "Easy", where $\phi(s) = 1$ for all $s>0$; (2) "Hard", where $\phi(s) = 1/s$, for all $s>0$.
% \vspace{-.5cm}

\subsection{Results}
Results for the unregularized case ($\lambda = 10^{-5}$) are shown in Figure \ref{fig:weakstrong}.
The generalization error for the linear model has two "bumps", one at $n=d$ and another at $n=d_1$, in the case of the "hard" prior. The first bump is the well-known multiple-descent phenomenon, which occurs in the variance term of the generalization error of min-norm interpolators in the presence of label-noise. The existence of the second bump was established in \cite{RosacoSource2021}, and is due to the fact that the problem is essentially $d_1$-dimensional.
% We observe that all the models have a bump at $n=d_1$. Thus, there is double-descent in the robustness profile in weak-strong features model. To the best of our knowledge, this is the first time such a phenomenon is observed for kernel regression or infinite-width neural networks in linearized regimes. A similar phenomenon was observed in \cite{dohmatob2021fundamental}, in the case of finite-width networks.
The curves for the absolute activation function are flat: generalization error is at $1$ and robustness profile is at $0$, indicating that the resulting kernel regressor degenerates to the null-predictor. This is consistent with the phase-transition predicted in Corollary \ref{cor:nn}.

Figure \ref{fig:strongstrong} shows results for the particular case of isotropic features, where $\Sigma=I_d$. Notice that the second bump has now disappeared.

Finally, notice in both Figure \ref{fig:weakstrong} and \ref{fig:strongstrong}, a clear tradeoff between generalization error and robustness, in setups and models,  for mild values of $\gamma=d/n$ and above.

\paragraph{Effect of regularization.}
\begin{figure*}[t]
    \centering
        \hspace{-0.15in}
\subfigure[Linear kernel]{\includegraphics[width=0.5\textwidth]{Linear_c2=0.1_zeta=1_reg=0.1_results.pkl.pdf}\label{fig:toto}}
     	\hspace{-0.05in}
\subfigure[Exponential kernel]{\includegraphics[width=0.5\textwidth]{Exponential_c2=0.1_zeta=1_reg=0.1_results.pkl.pdf}\label{fig:titi}}

\hfill
        \hspace{-0.15in}
\subfigure[Infinite-width ReLU NN (RF regime)]{\includegraphics[width=0.5\textwidth]{ReLURF_c2=0.1_zeta=1_reg=0.1_results.pkl.pdf}\label{fig:titi}}
     	\hspace{-0.05in}
\subfigure[Infinite-width absval NN (RF regime)]{\includegraphics[width=0.5\textwidth]{AbsValRF_c2=0.1_zeta=1_reg=0.1_results.pkl.pdf}\label{fig:titi}}
        % \vspace{-.3cm}
        \caption{Mildly regularized ($\lambda=0.1$).}
\end{figure*}

% \section{Empirical confirmation}
% Our theoretical results are also confirmed empirically in Figure \ref{fig:main}.


% \subsection{Isotropic features}
% \lorem 

% \lorem

% \begin{figure*}[!h]
%     \centering
%     % \begin{subfigure}{\textwidth}
%     % \centering
%     \includegraphics[width=\linewidth]{main_results_sob2_normalized.png}
%     \includegraphics[width=\linewidth]{main_results_err_test_normalized.png}
%     % \caption{Nonrobustness measure}
%     % \end{subfigure}
%     % \hfill
%     % \begin{subfigure}{\textwidth}
%     % \centering
%     % \includegraphics[width=\linewidth]{main_results_err_test.png}
%     % \caption{Generalization error}
%     % \end{subfigure}
%     % \hfill
%     \caption{\textbf{Top row.} Relative robustness $\widetilde{S} := \mathfrak{S}(\widehat{f}_{h,\lambda})^2/r_\star^2$ of KRR model $\widehat{f}_{h,\lambda}$, for different kernel functions and values of explicit regularization parameter $\lambda$. Error-bars (whiskers) correspond to actual values of the relative nonrobustness $\widetilde{S}$ for 5 different runs of the experiment; solid lines correspond to our theoretical predictions (Theorem \ref{thm:linearsignal}). The black horizonal lines are the predicted asymptotic values of the relative robustness: a value of $0$ (i.e the KRR model becomes essentially a constant function) in the limit $\gamma \to \infty$, corresponding to infinitely more features than data data; and a value of $1$ (i.e the KRR model becomes exactly as robust as the ground-truth model $f_\star$) in the limit $\gamma \to 0^+$ corresponding to infinite more data $n$ than features. We see an excellent match between theory and experimental results. \textbf{Bottom row.} Mean generalization / test error over the 5 runs, shown here as a sanity check.}
%     \label{fig:main}
% \end{figure*}

% \subsection{Experiment 2: Influence of covariance structure of data}

% \paragraph{Features.}
% \lorem

% \paragraph{Ground-truth coefficients $w_\star$.}
% \lorem

% \begin{figure*}[!h]
%     \centering
%     % \begin{subfigure}{\textwidth}
%     % \centering
%     \includegraphics[width=\linewidth]{main_results_sob2_normalized.png}
%     \includegraphics[width=\linewidth]{main_results_err_test_normalized.png}
%     % \caption{Nonrobustness measure}
%     % \end{subfigure}
%     % \hfill
%     % \begin{subfigure}{\textwidth}
%     % \centering
%     % \includegraphics[width=\linewidth]{main_results_err_test.png}
%     % \caption{Generalization error}
%     % \end{subfigure}
%     % \hfill
%     \caption{\textbf{Top row.} Relative robustness $\widetilde{S} := \mathfrak{S}(\widehat{f}_{h,\lambda})^2/r_\star^2$ of KRR model $\widehat{f}_{h,\lambda}$, for different kernel functions and values of explicit regularization parameter $\lambda$. Error-bars (whiskers) correspond to actual values of the relative nonrobustness $\widetilde{S}$ for 5 different runs of the experiment; solid lines correspond to our theoretical predictions (Theorem \ref{thm:linearsignal}). The black horizonal lines are the predicted asymptotic values of the relative robustness: a value of $0$ (i.e the KRR model becomes essentially a constant function) in the limit $\gamma \to \infty$, corresponding to infinitely more features than data data; and a value of $1$ (i.e the KRR model becomes exactly as robust as the ground-truth model $f_\star$) in the limit $\gamma \to 0^+$ corresponding to infinite more data $n$ than features. We see an excellent match between theory and experimental results. \textbf{Bottom row.} Mean generalization / test error over the 5 runs, shown here as a sanity check.}
%     \label{fig:main}
% \end{figure*}

% In section \ref{subsec:exprealdata}, we present a small experiment on the MNIST dataset \cite{mnist} which suggests that our theoretical results may hold for real datasets (at least, when applied to the features obtained via neural networks, rather than the raw data).

==> exponential-decay.tex <==
\subsection{Exponential Spectral Decay}
Suppose $\Sigma=\mbox{diag}(\lambda_1,\ldots,\lambda_d)$, with
\begin{eqnarray}
\lambda_k \asymp e^{-c_1 k^\alpha},\text{for some constants }c_1 > 0,\,\alpha > 1/2.
\end{eqnarray}
    Note that $\|w_0\|_\Sigma^2 \asymp \mbox{tr}(\Sigma) \asymp \sum_{k \ge 0}e^{-c_1 k^\alpha} = \Theta(1)$ w.h.p over $w_0$. Moreovern in this regime, it was shown in \cite{Gauss2Kolmogorov} that $\omega(S(r)) \asymp r\log^{-\alpha/2}(1/r)$ for all $r \in (0,C']$. Combining with Lemma xyz we obtain w.h.p over a draw of $w_0 \sim N(0,I_d)$ that
\begin{eqnarray}
\gamma^{\|\cdot\|_2}(r) \asymp r \log^{-\alpha/2}(1/r),\text{ for all }r \in (0,C'].
\end{eqnarray}
For $r \in (0,C']$, one then computes
\begin{eqnarray}
    h(r,\epsilon) \gtrsim \sup_{\lambda \ge (r/C'-1)_+}m(\lambda) = \sup_{\lambda \ge 0}m(\lambda),
\end{eqnarray}
with $m(\lambda):= r\log^{-\alpha/2}(\dfrac{1+\lambda}{r})-\lambda\epsilon$. Taking derivatives, we have
$$
m'(\lambda) \equiv -\frac{\alpha}{2}\frac{\log^{-1-\alpha/2}(u(\lambda))}{u(\lambda)}-\epsilon,
$$
where $u(\lambda) := (1+\lambda)/r$. Since $r \in [0,1)$, observe that $m'$ is negative on all of $[0,\infty)$, and therefore $m$ attains a global maximum at $\lambda=0$, i.e one has $h(r,\epsilon) \asymp m(0) = r\log^{-\alpha/2}(1/r)$, for any $\epsilon \ge 0$.

==> half-baked-stats.tex <==
\section{Statistics (Half-Baked!)}
Let $\|\cdot\|$ be a norm on $\mathbb R^d$, $r \ge 0$, $a \in \mathbb R^d$ and $S$ be a $d \times d$ positive-definite matrix.  For any $x \in \mathbb R^d$, define $F(x; a, S) := \|x-a\|_S^2 + r^2 \|x\|^2$ and $G(x; a, s) := \|x-a\|_S + r\|x\|$, where $\|z\|_S := \|S^{1/2} z\|_2 = \sqrt{z^\top S z}$. Also, define $f(a, S) := \inf_x F(x;a,S)$ and $g(a,S) := \inf_x G(x; a,S)$. Finally, let $(a_n)_n$ be a sequence in $\mathbb R^d$ which converges to $a$ and let $(S_n)_n$ be a sequence of psd matrices converging to $S$.

**Question.** Is it true that $f(a_n, S_n) \to f(a,S)$  and $g(a_n, S_n) \to g(a,S)$ ?

Let $\delta_n := \|a_n-a\|$ and $\epsilon_n := \|T_n-I\|_{op}$, where $T_n := S^{-1/2}(S_n-S) S^{-1/2} = S^{-1/2} S_n S^{-1/2} - I$.
Let $b_n$ be a minimizer of $G(\cdot;a_n,S_n)$ and $b$ be a minimizer of $G(\cdot; a_n,S_n)$
Then, 
\begin{eqnarray}
\begin{split}
    G(b_n;a,S) - G(b;a,S) &= G(b_n;a,S) - G(b_n;a_n,S_n)\\
    &\quad\quad+G(b_n;a_n,S_n) - G(b;a_n,S_n)\\
    &\quad\quad  + G(b;a_n,S_n) - G(b; a, S)\\
    &=G(b_n;a,S) - G(b_n;a_n,S_n)\\
    &\quad\quad  + G(b;a_n,S_n) - G(b; a, S)\\
    &= \|b_n-a\|_S - \|b_n-a_n\|_{S_n} + \|b-a_n\|_{S_n} - \|b-a\|_S.
    \end{split}
\end{eqnarray}
Now, for any $x \in \mathbb R^d$, one has $\|x-a_n\|_S - \|x-a\|_{S_n} = \|x-a_n\|_S - \|x-a\|_S + \|x-a\|_S - \|x-a\|_{S_n}$. Now, $\|x-a_n\|_S - \|x-a\|_S \le \|a_n-a\|_S \le \|S\|_{op} \delta_n$. Furthermore, for any $z \in \mathbb R^d$, we have
\begin{eqnarray}
\begin{split}
 \|z\|_S - \|z\|_{S_n} &= \sqrt{z^\top S z} - \sqrt{z^\top S_n z} = \frac{z^\top S z - z^\top S_n z}{\|z\|_S + \|z\|_{S_n}} = \frac{z^\top (S-S_n) z}{\|z\|_S + \|z\|_{S_n}}\\
 &= \frac{-v^\top T_n v^\top}{\|v\|_2 + \|z\|_{s_n}} \le \frac{\|v\|_2^2 \|T_n\|_{op}}{\|v\|_2 + \|z\|_{S_n}} \le \|T_n\|_{op} \|v\|_2 = \epsilon_n \|z\|_S.
 \end{split}
\end{eqnarray}
Taking $z = b_n-a$ and using the triangle inequality $\|b_n-a\|_S \le \|b_n-b\|_S + \|b-a\|_S = O(1)$ gives
\begin{eqnarray}
\|b_n-a\|_S - \|b_n-a\|_{S_n} \le O(\epsilon_n).
\end{eqnarray}

==> infnorm-attacks.tex <==
\section{General $\ell_p$-Norm Attacks on Isotropic Features}
We now assume the features are isotropic, i.e the covariance matrix is $\Sigma=I_d$.
As in the previous section, we assume the generative model $w_0$ is a random draw from $N(0,I_d)$.

\subsection{$\ell_\infty$-Norm Attacks}
\begin{restatable}{thm}{}
The following hold w.h.p over $w_0$. For any $r \ge 0$, we have the the upper-bound
\begin{eqnarray}
    \sqrt{E_{opt}^{\|\cdot\|_\infty}(r,\epsilon)} - \sigma \le r\sqrt{\log d}.
\end{eqnarray}

Moreover, if $r \ge 1/\sqrt{d}$ and $0 \le \epsilon \le cd/\sqrt{\log d}$ for some absolute constant $c \in [0,1)$, then we have a matching lower-bound
\begin{eqnarray}
    \sqrt{E_{opt}^{\|\cdot\|_\infty}(r,\epsilon)} - \sigma \asymp r\sqrt{\log d}.
\end{eqnarray}
\end{restatable}
From Lemma \ref{lm:gamma} combined with Bellec's \url{https://arxiv.org/pdf/1705.10696.pdf} (See formula (1) therein), one readily obtains
\begin{restatable}{lm}{}
$\gamma^{\|\cdot\|_\infty}(r) \asymp \omega(rB_1^d \cap B_2^d) \asymp r\sqrt{\log(ed(1 \land 1/r^2))} \land \sqrt d$.
\end{restatable}
Observe that for any $R \ge 0$, we have
$\gamma^{\|\cdot\|_\infty}(R) \lesssim R \sqrt{\log d},\text{ with equality if }R = O(1)$ as $d \to \infty$.
Thus, taking $R=r/(1+\lambda)$, we deduce that if $1+\lambda \le r \le \sqrt{d}$, then
\begin{eqnarray}
(1+\lambda)\gamma^{\|\cdot\|_\infty}(\frac{r}{1+\lambda}) = \gamma^{\|\cdot\|_\infty}(R) \asymp (1+\lambda)R\sqrt{\log(ed/R^2)} = r\sqrt{\log(ed(1+\lambda)^2/r^2)}.
\end{eqnarray}

Therefore, if $1 \le r \le \sqrt{d}$, we deduce that
\begin{eqnarray}
\begin{split}
h(r,\epsilon) & \gtrsim \sup_{0 \le \lambda \le r-1}m(\lambda),
\end{split}
\end{eqnarray}
where $m(\lambda):=r\sqrt{\log(ed(1+\lambda)^2/r^2)}-\lambda\epsilon\sqrt{d} = r\sqrt{\log(ed/R^2)}-(r/R-1)\epsilon\sqrt{d}$. Now, the derivative of $m$ is 
$$
m'(\lambda) = \frac{R(\lambda)}{\sqrt{\log(ed/R(\lambda)^2)}}-\epsilon\sqrt d,
$$
which vanishes at $\lambda = \lambda_\star$ such that $R(\lambda_\star) = \sqrt{d}\sqrt{\epsilon^2 W(e/\epsilon^2)} \asymp \sqrt{d}\sqrt{\epsilon^2\log(1/\epsilon^2)}$ for $\epsilon \to 0^+$.

==> justification_proof.tex <==
\subsection{Justification for using Dirichlet energy as a measure of adversarial vulnerability}
\label{subsec:justice}
Before moving any further, it is important to pause and explain why our proposed measure of robustness \eqref{eq:sobeq} is actually a measure of robustness. This would in term explain why the nonrobustness profile \eqref{eq:robprofile} is the right thing to look at when study the robustness of kernel regression as a function of problem parameters (sample size, input dimension, choice of kernel function, amount of explicit regularization, etc.).

% \paragraph{The gradient correlation matrix.}
Given a continuously-differentiable function $f : \mathbb R^d \to \mathbb R$, consider the $d \times d$ psd matrix $J(f)$ defined by
\begin{eqnarray}
J(f; P) := \mathbb E_{x \sim P}[\nabla_x f(x) \nabla_x f(x)^\top].
\end{eqnarray}
We will see that the spectrum of this matrix plays a key role in quantifying the robustness of $f$, w.r.t the distribution $P$.
% \paragraph{Robustness to random local fluctuactions.}

\paragraph{Link with adversarial robustness error.}
The following lemma shows that $\mathfrak{S}(f; P)^2 = \trace(J(f; P))$, and measures the (non)robustness of $f$ to random local fluctuations in its input.
\begin{restatable}
%[Derivative of robustness error]
{lm}{}
\label{lm:justice}
We have % the identity.
\begin{eqnarray}
\lim_{\delta \to 0^+}\frac{1}{\delta}\mathbb E_{x \sim P}[\Delta_f(x;\delta)] = \mathfrak{S}(f) = \trace(J(f; P))^{1/2},
\end{eqnarray}
where $\Delta_f(x;\delta) := \sup_{\|v\|\le \delta}|f(x+v)-f(x)|$.
\end{restatable}
A generalized form of the lemma is proved in the appendix.

% \paragraph{Robustness to universal adversarial perturbations.}

\paragraph{Link with universal adversarial perturbations.}
The next lemma shows that $\|J(f;P)\|_{op}$ measures the (non)robustness of $f$ to universal adversarial perturbations, in the sense of \cite{moosavi17}.
\begin{restatable}
% [Measure of robustness to universal perturbations]
{lm}{}
We have the identity
\begin{eqnarray}
\lim_{\delta \to 0^+}\frac{1}{\delta}\Delta_f(\delta; P) = \|J(f; P)\|_{op}^{1/2},
\end{eqnarray}
where $\Delta_f(\delta)^2:=\sup_{\|v\| \le \delta}\mathbb E_{x \sim P}(f(x+v)-f(x))^2$.
\end{restatable}
In particular, the leading eigenvector of $J(f;P)$ corresponds to (first-order) universal adversarial perturbations of $f$, in the sense of \cite{moosavi17}, which can be efficiently computed using the \emph{Power Method}, for example.

A rough sketch of the proof of the above lemma is as follows. To first-order, we have $f(x+v) - f(x) \approx v^\top \nabla x f(x)$. Thus,
\begin{eqnarray*}
\begin{split}
\Delta_f(\delta;P)^2 &\approx \sup_{\|v\| \le \delta}\mathbb E_{x \sim P}[(f(x+v)-f(x))^2]\\
&= \sup_{\|v\| \le \delta}\mathbb E_{x \sim P}[(v^\top \nabla_x f(x))^2 ]\\
&= \sup_{\|v\| \le \delta} v^\top J(f;P) v = \delta^2 \|J(f;P)\|_{op}^2.
\end{split}
\end{eqnarray*}
% The first lemma is proved via a similar argument.

Let $\|\cdot\|$ be any norm on $\mathbb R^d$ with dual norm $\|\cdot\|_\star$.
Given \textbf{any} function $f:\mathbb R^d \to \mathbb R$, a tolerance parameter $\delta \ge 0$ (the \emph{attack budget}), and a scalar $q \ge 1$, define $R_{P,\delta}(f)$ by
\begin{eqnarray}
    R_{q,\delta}(f,g; P) := \mathbb E_{x \sim P}\left[\Delta_f(x;\delta)^q\right],
\end{eqnarray}
where $\Delta_f(x;\delta) := \sup_{\|x'-x\| \le \delta}|f(x')-f(x)|$ is the maximal variation of $f$ in  a neighborhood of size $\delta$ around $x$.
For $q=2$, we simply write $R_{P,\delta}(f,g)$ for $R_{P,\delta,2}(f,g)$.
In particular, under the model \eqref{eq:signalplusnoise}, $G_{P,\delta}(f) := \mathbb E[R_{\delta}(f,f_\star; P)]$ is \emph{adversarial generalization error} and $G_0(f) := \mathbb E [R_0(f,f_\star; P)]$ is the ordinary \emph{generalization error} of $f$, where the expectations are w.r.t all sources of randomness in $f$ and $f_\star$. Of course $G_{P,\delta}(f)$ is an increasing function of $\delta$.

\paragraph{Approximate measure of adversarial generalization error.}
Define $R_{q,\delta}(f;P) := R_{q,\delta}(f,f; P)$ and $R_{\delta}(f;P) := R_{2,\delta}(f,f;P)$, which measure the deviation of the outputs of $f$ w.r.t to the outputs of $f$, under adversarial attack. Note $R_{q}(f; P) \equiv 0$. Also note that in the case where $\|\cdot\|$ is the euclidean $L_2$-norm: if $f$ is a near perfect model (in the classical sense), meaning that it ordinary generalization error $G_0(f;P)$ is small, then $R_{\delta}(f;P)$ is a good approximation for $G_{\delta}(f;P)$. Finally, (at least for small values of $\alpha$), we can further approximate $R_{\alpha}(f)$ (and therefore $G_{\delta; P}(f)$, for near perfect $f$) by $\delta^2$ times the Dirichlet energy $\mathfrak{S}(f;P)^2$. Indeed,
\begin{restatable}{lm}{justification}
\label{lm:justification}
Suppose $f$ is $P$-a.e differentiable and for any $q \in [1,\infty)$, define $\mathfrak{S}_{q}(f;P)$  by
\begin{eqnarray}
\label{eq:Sq}
    \begin{split}
\mathfrak{S}_{q}(f;P) &:= \left(\mathbb E_{x \sim P}[\|\nabla_x f(x)\|_\star^q]\right)^{1/q}.
    \end{split}
\end{eqnarray}
(In particular, if $\|\cdot\|$ is the euclidean $L_2$-norm and $q=2$, then $\mathfrak{S}_q(f;P)^2$ is the Dirichlet energy defined in \eqref{eq:sobeq} as our measure of robustness). We have the following

\textbf{(A) General case.} $\mathfrak{S}_{q}(f;P)$ is the right derivative of the mapping $\delta \mapsto R_{\delta}(f;P)^{1/q}$ at $\delta = 0$. More precisely, we have the following
\begin{eqnarray}
    \lim_{\delta \to 0^+}\frac{R_{q,\delta}(f;P)^{1/q}}{\delta} = \mathfrak{S}_{q}(f;P),
\end{eqnarray}
or equivalently, $R_{q,\delta}(f;P) = \delta^q\cdot \mathfrak{S}_{P}(f;P)^q + \text{ Higher order terms in }\delta^q$.

\textbf{(B) Case of Dirichlet energy}
In particular, if $\|\cdot\|$ is the euclidean $L_2$-norm and we take $q=2$,
\begin{eqnarray}
R_{\delta}(f;P) = \delta^2\cdot \mathfrak{S}_{P}(f;P)^2 + \text{ Higher order terms in }\delta^2.
\end{eqnarray}
\end{restatable}

The proof follows directly from \emph{Fubini's Theorem} and the following lemma.
\begin{restatable}{lm}{strongslope}
\label{lm:strongslope}
If $f$ is differentiable at $x$, then the function $\delta \mapsto \Delta_f(x;\delta):=\underset{\|x'-x\| \le \delta}{\sup}|f(x')-f(x)|$ is right-differentiable at $0$ with derivative given by $\Delta_f'(x;0) = \|\nabla_x f(x)\|_\star$.
\end{restatable}
% \justification*

\begin{proof}
As $f$ is differentiable, $f(x') = f(x) + \nabla_x f(x)^\top (x'-x) + o(\|x'-x\|)$ around $x$. Therefore for sufficiently small $\delta$, if $B(x;\delta)$ is ball of radius $\delta$ around $x$, then
\begin{eqnarray}
    \begin{split}
\Delta_f(x;\delta) &= \sup_{x' \in B(x;\delta)}\mid \nabla_x f(x)^\top (x'-x)+o(\|x'-x\|)\mid\\
&\le \sup_{x' \in B(x;\delta)}|\nabla_x f(x)^\top(x'-x)| + \sup_{y \in B(x;\delta)} o(\|x'-x\|)\\
&=\|\nabla_x f(x)\|_\star\delta + \sup_{y \in B(x;\delta)} o(\|x'-x\|) \frac{\Delta_f(x;\delta)}{\delta}\\
&\le\|\nabla_x f(x)\|_\star+ \sup_{x' \in B(x;\delta)} \frac{ o(\|x'-x\|)}{\delta}
\end{split}
\end{eqnarray}
% where $\sup_{x' \in B(x;\delta)}|\nabla_x f(x)(x'-x)|=\|\nabla_x f(x)\|_\star\delta$ follows from Cauchy-Schwarz.
Note that $\sup_{x' \in B(x;\delta)} \dfrac{ o(\|x'-x\|)}{\delta}\rightarrow 0$. This proves $\limsup_{\delta \to 0^+}(1/\delta)\Delta_f(x;\delta) \le \|\nabla_x f(x)\|_\star$. Similarly, one computes 
\begin{eqnarray}
    \begin{split}
\Delta_f(x;\delta) &=\sup\mid \nabla_x f(x)^\top (x'-x)+o(\|x'-x\|)\mid \\ &\ge \sup|\nabla_x f(x)^\top (x'-x)| - \sup o(\|x'-x\|) \\ &=\|\nabla_x f(x)\|\delta -\sup o(\|y-x\|)
    \end{split}
\end{eqnarray}
Hence $\liminf_{\delta \to 0^+}(1/\delta)\Delta_f(x;\delta) \ge \|\nabla_x f(x)\|_\star$, and we conclude that $\delta \mapsto \Delta_f(x;\delta)$ is differentiable at $\delta=0$, with derivative $\Delta_f'(x;0) = \|\nabla_x f(x)\|_\star$ as claimed.
\end{proof}
\begin{proof}[Proof of Lemma \ref{lm:justification}]
By basic properties of limits, one has
\begin{eqnarray}
\begin{split}
\left(\lim_{\delta \to 0^+}\frac{R_{q,\delta}(f;P)^{1/q}}{\delta^q}\right)^q &= \lim_{\delta \to 0^+}\frac{R_{q,\delta}(f;P)}{\delta}\\
&= \lim_{\delta \to 0^+}\frac{\mathbb E_{x \sim P}[|\Delta_f(x;\delta)|^q]}{\delta}\\
&= \mathbb E_{x \sim P}\left[\lim_{\delta \to 0^+}\frac{|\Delta_f(x;\delta)|^q}{\delta}\right]\\
&=\mathbb E_{x \sim P}\left[\left(\lim_{\delta \to 0^+}\frac{|\Delta_f(x;\delta)|}{\delta}\right)^q\right]\\
&= \mathbb E_{x \sim P}[\|\nabla_x f(x)\|_\star^q]\\
&:= \mathfrak{S}_q(f;P)^q,
\end{split}
\end{eqnarray}
where the 3rd line is thanks to \emph{Fubini's Theorem}, and the 5th line is thanks to lemma \ref{lm:strongslope} (and the fact that $\Delta_f(x;0) \equiv 0$). Noting that $R_{q,0}(f;P) \equiv 0$ then concludes the proof.
\end{proof}

\clearpage



==> lousyproofsketch.tex <==
We now outline the key ideas of the proof of our main result Theorem \ref{thm:lousy}, % The full details are be provided in the appendix.
split into various steps. 

% \lorem
 % As usual, asymptotic notation $F(d) = O(G(d))$ (also written $F(d) \lesssim G(d)$) means there exists a constant $c$ such that $F(d) \le c\cdot G(d)$ for sufficiently large $d$, while $F(d) = \Omega(G(d))$ means $G(d) = O(F(d))$, and $F(d) = \Theta(G(d))$ or $F(d) \asymp G(d)$ means $F(d) \lesssim G(d) \lesssim F(d)$. Finally, $F(d) = o(G(d))$ means $F(d)/G(d) \to 0$ as $d \to \infty$.

% \subsection{Optimally-Robust Models at Given Level of Ordinary Risk}


% \subsection{Complexity Parameters}

\paragraph{Step 1: Proxy for Adversarial Risk.}
An analytic formula for the adversarial risk $E(w,r)$ for a linear model $w$ was analytically obtained in Lemma \ref{lm:analytic}. Direct analysis of adversarial risk via this formula is still difficult. A first step towards proving Theorem \ref{thm:lousy} is to obtain a proxy for $E(w,r)$ which is more amendable to analysis.  This is done in the following lemma.% first step is to obtain an analytic formula for the adversarial risk $E(w,r)$ of an any linear model $w \in \mathbb R^d$. 
% Recall that the adversarial risk functional $E$ defined in \eqref{eq:Ewr}.
%\begin{restatable}{rmk}{}
%Note that $E(w,r) \ge \max(E(w),r^2\|w\|_\star^2)$ for any model $w \in \mathbb R^d$. In particular, the adversarial risk of the generative model $w_0$ is $E(w_0,r) = r^2\|w_0\|_\star^2$ which grows quadratically with the attack strength $r$. More generally if $w \in \mathbb R^d$ is nonzero an independent of $r$, then $$
%E(w,r) \ge r^2\|w\|_\star^2 \ge r^2\|w\|_\star^2 = \Omega(r^2) \overset{r \to \infty}{\to} \infty.
% $$
% \end{restatable}
% It is well-known that the ordinary risk of any linear model $w \in \mathbb R^d$ is given by $E(w) = \|w-w_0\|_\Sigma^2 + \sigma^2$.

% \subsection{Optimal Adversarial Risk and Proxy}
% Let $E_{opt}(r)$ be the optimal adversarial risk achievable by a linear model, i.e
% \begin{equation}
%     E_{opt}(r) := \inf_{w \in\mathbb R^d} E(w,r).
% \end{equation}
% Clearly, one has $E_{opt}(r) \le \min(\|w_0\|_\Sigma^2,r^2 \|w_0\|_\star^2)$, as can be seen by evaluating $E(w,r)$ at $w=0$ and $w=w_\star$.
\begin{restatable}{lm}{sandwich}
\label{lm:sandwich}
For any $w \in \mathbb R^d$ and $r \ge 0$, it holds that
\begin{eqnarray}
    \alpha K(w,r)^2 \le E(w,r) \le K(w,r)^2,
\end{eqnarray}
where $K(w,r) := \sqrt{E(w)} + r\|w\|_\star$ and $\alpha := (1+\sqrt{2/\pi})/2 \approx 0.899$ is an absolute constant.
% Henceforth, whenever possible we will work with the latter in place of the former.
\end{restatable}
% Thus, the adversarial risk functional $w \mapsto E(w,r)$ is equal to the proxy $w \mapsto K(w,r)^2$, up to within multiplicative absolute constants, or more succinctly, $E(w,r) \asymp K(w,r)^2$. The former will turn out to be easier to analyze.

\paragraph{Step 2: Restricting the Search to a Chord.}
Even with the analytic formula for $E(w,r)$ given by Lemma \ref{lm:analytic}, computing $E_{opt}(r,\epsilon) := \inf_{w \in \mathcal W_\epsilon} E(w,r)$, which is the main object of study of this paper, remains untractable. Instead, we will restrict the optimization to a line / chord in $\mathcal W_\epsilon$, parallel to the generative model $w_0$. It will turn out that up to within multiplicative constants, this strategy gives the correct value of $E_{opt}(r,\epsilon)$ as a function of all relevant problem parameters. To this end, let $E_{shrink}(r,\epsilon)$ be the optimal adversarial risk achieved by a linear model which is co-linear with the generative model $w_0$, i.e
\begin{eqnarray}
E_{shrink}(r,\epsilon) := \inf_{w \in \mathcal W_\epsilon \cap \langle w_0\rangle}E(w,r),
\end{eqnarray}
where $\langle w_0\rangle := \{t w_0 \mid t \in \mathbb R\}$ is the one-dimensional subspace of $\mathbb R^d$ spanned by the generative model $w_0$.

\begin{restatable}{prop}{keyprop}
The following estimates hold
\label{prop:keyprop}
\begin{align}
 E_{opt}(r,\epsilon) &\ge \alpha E_{shrink}(r,\epsilon)\label{eq:lower}\\
E_{opt}(r,\epsilon) &\le \frac{1}{\alpha} E_{shrink}(\eta_0 r,\epsilon) \le \frac{\eta_0^2}{\alpha} E_{shrink}(r,\epsilon)\label{eq:upper},
\end{align}
where $\alpha := (1 + \sqrt{2/\pi})/2 \approx 0.899$.
\end{restatable}
This auxiliary result, which is the main component of the proof of Theorem \ref{thm:lousy}, is proved in the supplemental, with the help of Lemma \ref{lm:sandwich}.

\paragraph{Step 3: Computing the Value of $E_{shrink}(r,\epsilon)$.} To complete the proof of Theorem \ref{thm:lousy}, it remains to show that 
the proxy $E_{shrink}(r,\epsilon)$ equals $H(r/r_0,\epsilon)^2$ up to within multiplicative absolute constants. The proof of Theorem \ref{thm:lousy} would then follow upon plugging such estimates into the bounds given in Proposition \ref{prop:keyprop}.
\begin{restatable}{prop}{shrinky}
For any $r,\epsilon \ge 0$, it holds that 
\begin{eqnarray}
\dfrac{E_{shrink}(r,\epsilon)}{\|w_0\|_\Sigma^2 }  \asymp E(t_{opt}w_0,r) \asymp \widetilde\sigma^2 + H(\frac{r}{r_0},\epsilon)^2,
\end{eqnarray}
% i.e the optimal shrinkage parameter is given by 
where the function $H$ is as defined in \eqref{eq:H}, and $r_0$ is the scalar defined in \eqref{eq:rOeta0}, and $t_{opt}=T(r/r_0,\epsilon) \in [0,1]$ is the optimal%,\footnote{Optimal, up to within multiplicative absolute constants in the adversarial risk.},
and where the function $T$ is as defined in \eqref{eq:T}.
\label{prop:shrinky}
\end{restatable}
Comparing Propositions \ref{prop:keyprop} and \ref{prop:shrinky}, it becomes clear how the function $F$ and $T$ enter the bounds \eqref{eq:thighnflt} in Theorem \ref{thm:lousy}.

==> new.tex <==
\section{Structure of Optima: Proof of Propositon \ref{prop:lagrangian} and Theorem \ref{thm:ridge}}
\lagrangian*

\begin{proof}
For any $w \in \mathbb R^d$ and $r\ge 0$, define $\widetilde E(w,r) := \|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2$.
Note that $E(w,r) \asymp  \sigma^2 + \widetilde E(w,r)$, uniformly on all $w \in \mathbb R^d$ and $r \ge 0$.
Thus,
\begin{eqnarray*}
    \begin{split}
\inf_{w \in \mathcal W_\epsilon}\widetilde E(w,r) &= \min_{\|w-w_0\|_\Sigma \le \epsilon^2\|w_0\|_\Sigma^2} \|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2\\
&= \min_w \sup_{\lambda \ge 0} + \|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2) + \lambda(\|w-w_0\|_\Sigma^2-\epsilon^2\|w_0\|_\Sigma^2)\\
&=\sup_{\lambda \ge 0} \min_w  + \|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2) + \lambda(\|w-w_0\|_\Sigma^2-\epsilon^2\|w_0\|_\Sigma^2)\\
&= \min_w \sup_{\lambda \ge 0} + \|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2) + \lambda(\|w-w_0\|_\Sigma^2-\epsilon^2\|w_0\|_\Sigma^2)\\
&=\sup_{\lambda \ge 0} \min_w  + \|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2) + \lambda(\|w-w_0\|_\Sigma^2-\epsilon^2\|w_0\|_\Sigma^2)\\
&=\sup_{\lambda \ge 0} -\epsilon^2\|w_0\|_\Sigma^2 \lambda + \min_w  (1+\lambda)\|w-w_0\|_\Sigma^2 + r^2\|w\|_\star^2\\
& \asymp \sup_{\lambda \ge 0} -\epsilon^2\|w_0\|_\Sigma^2 \lambda + (1+\lambda)\newgamma(r(\lambda)),
    \end{split}
\end{eqnarray*}
and the first part of the claim follows.
Note that the swapping of the inf and sup in the above is justified by Lagrangian strong duality in the form of \emph{Slater's Theorem}. Indeed, the primal problem is convex and the constraint set $\mathcal W_\epsilon$ has non-empty interior (in fact, it contains $w_0$) as soon as $\epsilon$ is positive.

The second part follows from the first part and the fact that ...
\end{proof}

\section{Results for Euclidean-Norm Attack}
% \subsection{Proof of Theorem \ref{thm:ridge}}
%\ridge*

\subsection{Isotropic Features}
Now consider the case of isotropic features where $\lambda_k = 1$ for all $k \in [d]$. The auxiliary function $H$ then simplifies to
\begin{eqnarray}
H(t) = \|w_0\|_2^2((1+t)^{-1}-\epsilon^2t^{-1}).
\end{eqnarray}
Now, $H'(t) = -1/(1+t)^2 + \epsilon^2/t^2$, and so, $H(t) \ge 0$ iff $(1+t)^2\epsilon^2 \ge t^2$ iff $(1+t)\epsilon \ge t$ iff $t \le t_\star:= \epsilon/(1-\epsilon)$. Thus, $H$ is increasing on $[0,t_\star]$ and decreasing on $[t_\star,\infty)$.

Case 1: $t_\star(\epsilon) \le r^2$, i.e $\epsilon/(1-\epsilon) \le r^2$, i.e $\epsilon \le \epsilon_\star(r):=r^2/(1+r^2)$, then $H$ attains its max on $[0,r^2]$ at $t=t_\star(\epsilon)$.
\begin{eqnarray}
\begin{split}
E_{opt}(r,\epsilon) &\asymp \epsilon^2\|w_0\|_2^2 + r^2 H(t_\star(\epsilon)) = \epsilon^2\|w_0\|_2^2 + r^2\|w_0\|_2(1-\epsilon - (1-\epsilon)\epsilon)\\
&= \epsilon^2\|w_0\|_2^2 + \|w_0\|_2^2(1-\epsilon)^2r^2.
\end{split}
\end{eqnarray}

Case 2: $t_\star(\epsilon) \ge r^2$, i.e $\epsilon \ge \epsilon_\star(r)$. Then, $H$ attains it maximum on $[0,r^2]$ at $t=r^2$, and so
\begin{eqnarray}
\begin{split}
E_{opt}(r,\epsilon) \asymp \sigma^2 + \epsilon^2\|w_0\|_2^2 + r^2 H(r^2) = \sigma^2 + \frac{r^2}{1+r^2}\|w_0\|_2^2 = \sigma^2 + \epsilon_\star(r)\|w_0\|_\Sigma^2
\end{split}
\end{eqnarray}

We have thus proved the following result.
\begin{restatable}{thm}{}
Given an attack strength $r \ge 0$, define a threshold
\begin{eqnarray}
\epsilon_\star(r) := r^2/(1+r^2) \in [0,1].
\end{eqnarray}
For any $\epsilon \ge 0$, the following hold.

-- If $0 \le \epsilon \le \epsilon_\star(r)$,
then $E_{opt}(r,\epsilon) \asymp \sigma^2 + \sigma^2 + \epsilon^2\|w_0\|_2^2 + \|w_0\|_2^2(1-\epsilon)^2 r^2$.

-- If $\epsilon \ge \epsilon_\star(r)$, then $E_{opt}(r,\epsilon) \asymp \sigma^2 + \epsilon_\star(r)\|w_0\|_2^2$.
\end{restatable}

Thus, as soon as $r=\Omega(1)$, there $\epsilon_\star=\Omega(1)$ and a phase-transition occurs at $\epsilon=\epsilon_\star(r)$.
\lorem


==> nn.tex <==
\section{Main results for infinite-width neural networks}
\label{sec:nn}
We now turn to study of the robustness profile \eqref{eq:robprofile} of the inner-product kernels that arise in the infinite-width limit of neural networks in the RF and NTK regimes. We analyze this profile as a function of the activation function $\sigma$, and other relevant variables: aspect radio $\gamma=d/n$, SNR, etc. etc. The results we obtain in this section are important corollaries to Theorem \ref{thm:master}, specialized to neural networks.
Let $K_\sigma^\rf(x,x'):= h_\sigma^\rf(x^\top x')$ and $K_\sigma^\ntk(x,x') = h_\sigma^\ntk(x^\top x')$ be the associated inner-product kernels defined in \eqref{eq:hRF}.
% We will assume the following condition, which ensures that the kernels $K_\sigma^{\rf/\ntk}$ are indeed inner-product kernels.
% \begin{restatable}[Isotropic features]{cond}{}
% The distribution $P$ of the features is uniform on the sphere $\sphere(\sqrt{d})$.
% % of radius $\sqrt{d}$ in $\mathbb R^d$.
% \label{cond:sphericaldata}
% \end{restatable}
% The uniformity restriction can be relaxed by simply demanding that $P$ have a rotationally-invariant density w.r.t to the Lebesgue measure on $\mathbb R^d$.

\subsection{Implicit regularization of induced kernel functions}
We will need the following condition, which is verified for all activation functions used in practice. Similar regularity conditions were assumed in \cite{daniely2016} to study the capacity of neural nets in the infinite-width limit.
\begin{restatable}[Regularity of the activation function]{cond}{}
The activation function $\sigma$ is either
(A) thrice continuously-differentiable,
% with $\|\sigma'\|_\infty,\|\sigma''\|_\infty \le C$,
\textbf{OR} equal to one of the ReLU or absolute-value activation functions.
\label{cond:smoothsigma}
\end{restatable}
% Note that the above condition covers all popular activation functions used in practice. For example, activation functions satisfying Condition \ref{cond:smoothsigma} include (but are not limited to): tanh, sine, cosine, gaussian Erf, etc.
% Condition \ref{cond:smoothsigma} ensure that the induced inner-product kernel function $h_\sigma$ satisfies the smoothness requirement \ref{cond:smooth}. A  condition similar to Condition \ref{cond:smoothsigma}(A) has been introduced in \cite{daniely2016}, under the name of "$C$-smooth activation functions", and used to derive generalization bounds.

 \begin{table*}[h!]
   \begin{center}
       {\tabulinesep=1.2mm
     \begin{tabu}{|c|c|c|c|}
     \hline
    Activation function $\sigma$ & $c_1(\sigma)^2$ & RF kernel function $h^\rf_\sigma(t)$ & NTK function $h_\sigma^\ntk(t)$\\
     \hline
      Identity & $1$ & $t$ & $t$\\
      \hline
      ReLU & $1/4$ & $\frac{1}{2\pi}(t\arccos(-t) + \sqrt{1-t^2})$ & $\frac{1}{2\pi}t\arccos(-t)$ \\
      \hline
      PReLU & $(1+\alpha)^2/4$ & --  & --
      \\
      \hline
      Sign & $2$ & $(2/\pi)
      \arcsin(t)$ & NA\\
      % $\dfrac{t}{2\pi\sqrt{1-t^2}}$ & ...\\
      \hline
      Unit-step & $1/(2\pi)$ & $\arccos(-t)/(2\pi)$ & NA\\
      % $\dfrac{t}{2\pi\sqrt{1-t^2}}$ & ..\\
    %  \hline
    %  $\tanh(z)$ & 
    \hline
    Gaussian Erf & $4/(3\pi)$ & $(2/\pi)\arcsin(2t/3)$ & $\dfrac{4t}{\pi\sqrt{9-4t^2}}$ \\
    \hline
    Tanh & $0.605706$ & -- & -- \\
   \hline
    Soft-thresholding & $2(1-\Phi(\alpha))$ & -- & -- \\
     \hline
    %  % $\tanh(z) $ & ...\\
    %  \hline
     Quadratic & $b^2$ & $b^2t + c^2$ & $b^2t$\\
    \hline
    Sine & $1/e$ & $\sinh(t)/e$ & $ t\cosh(t)/e$\\
     \hline
    Cosine  & $0$ & $\cosh(t)/e$ & $t\sinh(t)/e$\\
     \hline
    %  % $a z^2 + c$ & $c^2$\\
    %  % \hline
    Absolute value & $0$ &  $2(t\arcsin(t) + \sqrt{1-t^2})/\pi$ & $(2/\pi)t\arcsin(t)$\\
    \hline
     \end{tabu}
     }
     \end{center}
     \caption{Summary of results for kernel methods induced by infinite-width two-layer neural networks in RF regime, for different activation functions $\sigma$. Also see \cite{inductivebietti,daniely2016} and \cite{couillet18} (especially Table 1 thereof). Note that the quadratic activation function is defined by $\sigma(z) := az^2 + bz + c$, for some $a,b,c \in \mathbb R$; the soft-shrinkage activation function is defined by $\sigma(z) := \mathrm{sign}(z)(|z|-\alpha)_+$, for some bandwidth parameter $\alpha \ge 0$; the unit-step activation function is defined by $\sigma(z) := \relu'(z) = 1[z \ge 0]$; the PRELU (Parametric ReLU) activation function is defined by $\sigma(z) := \max(z,\alpha z)$, for some $\alpha \in (-1,1)$.}
     \label{tab:hsigma}
\end{table*}

\subsection{Implicit regularization by the activation function}
\label{subsec:implicitregsigma}
Let us begin with the folllowing elementary lemma which is our first step towards a complete characterization of the robustness profile of (infinite-width) neural networks.
\begin{restatable}{lm}{smoothh}
Under Condition \ref{cond:smoothsigma}, the kernel functions $h_\sigma^{\rf}$ and $h_\sigma^\ntk$ defined in \eqref{eq:hRF} and \eqref{eq:KNTK} respectively, are twice continuously-differentiable on $(-1,1)$. Moreover, we have the identity
\begin{eqnarray}
(h_\sigma^\rf)'(0) = (h_\sigma^\ntk)'(0) = c_1(\sigma)^2 =:\theta_2(\sigma),
\end{eqnarray}

where $\theta_2(\sigma) \ge 0$ is as defined in \eqref{eq:theta2} and $c_1(\sigma)$ is the first order Hermite coefficient of $\sigma$.
\label{lm:smoothh}
\end{restatable}

In particular, we deduce that the implicit regularization induced by the activation function is
\begin{eqnarray}
\begin{split}
\lambda_{h_\sigma} := 
\begin{cases}
% h_\sigma^\rf(1) - h_\sigma^\rf(0) - (h_\sigma^\rf)'(0) =
\theta_1(\sigma)-\theta_0(\sigma)-\theta_2(\sigma) \ge 0,&\mbox{ for }\rf\\
% \lambda_{h_\sigma^\ntk} := h_\sigma^\ntk(1) - h_\sigma^\ntk(0) - (h_\sigma^\ntk)'(0) =
\theta_1(\sigma')-\theta_2(\sigma) \ge 0,&\mbox{ for }\ntk,
\end{cases}
\end{split}
\end{eqnarray}
where $\theta_1(\sigma) := c_0(\sigma^2)$, $\theta_0(\sigma) := c_0(\sigma)^2$, and $\theta_2(\sigma) := c_1(\sigma)^2$, with $c_k(\sigma)$ being the $k$th Hermite coefficient of $\sigma$.
% Note that the coefficients $\theta_0(\sigma)$, $\theta_1(\sigma)$, and $\theta_2(\sigma)$ have appeared in the theoretical literature on neural networks \cite{montanari2020,Mei2019,Ghorbani19,ascoli20,pennington17,pennington2017ressurect,peche19} as an essential ingredient that control the generalization in neural networks.
If $c_1(\sigma) \ne 0$, we also deduce that the $\alpha$ coefficient in Theorem \ref{thm:main} reduces to
\begin{eqnarray}
\begin{split}
    \alpha_{h_\sigma} := \frac{h_\sigma(0)}{h'_\sigma(0)} = \begin{cases}
    \theta_0(\sigma)/\theta_2(\sigma),&\mbox{ if }\rf,\\
    0,&\mbox{ if }\ntk
    \end{cases}
\end{split}
\end{eqnarray}



\subsection{A sharp separation between activation functions}
Note that we can always orthogonally decompose the activation function like so
\begin{eqnarray}
\sigma(z) = c_0(\sigma) + c_1(\sigma)z + \sigma^\perp(z),
\end{eqnarray}

with $c_1(\sigma^\perp) = c_0(\sigma^\perp) =  0$.
Since $(h_\sigma^{\rf/\ntk})'(0)=\theta_2(\sigma)$ thanks to Lemma \ref{lm:smoothh}, Theorem \ref{thm:master} predicts that the kind (i.e "universality class") of the robustness profile of the corresponding kernel $K_\sigma^{\rf/\ntk}$ is completely determined by whether $c_1(\sigma) = 0$ or not.
% \begin{itemize}
% \item[(A)] $\theta_2(\sigma)=0$, in which case $\sigma$ is said to be of \textbf{Type I} or \emph{covariance-aligned}.
% \item[(B)] $\theta_2(\sigma)>0$, in which case $\sigma$ is said to be of \textbf{Type II} or \emph{distortion-induced}.
% \end{itemize}
% % The above nomenclature was coined in
% \mytodo{Cite Couillet and students} and \cite{pennington17,peche19}. Covariance-oriented activation functions include: absolute-value, cosine, and exponential quadratic $z \mapsto e^{-z^2/2}$, and pure quadratic $z \mapsto az^2 + c$. The former leads to much more robust models than the latter. The remainder of the section explores this phenomenon.
% \subsubsection{Nonrobust activation functions}
The following corollary to Theorem \ref{thm:master} is one of our main contributions.
% \begin{mdframed}[backgroundcolor=cyan!10,rightline=false,leftline=false]
\begin{restatable}[Robustness profile for infinite-width neural nets in RF and NTK regimes]{cor}{nn}
Assume Condition
% \ref{cond:sphericaldata} and
\ref{cond:smoothsigma} is in order and consider kernel regression \eqref{eq:kridge} with kernel function $h_\sigma \in \{h^{\rf}_\sigma,h_\sigma^\ntk\}$ defined in \eqref{eq:hRF} and \eqref{eq:KNTK}. For large $n \asymp d$, it holds w.h.p over the training data $\mathcal D_n \equiv (X,y)$ that,
\begin{eqnarray}
\mathfrak{S}(\widehat{f}_{h_\sigma,\lambda})^2 = \begin{cases}
c^\top Q c /d + o_{n}(1),&\mbox{ if }c_1(\sigma) \ne 0,\\
o_{n}(1),&\mbox{ if }c_1(\sigma) =0.
\end{cases}
\end{eqnarray}
where $Q := XX^\top /d \in \mathbb R^{n \times n}$ and $c := (Q + \overline{\lambda}_{h_\sigma} I_n + \alpha_{h_\sigma}1_n1_n^\top)^{-1} y \in \mathbb R^n$.
% \begin{itemize}
% \item[--] \textbf{ReLU}, defined by $\sigma(z) := \max(z,0)$,
% \item[--] \textbf{Sign}, defined by $\sigma(z) := \mathrm{sign}(z)$,
% \item[--] \textbf{Positive}, defined by $\sigma(z) := 1[z \ge 0]$,
% \item[--] \textbf{Tanh}, defined by $\sigma(z) := \tanh(z)$,
% \item[--] \textbf{Sine}, defined by $\sigma(z) := \sin(z)$,
% \item[--] \textbf{Erf} (Gaussian error-function), defined by $\sigma(z) := (2/\sqrt{\pi})\int_0^z e^{-t^2}dt$.
% \end{itemize}
Moreover, if $\theta_2(\sigma) > 0$, then the conclusions of Theorem \ref{thm:master} hold with $h=h_\sigma$.

Finally, for data generated according to \eqref{eq:linearf}, the conclusions of Theorem \ref{thm:linearsignal} and Corollary \ref{cor:extremecases} 
\label{cor:extremecasesnn}
hold.% with $h=h_\sigma$.
\label{cor:nn}
\end{restatable}
% \end{mdframed}

\begin{proof}
Thanks to Lemma \ref{lm:smoothh}, the induced kernel functions $h_\sigma^{\rf}$ and $h_\sigma^\ntk$ are at least twice-differentiable with $(h_\sigma^{\rf/\ntk})'(0) = \overline{\sigma}'(0) = c_1(\sigma)^2$. The result then follows directly from Theorem \ref{thm:main}.
% The result then follows directly from Theorem \ref{thm:master}.
\end{proof}
% The above theorem provides a theoretical justification of the \emph{open space risk hypothesis} purported in \mytodo{Cite SPLASH and tent papers}.


% \subsubsection{Robustness profile of covariance-oriented activation functions}
% \begin{restatable}{lm}{}
% $h_\sigma'(0) = \theta_2(\sigma)$. In particular, if $\sigma$ is symmetric symmetric in a neighborhood of $0$, then $h'_\sigma(0) = 0$.
% \end{restatable}
% \begin{restatable}{lm}{}
% If $\sigma$ is left and right- differentiable at $0$, then
% \begin{eqnarray}
% h_\sigma'(0) = \frac{(\sigma(0^+)+\sigma(0^-))^2}{4}.
% \end{eqnarray}
% \end{restatable}
% For example, we deduce that $h_\sigma'(0) = (1+0)^2/4 = 1/4$ if $\sigma$ is the ReLU activation function, while $h_\sigma'(0) = (1-1)^2/4 = 0$ for the absolute-value (or in fact, any activation function which is locally symmetric around $0$).

% \lorem

% \lorem 

% \paragraph{Faster training and robustness from dynamical iso-spectrality.}
% % Define a scalars $\theta_0(\sigma)$, $\theta_1(\sigma)$, and $\theta_2(\sigma) \ge 0$ by
% % \begin{eqnarray}
% % \theta_0(\sigma)=(\mathbb E[\sigma(z)])^2,\,\theta_1(\sigma)=(\mathbb E[\sigma(z)^2]),\,\theta_2(\sigma) := (\mathbb E[z\sigma(z)])^2,
% % \end{eqnarray}
% % $z \sim N(0,1)$.
% In view of the above results, we see that there is a phase-transition in robustness between $\theta_2(\sigma)=0$ (e.g for absolute-value, cosine, etc. activation functions) and $\theta_2(\sigma)>0$ (e.g ReLU, tanh, Erf, etc., activation functions). This provides rigorous theoretical justification of the observations in \mytodo{Cite SPLASH and tent papers}.
% Also, in \cite{pennington2017ressurect,pennington17,peche19}, it was shown that the condition $\theta_2(\sigma)=0$ (combined with $\theta_0(\sigma)=0$) corresponds to activation function which don't modify the eigenvalue distribution of the empirical covariance matrix of the inputs as they go through layers in a feedforward neural network with activation functions $\sigma$. This property was advocated to favor faster training of such neural networks. As our results show, such activation functions also have \emph{Type I} robustness profile, i.e there are induce the most robust kernel methods.


==> oldpolynomial.tex <==
\subsection{Polynomial Decay}
\textcolor{red}{This subsection is outdated. Go to Section \ref{subsec:polynomial2} instead!}

Suppose the eigenvalues $(\lambda_k)_k$ and alignment coefficients $(c_k)_k$ satisfy following decay conditions
\begin{align}
\lambda_k &\asymp k^{-\beta},\text{ for some constant }\beta > 1,\\
c_k &= 1\,\forall k \in [d].% ,\text{ for some constant }\delta \in [0,1/2).
\end{align}

It is easy to see that for Euclidean-norm attack,
\begin{eqnarray}
    \begin{split}
        r_0 &= \|w_0\|_\Sigma / \|w_0\|_2 \asymp \sqrt{\mbox{tr}(\Sigma)}/\sqrt{d} \asymp 1/\sqrt d,\\
        r_1 &= \|\Sigma w_0\|_2 / \|w_0\|_\Sigma \asymp 1/\sqrt{\mbox{tr}(\Sigma)} \asymp 1,
    \end{split}
\end{eqnarray}
Thus, $r_0 \ll r_1$, and the bounds given by Theorem \ref{thm:lousy} can be expected to be completely off. It turns out that using a different technique, one can still get a respectable lower-bound.

We start with the following instrumental lemma.
\begin{restatable}{lm}{}
\label{lm:weiwainwright}
Consider Euclidean-norm attack with strength $r$ such that $r = o(1)$. Then,
\begin{eqnarray}
\gamma(r) \asymp s(r) := \min(r^{1-1/\beta},r\sqrt d).
\end{eqnarray}
\end{restatable}

The following result shows that there is no cross-over / phase-transition phenomenon in this polynomial decay regime.
\begin{restatable}{thm}{powerlaw}
\label{thm:powerlaw}
% Consider the power-law model above.
Consider Euclidean-norm attacks with strength $r \ge 0$ such that
\begin{eqnarray}
    r \to 0,\, rd^{\beta/2} \to \infty.
\end{eqnarray}
Define the thresholds
\begin{eqnarray}
    \epsilon_1 = \epsilon(d) := (1/\beta)d^{-(\beta-1)/2},\,\epsilon_2(r) := (1/\beta) r^{1-1/\beta}.
\end{eqnarray}
Then, for any the following holds:

-- \textbf{Very accurate models.} If $0 \le \epsilon \le \epsilon_1$, then $E_{opt}(r,\epsilon) \asymp \sigma^2+ r^2 d$.

-- \textbf{Intermediate regime.} If $\epsilon_1 \le \epsilon \le \epsilon_2$, then $E_{opt}(r,\epsilon) \asymp \sigma^2 + \epsilon^{-2/(\beta-1)} r^2 + \epsilon^2$.

-- \textbf{Uneventful regime.} If $\epsilon \ge \epsilon_2$, then $E_{opt}(r,\epsilon) \asymp  \sigma^2 + r^{2(1-1/\beta)}$
\end{restatable}
Since $\epsilon_1,\epsilon_2 = o(1)$, there is no cross over in this polynomial decay regime.

\appendix
\section{Proof of Theorem \ref{thm:powerlaw}}
\powerlaw*
\begin{proof}
First note that $\|w_0\|_\Sigma^2 \asymp \mbox{tr}(\Sigma) \asymp \sum_{k \ge 1}k^{-\beta} = \zeta(\beta) = \Theta(1)$.
    Also, we know from Lemma \ref{lm:weiwainwright} that if $d^{-\beta/2} \le t = o(1)$, then 
    \begin{eqnarray}
    \label{eq:clue}
\gamma(t) \asymp s(t):=t^{1-1/\beta}.    
    \end{eqnarray}
    
    \paragraph{Step 1: Simplification.}
    By Proposition \ref{prop:oracleexact}, $E_{opt}(r,\epsilon) \asymp \sigma^2 + h(r,\epsilon)^2$, with
\begin{eqnarray*}
\begin{split}
    h(r,\epsilon) &:= \sup_{\lambda \ge 0}(1+\lambda)\gamma\left(\frac{r}{1+\lambda}\right)-\lambda\epsilon\|w_0\|_\Sigma \\
    &\asymp \sup_{ \lambda \ge 0}m(r),
    \end{split}
\end{eqnarray*}
where $m(\lambda) := (1+\lambda)s(r/(1+\lambda))-\lambda\epsilon$, where $s(t):=\min(t^{1-1/\beta},t\sqrt d)$. In the second line, we have applied \eqref{eq:clue} with $t = r(\lambda):=r/(1+\lambda)$.

\textbf{Case 1: $r(\lambda) \ge d^{-\beta/2}$.} This is equivalent to $0 \le \lambda \le rd^{\beta/2}-1$. This is only possible if $r \ge d^{-\beta/2}$. Then, $s(r(\lambda)) = t\sqrt d$, and so
\begin{eqnarray}
    \sup_{\lambda \ge 0,\, r(\lambda) \le d^{-\beta/2}} r\sqrt d - \epsilon\lambda = r\sqrt d + \sup_{\lambda \ge rd^{\beta/2}-1}  - \epsilon\lambda = r\sqrt d - (rd^{\beta/2}-1)\epsilon = (\sqrt d - \epsilon d^{\beta/2})r + \epsilon.
\end{eqnarray}

\paragraph{Step 2: Optimization.}
Now, derivative is $m'(\lambda) = \dfrac{s(r)}{\beta}\dfrac{1}{(1+\lambda)^{1-1/\beta}}-\epsilon$, which is positive on $[0,\lambda_\star]$ and negative on $[\lambda_\star,\infty)$, where \begin{eqnarray}
\lambda_\star := \left(\dfrac{s(r)}{\beta\epsilon}\right)^{\beta/(\beta-1)}-1 = \dfrac{r}{(\beta\epsilon)^{\beta/(\beta-1)}}-1 = r/r_\star-1.   
\end{eqnarray}
\begin{itemize}
\item If $\lambda_\star <  0$, i.e if $\epsilon \ge (1/\beta)r^{1-1/\beta}$, then the supremum of $m$ on $[0,\infty)$ is attained at $0$ and we deduce that
\begin{eqnarray}
h(r,\epsilon) \gtrsim m(0) = s(r) = r^{1-1/\beta}.
\end{eqnarray}
This lower-bound is trivial because the RHS is $E_{opt}(r)=E_{opt}(r,1)$, which as we know is an unconditional lower-bound for $E_{opt}(r,\epsilon)$, thanks to ...

\item If $0 \le \lambda_\star \le rd^{\beta/2} - 1$, i.e if otherwise $(1/\beta)d^{-(\beta-1)/2} \le \epsilon \le (1/\beta)r^{1-1/\beta}$, then $m$ attains its supremum of $[0,\infty)$ and $\lambda_\star$. Thus,
\begin{eqnarray}
\begin{split}
h(r,\epsilon) &\asymp m(\lambda_\star) = s(r) \dfrac{r^{1/\beta}}{(\beta\epsilon)^{1/(\beta-1)}} - \left(\dfrac{r}{(\beta\epsilon)^{\beta/(\beta-1)}} - 1\right)\epsilon\\
&= \frac{r}{(b\epsilon)^{1/(\beta-1)}} - \frac{r}{(\beta\epsilon)^{\beta/(\beta-1)}} + \epsilon \asymp r\epsilon^{-1/(\beta-1)} + \epsilon
\end{split}
\end{eqnarray}
\item Finally, if $0 \le \epsilon \le (1/\beta)d^{-(\beta-1)/2}$, then $\lambda_\star \ge rd^{\beta/2}-1$, and so
\begin{eqnarray}
\begin{split}
    h(r,\epsilon) &\asymp m(rd^{\beta/2}-1) = r\sqrt d - (rd^{\beta/2}-1)\epsilon = (1-\epsilon d^{(\beta-1)/2})r\sqrt d + \epsilon\\
    &\gtrsim (1-1/\beta)r \sqrt d \asymp r\sqrt d.
    \end{split}
\end{eqnarray}
\end{itemize}

Combining with Proposition \ref{prop:oracleexact} completes the proof.
\end{proof}


==> overfitting.tex <==

\section{Tradeoffs Due to Overfitting}
Consider the case of isotropic features $\Sigma=I_d$. We restrict our considerations to Euclidean-norm attacks. To further easy our analysis, we suppose the generative model $w_0$ is drawn from $N(0,\alpha^2 I_d)$ independently from the design matrix $X = (x_1,\ldots,x_n) \in \mathbb R^{n \times d}$. Thus, the training data is as follows
\begin{align}
w_0 &\sim N(0,\alpha^2 I_d),\\
x_1,\ldots,x_n &\overset{iid}{\sim}N(0,I_d) \perp w_0,\\
z_1,\ldots,z_n &\overset{iid}{\sim} N(0,\sigma^2) \perp w_0,x_1,\ldots,x_n.
\end{align}

Let $\widehat\Sigma_n := X^\top X/n \in \mathbb R^{d \times d}$ be the empirical covariance matrix of the features. With abuse of notaiton, let $y=(y_1,\ldots,y_n) \in \mathbb R^n$ be the response vector, and let $z=(z_1,\ldots,z_n) \in \mathbb R^n$ be the noise vector, so that $y = Xw + z$. Let $\widehat{\mathcal W}_{\epsilon,n}$ be the set of models with training error at most $\epsilon^2\|w_0\|_2^2$, i.e
\begin{eqnarray}
    \widehat{\mathcal W}_{\epsilon,n} = \{w \in \mathbb R^d \mid (1/n)\|Xw-y\|_2 \le \epsilon^2\|w_0\|_\Sigma^2\}.
\end{eqnarray}
We are interested in computing
\begin{eqnarray}
    \widehat E_{opt}(r,\epsilon) := \inf_{w \in \widehat{\mathcal W}_\epsilon} E(w,r).
\end{eqnarray}
We place ourselves in the so-called proportionate scaling regime where the sample size $n$ and input-dimension $d$ tend to $\infty$ at the same rate, i.e
\begin{eqnarray}
    \label{eq:proportionate}
    n,d \to \infty, n/d \to \gamma \in (0,\infty).
\end{eqnarray}
Let $\mu_\gamma$ be the Marchenko-Pastur density with shape parameter $\gamma$ and let $m_\gamma$ be it Stieltjes transform defined by
\begin{eqnarray}
    m_\gamma(t) := \int \frac{1}{s+t}\mbox{d}\mu_\gamma(s).
\end{eqnarray}

Playing the Lagrangian strong duality trick once again as in Section \ref{sec:lagrangian}, we can show
\begin{eqnarray}
    \widehat E_{opt}(r,\epsilon) \asymp E(\widehat w_n(\widehat \mu_n(r,\epsilon)),r),
\end{eqnarray}
where $\widehat \mu_n(r,\epsilon) \ge 0$ is "optimal dual variable" and $\widehat w_n(\mu)$ is the unique minimizer of the function $w \mapsto K(w,r) + \mu\|Xw-y\|_2^2/n$. Now, setting derivatives to zero, we obtain that for any $\mu \ge 0$, the vector $w=\widehat w_n(\mu)$ must satisfy
$$
0 = w-w_0 + r^2w + \mu X^\top (Xw-y) = (\mu \widehat\Sigma + (1+r^2)I_d)w - (I_d + \mu \widehat\Sigma )w_0 - \mu X^\top z/n,
$$
that is
\begin{eqnarray}
    \widehat w_n(\mu) = (\mu \widehat\Sigma_n + (1+r^2)I_d)^{-1}((I_d + \mu \widehat\Sigma_n)w_0 + \mu X^\top z/n).
\end{eqnarray}
Now, define
\begin{eqnarray}
    \widehat F_n(\mu) := \mathbb E \left[\|\widehat w_n(\mu)-w_0\|_2^2 \mid X \right].
\end{eqnarray}
Noting that $w_0$ and $z$ are independent, a simple computation gives,
\begin{eqnarray*}
\begin{split}
\|\widehat w_n(\mu)-w_0\|_2^2 &= r^2 \mathbb E_{w_0} \|(\mu\widehat\Sigma_n + (1+r)^2I_d)^{-1}w_0\|_2^2 + \mathbb E_{z}\|(\mu\widehat\Sigma_n + (1+r)^2I_d)^{-1}X^\top z/n\|^2\\
&= \frac{\alpha^2}{d} r^2\mbox{tr}((\mu\widehat\Sigma_n + (1+r)^2I_d)^{-2}) + \frac{\sigma^2}{n}\mbox{tr}(\widehat\Sigma_n(\mu\widehat\Sigma_n + (1+r)^2I_d)^{-2})\\
&= \frac{\alpha^2}{d} \frac{r^2}{\mu^2}\mbox{tr}((\widehat\Sigma_n + t(\mu)^2 I_d)^{-2}) + \frac{\sigma^2}{n\mu^2}\mbox{tr}(\widehat\Sigma_n(\widehat\Sigma_n + t(\mu)^2 I_d)^{-2}),\text{ with }t(\mu) := \frac{r}{\sqrt{\mu + 1}}\\
&\overset{p}{\to}  \frac{\alpha^2 r^2}{\mu^2}\int_0^\infty \frac{1}{(s+t(\mu))^2}\mbox{d}\mu_\gamma(s) + \frac{\sigma^2}{\mu^2}\int_0^\infty \frac{s}{(s+t(\mu))^2}\mbox{d}\mu_\gamma(s),\text{ by MP theory}\\
&= \frac{\sigma^2}{\mu^2}\int_0^\infty \frac{s + r^2\mbox{SNR}}{(s+t(\mu))^2}\mbox{d}\mu_\gamma(s) = \frac{\sigma^2}{\mu^2}(m_\gamma(-t(\mu)^2) + (r^2\mbox{SNR}-t(\mu)^2)m'_\gamma(-t(\mu)^2)).
\end{split}
\end{eqnarray*}

==> proofs.tex <==
\input{new.tex}

\section{Some Spectral Results}
Recall that $\Sigma = \sum_k \lambda_k \phi_k\phi_k^\top$ is the SVD of the feature covariance matrix $\Sigma$ and $c_k = \phi_k^\top w_0$ is the $k$th aligmnent coefficient of the generative model $w_0$, so that $w_0 = \sum_k c_k \phi_k$.

\subsection{Support Function of Intersection of Ellipsoid and Euclidean Ball}
We will need the lemma for some of proofs.
\begin{restatable}{lm}{}
\label{lm:gaussianwidth}
For any $r \ge 0$, it holds that
\begin{eqnarray}
\sum_k \min(r^2,\lambda_k) c_k^2 \le \gamma(r)^2 \le 2\sum_k \min(r^2,\lambda_k)^2 c_k^2.
\end{eqnarray}
\end{restatable}
\begin{proof}
    Note that $\gamma(r) = \sup_{z \in E \cap rB_2^d}z^\top c$, where $E := \{z \in \mathbb R^d \mid \sum_k z_k^2/\lambda_k \le 1\}$ and $c=(c_1,\ldots,c_d)$. To prove the result, it then suffices to show that
    \begin{eqnarray}
    A(r) \subseteq E \cap rB_2^d \subseteq \sqrt{2} A(r),
    \end{eqnarray}
    where $rB_2^d$ is the unit-ball of radius $r$ in $\mathbb R^d$, and $A(r) := \{z \in \mathbb R^d \mid \sum_k z_k^2/\min(r^2,\lambda_k) \le 1\}$. If $z \in A(r)$, then $\sum_k z_k^2/\min(r^2,\lambda_k) \le 1$, and so
    \begin{itemize}
        \item  $\sum_k z_k^2/r^2 \le 1$, i.e $z \in rB_2^d$, and
        \item $\sum_k z^k/\lambda_k \le 1$, i.e $z \in E$,
    \end{itemize}
    i.e, $x \in E \cap rB_2^d$.
Conversely, if $x \in E \cap rB_2^d$, then
    $$
    \sum_k z_k^2/\min(r^2,\lambda_k) = \sum_k z_k^2\max(1/r^2,1/\lambda_k) \le \sum_k z_k^2/r^2 + \sum_k z_k^2/\lambda_k \le 1 + 2 = 2,
    $$
    i.e $x \in \sqrt 2 A(r)$.

The result then follows upon noting that $\sup_{z \in A(r)}z^\top c = \sqrt{\sum_k \min(r^2,\lambda_k)}$.
\end{proof}

\subsection{Effective Dimension Induced by Polynomial Spectral Decay}
We will need the following lemma.
\begin{restatable}{lm}{}
\label{lm:kstar}
 If $\lambda_k \asymp k^{-\beta}$ and $c_k^2 \asymp k^{-\delta}$ for all $k \in [d]$ and for some $\beta \in (1,\infty)$ and $\delta \in [0,1)$, then we have the following estimate
\begin{eqnarray}
\sum_k \frac{\lambda_k}{\lambda_k + t} \asymp \min(t^{-(1-\delta)/\beta},d^{1-\delta}),\text{ for }t = o(1).
\end{eqnarray}
\end{restatable}
\begin{proof}
    Let $k_\star = k_\star(t) \in [d]$ be the largest $k \in [d]$ such that $\lambda_k \ge t$. Then, $k_\star$ is the min of $d$ and floor of $t^{-1/\beta}$. Moreover, $t^{-1/\beta}$ if of same order as its floor since since $t^{-1/\beta} = \omega(1)$ because $t=o(1)$. We deduce that  $k_\star \asymp \min(t^{-1/\beta},d)$. Thus,
    \begin{eqnarray}
    \label{eq:base}
        \sum_k \frac{\lambda_k c_k^2}{\lambda_k + t} \asymp \sum_{k=1}^{k_\star}c_k^2 + \frac{1}{t}\sum_{k=k_\star+1}^d \lambda_k c_k^2.
    \end{eqnarray}
Now, the first sum in \eqref{eq:base} evaluates to
\begin{eqnarray}
 \sum_{k=1}^{k_\star}c_k^2 \asymp \int_1^{k_\star} z^{-\delta}\mathrm{d}z \asymp k_\star^{1-\delta} = k_\star^{1-\delta} \asymp \min(t^{-1/\beta},d)^{1-\delta} \asymp \min(t^{-(1-\delta)/\beta},d^{1-\delta}).
\end{eqnarray}
Analogously, we can show that the second sum in \eqref{eq:base} evaluates to  the same thing, thus completing the proof.
\end{proof}

\section{Proof of Proposition \ref{prop:gammaoracle}}
\gammaoracle*
\begin{proof}
    Indeed, thanks to Lemma xyz of Scetbon and Dohmatob (AISTATS 2023) and using the method of Lagrange multipliers to remove the constraint, one computes
\begin{eqnarray*}
\begin{split}
\sqrt{E_{opt}(r,\epsilon)} \asymp \inf_{w \in \mathcal W_\epsilon} K(w,r) &= \inf_{\|w-w_0\|_\Sigma \le \epsilon\|w_0\|_\Sigma} \sqrt{\|w-w_0\|_\Sigma^2 + \sigma^2} + r\|w\|_\star\\
&\asymp \sigma+\inf_{\|w-w_0\|_\Sigma \le \epsilon\|w_0\|_\Sigma} \|w-w_0\|_\Sigma + r\|w\|_\star\\
&= \sigma + \inf_w \sup_{\lambda \ge 0} \|w-w_0\|_\Sigma + r\|w\|_\star + \lambda(\|w-w_0\|_\Sigma - \epsilon\|w_0\|_\Sigma)\\
&= \sigma + \sup_{\lambda \ge 0}\inf_w \|w-w_0\|_\Sigma + r\|w\|_\star + \lambda(\|w-w_0\|_\Sigma - \epsilon\|w_0\|_\Sigma)\\
&= \sigma + \sup_{\lambda \ge 0}-\lambda\epsilon\|w_0\|_\Sigma + \inf_w (1+\lambda)\|w-w_0\|_\Sigma + r\|w\|_\star\\
&= \sigma + \sup_{\lambda \ge 0}-\lambda\epsilon\|w_0\|_\Sigma + (1+\lambda)\inf_w \|w-w_0\|_\Sigma + \frac{r}{1+\lambda}\|w\|_\star \\
&=  \sigma + \sup_{\lambda \ge 0}-\lambda\epsilon\|w_0\|_\Sigma + (1+\lambda)\gamma(\frac{r}{1+\lambda}),
\end{split}
\end{eqnarray*}
as claimed. Note that in the 4th line, we have used \emph{Lagrangian Strong Duality} (in the form of \emph{Slater's Theorem}) to swap the sup and inf operations. This is allowed because (1) the problem is convex, and (2) there exists a strictly feasible primal point, namely $w_0$ because $\epsilon > 0$ and so $\epsilon\|w_0\|_\Sigma > 0 = \|w_0-w_0\|_\Sigma$.
\end{proof}

\section{Proof of Theorem \ref{thm:lousy}}
\lousy*
\begin{proof}
Thanks Proposition \ref{prop:gammaoracle} and the second part of Lemma \ref{lm:gamma}, one has
\begin{eqnarray}
\label{eq:sugar}
\widetilde\sigma^2 + h_0(r/r_1,\epsilon)^2 \lesssim \frac{E_{opt}(r,\epsilon)}{\|w_0\|_\Sigma^2} \lesssim \widetilde\sigma^2 + h_0(r/r_0,\epsilon)^2,
\end{eqnarray}
where the function $h_0:\mathbb R_+^2 \to \mathbb R_+$ is defined by
\begin{eqnarray}
    \begin{split}
  h_0(c,\epsilon):=\sup_{\lambda \ge 0}-\lambda\epsilon + (1+\lambda)\min(1,\frac{c}{1+\lambda}) = \max(h_-(c,\epsilon),h_+(c,\epsilon)),
    \end{split}
\end{eqnarray}
where
\begin{eqnarray}
\begin{split}
h_-(c,\epsilon) &:= \sup_{0 \le \lambda c-1}m(\lambda),\\
h_+(c,\epsilon) &:= \sup_{\lambda \ge (c-1)_+}m(\lambda),\\
m(\lambda) &:= -\lambda\epsilon + (1+\lambda)\min(1,r/(1+\lambda)).
\end{split}
\end{eqnarray}
Now, observe that
\begin{eqnarray}
\begin{split}
    h_+(c,\epsilon) &:= \sup_{\lambda \ge (c-1)_+}-\lambda\epsilon + c = c - (c-1)_+\epsilon\\
    &= \begin{cases}
    c,&\mbox{ if }c \le 1,\\
    (1-\epsilon)c + \epsilon,&\mbox{ else.}
    \end{cases}
    \end{split}
\end{eqnarray}

On the other hand, if $c \le 1$, then $h_-(c,\epsilon)=-\infty$. Otherwise (i.e if $c \ge 1$), then one computes
\begin{eqnarray}
\begin{split}
h_-(c,\epsilon) &= \sup_{0 \le \lambda \le c-1}-\lambda\epsilon + 1+\lambda = 1 + \sup_{0 \le \lambda \le c-1} (1-\epsilon)\lambda\\
&= 1+(1-\epsilon)(c-1) = (1-\epsilon)c+\epsilon.
\end{split}
\end{eqnarray}
We conclude that for all $c\ge 0$ and $\epsilon \in [0,1]$,
\begin{eqnarray}
    h_0(c,\epsilon) = h_+(c,\epsilon) = \begin{cases}
    c,&\mbox{ if }c \le 1,\\
    (1-\epsilon)c + \epsilon,&\mbox{ else.}
    \end{cases}
\end{eqnarray}
Combining with \eqref{eq:sugar} and rearranging gives the first part of the theorem. The second part follows directly from the first.
\end{proof}

\subsection{Proof of Theorem \ref{thm:weakstrong}}
\weakstrong*

\begin{proof}
Note that $h(r,\epsilon) = \sup_{\lambda \ge 0}m(\lambda)$, where
$$
m(\lambda):=(1+\lambda)\gamma(r(\lambda))-\lambda\epsilon\|w_0\|_\Sigma \asymp \min(1+\lambda,r)u + \min((1+\lambda)b,r)v - R\epsilon\lambda.
$$
Note that we have used Lemma \ref{lm:gaussianwidth} and the fact that $r(\lambda)\le r$ for all $\lambda \ge 0$.

To compute the optimum value of $m$ over the interval $[0,\infty)$, we consider different cases according to the values of $r(\lambda)$.

\textbf{Case 1: $0 \le r(\lambda) \le b$.} This is equivalently to $\lambda \ge (r/b-1)_+$. Here, $m(\lambda) \asymp (u+v)r - R\epsilon\lambda$ and so
\begin{eqnarray}
\begin{split}
    \sup_{0 \le r(\lambda) \le b}m(\lambda) &\asymp \sup_{\lambda \ge (r/b-1)_+} (u+v)r-R\epsilon\lambda = (u+v)r-R\epsilon(r/b-1)_+\\
    &=: h_1(r,\epsilon).
    \end{split}
\end{eqnarray}

\textbf{Case 2: $b \le r(\lambda) \le 1$.} This is equivalent to, $(r-1)_+ \le \lambda \le r/b-1$, which is only possible if $r \ge b$. Here, $m(\lambda) = ur + vb + (vb - R\epsilon)\lambda $ and so
\begin{eqnarray}
\begin{split}
    \sup_{\lambda \ge 0,\,b \le r(\lambda) \le 1}m(\lambda) &\asymp ur + vb + \sup_{ (r-1)_+ \le \lambda \le r/b-1} (vb-R\epsilon)\lambda\\
    &= ur + vb + (vb-R\epsilon)\cdot \begin{cases}
    r/b-1,&\mbox{ if }\epsilon \le vb/R,\\
    (r-1)_+,&\mbox{ else}
    \end{cases}\\
    &:= h_2(r,\epsilon).
    \end{split}
\end{eqnarray}

\textbf{Case 3: $r(\lambda) \ge 1$.} This is equivalent to $0 \le \lambda \le r-1$, which is only possible if $r \ge 1$. Here,  $m(\lambda) \asymp ua+vb + (u+vb - R\epsilon)\lambda$, and so
\begin{eqnarray}
\begin{split}
    \sup_{\lambda \ge 0,\,r(\lambda) \ge 1}m(\lambda) &\asymp u + vb + \sup_{0 \le \lambda \le r-1} (u+vb - R\epsilon)\lambda\\
    &= u + vb + (u+vb - R\epsilon)_+(r-1)\\
    &=: h_3(r,\epsilon).
    \end{split}
\end{eqnarray}

Putting things together, we obtain the following
\begin{eqnarray}
   h(r,\epsilon) \asymp \begin{cases}
    h_1(r,\epsilon) = (u+v)r - R\epsilon(r/b-1)_+ = (u+v)r,&\mbox{ if }0 \le r \le b,\\
    \max(h_1(r,\epsilon),h_2(r,\epsilon)),&\mbox{ if }b \le r \le 1,\\
    h_3(r,\epsilon) = u+vb+(u+vb-R\epsilon)_+ (r-1),&\mbox{ if }r \ge 1.
    \end{cases}
\end{eqnarray}

We now prove the first part of the result. If $0 \le \epsilon \le vb/R$, it is easy to check that
\begin{eqnarray}
    \begin{split}
h_2(r,\epsilon)-h_1(r,\epsilon) &= v(b-r)+vb(r/b-1) = v(b-r) + vr -vb=0,\\
u+vb-R\epsilon &\ge u+vb-vb = u \ge 0.
    \end{split}
\end{eqnarray}
Moreover, $h_1(r,\epsilon) = (u+v-R\epsilon/b)r+R\epsilon$ and $h_3(r,\epsilon) = (u+vb-R\epsilon)r$, for such values of $\epsilon$.

For the second part, if $vb/R \le \epsilon \le vb/R + u/R$, then
\begin{eqnarray*}
    \begin{split}
h_2 &= ur + vb,\\
h_2(r,\epsilon) - h_1(r,\epsilon) &= v(b-r) + R\epsilon(r/b-1)\\
&\ge v(b-r) + vb(r/b-1)\\
&= v(b-r) + vr - vb = 0,\text{ for }b \le r \le 1\\
h_3(r,\epsilon) &= u + vb,
    \end{split}
\end{eqnarray*}
and so
\begin{eqnarray*}
\begin{split}
    h(r,\epsilon) &\asymp \begin{cases}
        (u+v)r,&\mbox{ if }0 \le r \le b,\\
        ur+vb,&\mbox{ if }b \le r \le 1,\\
        u+vb,&\mbox{ if }r \ge 1.
    \end{cases}\\
    &= \min(1,r)u + \min(b,r)v\\
    &\asymp \gamma(r).
\end{split} 
\end{eqnarray*}
To complete the proof, note that if $\epsilon \ge vb/R+u/R$, then
$\gamma(r) \le h(r,\epsilon) \le h(\epsilon,vb/R+u/R) \asymp \gamma(r)$. We conclude that $h(r,\epsilon) \asymp \gamma(r)$ for all $\epsilon \ge vb/R$ as claimed. This completes the proof.
\end{proof}



\section{Proof of Theorem \ref{thm:powerlaw}}
\powerlaw*

We will need the following proposition.
Exploiting the above estimate, we can establish the following result.
\begin{restatable}{prop}{hydra}
\label{prop:hydra}
Let $r,\epsilon \ge 0$ and define scalars $a_1,a_2,a_3,a_4,a_5,a_6 \ge 0$ by
\begin{eqnarray}
\begin{split}
   \beta &:= \beta/(1-\delta),\, a_1 := d^{1-\delta},\,a_2 := \epsilon^2,\,a_3 := r^2,\,a_4 := a_1^{-\beta},\\
   a_5 &:= (\beta a_2)^{\beta/(\beta-1)},\,
    a_6 :=\min(\max(a_5,a_4),a_3).
    \end{split}
\end{eqnarray}
Then, we have
\begin{eqnarray}
    E_{opt}(r,\epsilon) \asymp \sigma^2 + \epsilon^2 + r^2 \cdot \max(g_1(a_4),g_2(a_6)),
\end{eqnarray}
where $g_1(t):=a_1 - a_2/t$ and $g_2(t) := t^{-1/\beta}-a_2/t$.
\end{restatable}

For the proof of the proposition, we make use of the following lemma.
\begin{restatable}{lm}{}
\label{lm:hydra}
Let $\beta > 1$, $a_1,a_2,a_3 \ge 0$ be fixed, and consider the function $g(t) := \min(t^{-1/\beta},a_1)-a_2/t$. Then,
\begin{eqnarray}
\sup_{0 \le t \le a_3}g(t) = \max(g_1(a_4),g_2(a_6)),
\end{eqnarray}
where $a_4 := a_1^{-\beta}$, $a_5 := (\beta a_2)^{\beta/(\beta-1)}$, $a_6:=\mathrm{clip}(a_5,[a_4,a_3]) = \min(\max(a_5,a_4),a_3)$, and the functions $g_{1,2}$ are defined by $g_1(t) := a_1-a_2/t$, $g_2(t) := t^{-1/\beta}-a_2/t$.
\end{restatable}

\begin{proof}
We split the domain of optimization $[0,a_3]$ like so:

-- $t^{-1/\beta} \ge a_1$, $0 \le x \le a_4:=a_1^{-\beta}$,

-- $t^{-1/\beta} \le a_1$, i.e $t \ge a_4$.

There are multiple cases to consider.

\textbf{Case 1: $a_4 \le a_3$.} Then $g(t) \equiv g_1(t)$ on $[0,a_4]$ and $g(t) \equiv g_2(t)$ on $[a_4,a_3]$. Let $m_1$ be the sup of $g_1$ on $[0,a_4]$ and let $m_2$ be the sup of $g_2$ on $[a_4,a_3]$. It is clear that $m_1=g_1(a_4)$. On the other hand,
$$
g_2'(t) = -(1/\beta)1/t^{1+1/\beta}+a_2/t^2 \ge 0\iff a_2/t^{1-1/\beta} \ge 1/\beta \iff t \le a_5:=(\beta a_2)^{\beta/(\beta-1)}.
$$
Now,
\begin{itemize}
\item If $a_5 \le a_4$, then $m_2=g_2(a_4)$.
    \item If $a_4 \le a_5 \le a_3$, then $m_2=g_2(a_5)$.
    \item If $a_5 \ge a_3$, then $m_2 = g_2(a_3)$.
\end{itemize}
That is, $m_2 = g_2(a_6)$, where $a_6:=\mathrm{clip}(a_5,[a_4,a_3]) = \min(\max(a_5,a_4),a_3)$.

\textbf{Case 2: $a_4 \ge a_3$.} Here $g=g_1$ on all of the optimization domain $[0,a_3]$, and so $m=m_1$.

We conclude that $\sup_{0 \le t \le a_3}g(t)=\max(g_1(a_4),g_2(a_6))$
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop:hydra}]
Let $H$ be the scalar function appearing in Proposition \ref{prop:lagrangian}.
For the polynomially decaying spectrum, we have
\begin{eqnarray}
H(t) = \min(t^{-1/\beta},d) - \frac{\epsilon^2\|w_0\|_2^2}{t} \asymp \min(t^{-1/\beta},d) - \frac{\epsilon^2}{t},\text{ for }t=o(1).
\end{eqnarray}
where the last step is thanks to Lemma \ref{lm:kstar} applied with $\delta=0$, and the fact that
$$
\|w_0\|_\Sigma^2 = \sum_k \lambda_k c_k^2 = \sum_k k^{-\beta} = \zeta(\beta) = \Theta(1).
$$
The proof then follows from Proposition \ref{prop:lagrangian} and Lemma \ref{lm:hydra}.
\end{proof}

We are now ready to proof Theorem \ref{thm:powerlaw}.
\begin{proof}[Proof of Theorem \ref{thm:powerlaw}]
Recall the notation from Proposition \ref{prop:hydra}. First note that $g_1(a_4) = d-\epsilon^2d^{\beta}$.

-- \textbf{Case 1: $0 \le \epsilon^2 \le \epsilon_1^2 := (1/\beta)d^{-(\beta-1)}$.} Here, one easily computes
$$
a_6 = \min(d^{-\beta},r^2) = d^{-\beta},\,g_2(a_6) = d-\epsilon^2d^{\beta} = g_1(a_4) \ge (1-1/\beta)d \asymp d,
$$
and so $E_{opt}(r,\epsilon) \asymp \sigma^2 + \epsilon^2 + (d-\epsilon^2 d^{\beta})r^2 \asymp \sigma^2 + \epsilon^2 + (\beta-\epsilon^2/\epsilon_1^2)r^2 d \gtrsim \sigma^2 + r^2 d$.

-- \textbf{Case 2: $\epsilon_1^2 \le \epsilon^2 \le \epsilon_2^2 := \epsilon_\star := (1/\beta)r^{2(1-1/\beta)}$.} Here, we have $g_1(a_4) = d-\epsilon^2 d^{\beta} \le (1-1/\beta)d$, $a_6 = a_5 = (\beta\epsilon^2)^{\beta/(\beta-1)}$, and
\begin{eqnarray}
\begin{split}
g_2(a_6) &= (\beta\epsilon^2)^{-1/(\beta-1)} - \epsilon^2\cdot(\beta\epsilon^2)^{-\beta/(\beta-1)}\\
&= (1-1/\beta)(\beta\epsilon^2)^{-1/(\beta-1)} \ge (1-1/\beta)d.
\end{split}
\end{eqnarray}
Therefore, $\max(g_1(a_4),g_2(a_6)) = g_2(a_6) = (1-1/\beta)(\beta\epsilon^2)^{-1/(\beta-1)} \ge (1-1/\beta)d$, and so
\begin{eqnarray}
    E_{opt}(w,_0r) \le E_{opt}(r,\epsilon) \lesssim \sigma^2 + \epsilon^2 + (1-1/\beta)r^2d \asymp \sigma^2 + \epsilon^2 + r^2d \asymp E(w_0,r),
\end{eqnarray}
that is $E_{opt}(r,\epsilon) \asymp E(w_0,r) \asymp \sigma^2 + \epsilon^2 + r^2 d$.

\textbf{Case 3: $\epsilon^2 \ge \epsilon_2^2$.} Here, $a_6 = a_3 = r^2$, and
\begin{eqnarray}
    g_2(a_6) = g_2(r^2) = r^{-2/\beta} - \epsilon^2/r^2 \ge g_1(a_4).
\end{eqnarray}
Thus, $\max(g_1(a_4),g_2(a_6)) = g_2(a_6) = r^{-2/\beta}-\epsilon^2/r^2$, and so
\begin{eqnarray}
    E_{opt}(r,\epsilon) \asymp \sigma^2 + \epsilon^2 + r^2 \cdot (r^{-2/\beta}-\epsilon^2/r^2) = r^{2(1-1/\beta)}.
\end{eqnarray}
\end{proof}

\section{New: A Clean Analysis of the Euclidean Case}
Recall that $\Sigma = \sum_k \lambda_k \phi_k\phi_k^\top$ is the SVD of the feature covariance matrix $\Sigma$ and $c_k = \phi_k^\top w_0$ is the $k$th alignment coefficient of the generative model $w_0$, so that $w_0 = \sum_k c_k \phi_k$.
For Euclidean-norm attacks, the optimal solution for proxy adversarial energy is the ridge $w(t) = (\Sigma + tI_d)^{-1} \Sigma w_0$, for some regularization parameter $t \in [0,r^2]$. Observe that
\begin{eqnarray}
\|w(t)\|_2^2 = \|(\Sigma+ t I_d)^{-1}\Sigma w_0\|_2^2 = \sum_k \frac{\lambda_k^2 c_k^2}{(\lambda_k + t)^2}.
\end{eqnarray}
The standard and adversarial risks of $w(t)$ are then given by
\begin{eqnarray}
\begin{split}
E(w(t)) - \sigma^2 &= \|w-w_0\|_\Sigma^2 = t^2\|(\Sigma + t I_d)^{-1} w_0\|_\Sigma^2 = t^2 \sum_k \frac{\lambda_k c_k^2}{(\lambda_k + t)^2} =: F(t),\\
E(w(t),r) &\asymp E(w(t)) + r^2\|w(t)\|^2 \asymp \sigma^2 + G(r,t),\\
\text{ with }G(r,t) &= F(t) + r^2\sum_k \frac{\lambda_k^2 c_k^2}{(\lambda_k+t)^2}
\end{split}
\end{eqnarray}
Note that in particular,
\begin{eqnarray}
    E_{opt}(r) \asymp E(w(r^2),r) \asymp \sigma^2 + G(r,r^2).
\end{eqnarray}

\begin{mdframed}
\textbf{Key Insight:} The whole situation can understood via the $\lambda_k$'s, the $c_k$'s, and $r$! 
\end{mdframed}
Indeed, as we shall see, the auxiliary functions $F$ and $G$ can be analytically analyzed under some structural assumptions on the problems, namely on the $\lambda_k$'s, the $c_k$'s.

\subsection{Cost of Being Accurate: A Lower-Bound}
For $w(t)$ to be feasible, we need $F(t) \le \epsilon^2\|w_0\|_\Sigma^2$.
We deduce that
\begin{eqnarray}
    E_{opt}(r,\epsilon) \gtrsim \sigma^2 + \underline{G}_{opt}(r,\epsilon),\text{ with }\underline{G}_{opt}(r,\epsilon) := \inf_{t \in I(r,\epsilon)} G(r,t),
\end{eqnarray}
where $I(r,\epsilon) := \{0 \le t \le r^2 \mid F(t) \le \epsilon^2\|w_0\|_\Sigma^2\}$. We shall heavily exploit the above observation to obtain non-trivial lower-bounds.

\subsection{The Possibility of Free Lunch / No Tradeoff}
Note that $E_{opt}(r) \asymp E(w(r^2),r) \asymp \sigma^2 + G(r,r^2)$. If $w(r^2)$ is feasible, i.e if
\begin{eqnarray}
F(r^2) \le \epsilon^2 \|w_0\|_\Sigma^2,\text{ or equivalently, } \epsilon \ge \epsilon_\star(r):=\frac{\sqrt{F(r^2)}}{\|w_0\|_\Sigma},
\end{eqnarray}
then we must have $E_{opt}(r,\epsilon) \lesssim G(r,r^2)$, i.e $E_{opt}(r,\epsilon) \asymp G(r,r^2)$.
Let us state this more explicitly
\begin{restatable}{thm}{}
Let $r \ge 0$ be an imperceptible attack strength such that $\epsilon_\star(r) = o(1)$. Then for any fixed $\epsilon \in (0,1]$, it holds that
\begin{eqnarray}
    E_{opt}(r,\epsilon) \asymp E_{opt}(r).
\end{eqnarray}
That is, no tradeoff is needed!
\end{restatable}

\section{Some Worked Examples}
\subsection{A Case of Necessary Tradeoff: Isotropic Features}
Suppose $\lambda_k = 1$ for all $k \in [d]$. One easily computes
\begin{eqnarray}
\begin{split}
F(t) &= \dfrac{t^2\|w_0\|_2^2}{(1+t)^2},\\
G(r,t) &= \frac{(r^2+t^2)\|w_0\|_2^2}{(1+t)^2}.
\end{split}
\end{eqnarray}
Also, $I(r,\epsilon) = \{t \ge 0 \mid t \le \epsilon/(1-\epsilon)\} = [0,\epsilon/(1-\epsilon)]$. Thus, the lower-bound is given by
\begin{eqnarray}
\begin{split}
    E_{opt}(r,\epsilon) \gtrsim \sigma^2 + \underline{G}_{opt}(r,\epsilon) &\ge \sigma^2 + \|w_0\|_2^2 \inf_{0 \le t \le \epsilon/(1-\epsilon)} \frac{r^2 + t^2}{(1+t)^2}\\
    &= \sigma^2 + \|w_0\|_2^2 \left[\frac{r^2 + \epsilon^2/(1-\epsilon)^2}{(1+\epsilon/(1-\epsilon))^2}\right]\\
    &= \sigma^2 + \|w_0\|_2^2 (r^2(1-\epsilon)^2 + \epsilon^2)\\
    &\ge \sigma^2 + \|w_0\|_2^2(1-\epsilon)^2 r^2,
    \end{split}
\end{eqnarray}
valid for any $r \ge 0$ and $\epsilon$. This recovers a lower-bound we established earlier via a completely different argument. 

The interpretation of the above result is that: terms of standard accuracy, there is a necessary tradeoff for robustness. A similary finding was made in \cite{Javanmard2020PreciseTI}. 

Note that, here  one easily computes $\epsilon_\star(r) = \sqrt{F(r^2)} / \|w_0\|_\Sigma= r^2/(1+r^2) \in [0,1]$
BTW, note that $\epsilon_\star(r) \asymp \min(r^2,1)$.

\subsection{Free Lunch / A Case of No Tradeoff: Polynomial Spectral Decay}
We let $d=\infty$, i.e infinite input-dimension and consider the following structure for the eigenvalues $(\lambda_k)_k$ feature covariance and alignment coefficients $(c_k)_k$
\begin{eqnarray}
\lambda_k \asymp k^{-\beta},\, c_k^2 \asymp k^{-\delta}\text{ for all }k \in \mathbb Z_{++}\text{ and for some constants }\beta > 1,\,\delta \ge 0.
\end{eqnarray}
The condition $\beta > 1$ is to ensure that
\begin{align}
% \|w_0\|_2^2 &= \sum_{k=1}^\infty c_k^2 = \zeta(\delta) < \infty,\\
\|x\|^2 &\asymp \sum_{k=1}^\infty \lambda_k \asymp \sum_{k=1}^\infty k^{-\beta} = \zeta(\beta) < \infty\text{ w.h.p over }x \sim P_x = N(0,\Sigma),\\
\|w_0\|_\Sigma^2 &= \sum_{k=1}^\infty \lambda_k c_k^2 \asymp \sum_{k=1}^\infty k^{-\beta-\delta} = \zeta(\beta+\delta) < \infty.
\end{align}

Observe that $\delta \in [0,1)$, then the generative model $w_0$ itself has catastrophic non-robustness to any positive attack strength $r$, since
$$
E(w_0,r) \ge r^2\|w_0\|_2^2 = r^2 \sum_{k=1}^\infty c_k^2 \asymp r^2\sum_{k=1}^\infty k^{-\delta} = r^2\zeta(\delta) = \infty.
$$

We have the following crucial lemma.
\begin{restatable}{lm}{}
$F(t) \asymp t^{1-(1-\delta)/\beta}$ for $t = o(1)$.
\end{restatable}
With this lemma, we deduce that for an imperceptible attack strength $r=o(1)$, we must have
\begin{eqnarray} 
\epsilon_\star(r) := \frac{\sqrt{F(r^2)}}{\|w_0\|_\Sigma^2} \asymp r^{1-(1-\delta)/\beta}=o(r)=o(1).
\end{eqnarray}
Combining with Proposition abc, we obtain the following important result.
\begin{restatable}{thm}{}
In the case polynomial spectral regime, tradeoff between accuracy and robustness is not necessary. More precise, if for any fixed $\epsilon \in (0,1]$ and an imperceptible attack strength $r=o(1)$, it holds that
\begin{eqnarray}
    E_{opt}(r,\epsilon) \asymp E_{opt}(r).
\end{eqnarray}
\end{restatable}

\section{Weak-Strong Features}
\textcolor{red}{Obsolete (ignore!). Reason: No clear conclusion from this section.}
Here, $\lambda_k = 1_{k \le d_1} + b1_{k \ge d_1+1}$ for all $k \in [d]$, with $b \in [0,1]$ and $d_1 \in [d]$. It is clear that $\|w_0\|_\Sigma^2 = u^2 + b^2 v^2$, where
\begin{eqnarray}
    u^2 := \sum_{k \le d_1}c_k^2,\, v^2 := \sum_{k=d_1+1}^d c_k^2.
\end{eqnarray}
One computes
\begin{align}
F(t) &= \frac{u^2 t^2}{(1+t)^2} + \frac{b^2 v^2 t^2}{(b^2+t)^2} \asymp \min(t^2,1)u^2 + \min(t^2,b^2)v^2,\\
G(r,t) &= F(t) + \frac{r^2}{(1+t)^2} + \frac{r^2b^4}{(b^2+t)^2} \asymp F(t) + r^2(\min(1,1/t^2)u^2 + \min(1,b^4/t^2)v^2).
\end{align}

The critical threshold is given by
\begin{eqnarray}
\begin{split}
\epsilon_\star(r) = \frac{\sqrt{F(r^2)}}{\|w_0\|_\Sigma} &\asymp \sqrt{\frac{\min(r^4,1)u^2 + \min(r^4,b^2)v^2}{u^2+b^2 v^2}}\\
&=\begin{cases}
\sqrt{\frac{u^2 + b^2v^2}{u^2+b^2 v^2}} = 1,&\mbox{ if }r \ge 1,\\
\sqrt{\frac{r^4u^2 + b^2 v^2}{u^2+b^2 v^2}},&\mbox{ if }\sqrt{b} \le r \le 1,\\
\sqrt{\frac{r^4(u^2 + b^2 v^2)}{u^2+b^2 v^2}}=r^2,&\mbox{ if }b \le r \le \sqrt b,\\
??,&\mbox{ if }r \le b.
\end{cases} 
\end{split}
\end{eqnarray}
Note that if $v \lesssim u$, then $\epsilon_\star(r) \lesssim \min(r^2,1) \le r^2$.

Now, suppose $r = O(\sqrt b)$. Then, on the interval $[0,r^2] \supseteq I(r,\epsilon)$, we have
\begin{align}
F(t) \asymp t^2(u^2+v^2) = t^2\|w_0\|_\Sigma^2,\\
G(r,t) \asymp F(t) + r^2(u^2 + v^2) \asymp (r^2 + t^2)\|w_0\|_\Sigma^2 \asymp \|w_0\|_\Sigma^2.
\end{align}
We deduce that $E_{opt}(r) \lesssim E_{opt}(r,\epsilon) \lesssim \sigma^2 + G_{opt}(r,\epsilon) \lesssim \sigma^2 + r^2\|w_0\|_\Sigma^2 \lesssim \sigma^2 + G(r,r^2) \asymp E_{opt}(r)$,
that is
\begin{eqnarray}
    E_{opt}(r,\epsilon) \asymp E_{opt}(r).
\end{eqnarray}
For example, this is the case when $d_1=1$, and $c_k \equiv 1$, $b^2=1/d$, and $r = O(1/d^{1/4})$


% There are different cases to consider.

% \textbf{Case 1: $0 \le t \le b^2$.} Here $F(t) \asymp t^2(u^2 + v^2) = t^2\|w_0\|_2^2$ and
% \begin{eqnarray}
% G(r,t) \asymp F(t) + r^2(u^2+v^2) = (t^2+r^2)\|w_0\|_2^2  \ge r^2\|w_0\|_2^2.
% \end{eqnarray}

% \textbf{Case 2: $b^2 \le t \le b$.} Here, $F(t) \asymp t^2(u^2 + v^2) = t^2\|w_0\|_2^2$ and $G(r,t) \asymp F(t) + r^2(u^2 + b^4v^2/t^2)$, and so
% \begin{eqnarray}
%    \inf_{t \in \cap [0,b^2] \cap I(r,\epsilon)}G(r,t) \gtrsim F(b) + r^2(u^2+b^2v^2) \ge r^2(u^2 + b^2 v^2),
% \end{eqnarray}

% \textbf{Case 3: $b \le t \le 1$.} Here, $F(t) \asymp t^2 u^2 + b^2 v^2$ and $G(r,t) \asymp F(t) + r^2(u^2 + b^4v^2/t^2)$, and so
% \begin{eqnarray}
%    \inf_{t \in \cap [b,1] \cap I(r,\epsilon)}G(r,t) \gtrsim F(1) + r^2(u^2+b^4v^2) \ge r^2(u^2 + b^4 v^2),
% \end{eqnarray}

% \textbf{Case 4:} $t \ge 1$. This only occurs if $1 \le \epsilon/(1-\epsilon)$, i.e if $\epsilon \ge 1/2$. Here, $F(t) \asymp u^2/t + b^2 v^2/t$ and $G(r,t) \asymp F(t) + r^2(u^2 + b^4v^2) / t^2$, and so
% \begin{eqnarray}
%    \inf_{t \in \cap [1,\infty) \cap I(r,\epsilon)}G(r,t) \gtrsim F(\epsilon/(1-\epsilon)^2) + r^2(u^2+b^4v^2) \ge r^2(u^2 + b^4 v^2)(1-\epsilon)^2/\epsilon^2,
% \end{eqnarray}

% Taking the min of all three cases, we get
% \begin{eqnarray}
%      \underline{G}_{opt}(r,\epsilon) \gtrsim r^2(u^2+b^4 v^2)\min(1,(1-\epsilon)^2/\epsilon^2).
% \end{eqnarray}
% We have thus proved the following.
% \begin{restatable}{thm}{}
% For any $r \ge 0$ and $\epsilon \in [0,1)$,
% \begin{eqnarray}
%     E_{opt}(r,\epsilon) \gtrsim \sigma^2 + r^2(u^2+b^4 v^2)\min(1,(1-\epsilon)^2/\epsilon^2).
% \end{eqnarray}
% Moreover, if $\epsilon \ge \epsilon_\star(r)$ given as in \eqref{eq:abc}, then
% \begin{eqnarray}
%     E_{opt}(r,\epsilon) \asymp E_{op}(r).
% \end{eqnarray}
% \end{restatable}

% \subsection{Case of Many Strong Features}
% Now consider the following weak-strong feature settings
% \begin{align}
%     d_1 &= d/2,\, b^2 = 1/d,\,c_k^2 = 1\forall k \in [d]\label{eq:manystrong1},\\
%     d_1 &= d/2,\, b^2 = O(1),\,c_k^2 = 1\forall k \in [d]\label{eq:manystrong2}.
% \end{align}
% In the first case \eqref{eq:manystrong1}, it is easy to compute
% \begin{eqnarray}
% \begin{split}
% u =\sqrt{d_1} \asymp \sqrt d,\, v&=\sqrt{d_2} \asymp \sqrt d,\,\sqrt{u^2+b^2 v^2}  \asymp\sqrt d.
% \end{split}
% \end{eqnarray}
% Taking $r = 1$, which is imperceptible since $1 \ll \|x\|$ w.h.p over $x \sim P_x = N(0,\Sigma)$, we have $\epsilon_\star(1) = \Theta(1)$, The previous theorem gives
% \begin{restatable}{cor}{}
% For all $r \ge 1$ and $\epsilon \in (0,1)$.
% \begin{eqnarray}
% \begin{split}
% E_{opt}(r) &\asymp \sigma^2 + G(r,r^2) \asymp \sigma^2 + d,\\
%     E_{opt}(r,\epsilon) &\gtrsim \sigma^2 +  \min(1,(1-\epsilon)^2/\epsilon^2)r^2 d.
%     \end{split}
% \end{eqnarray}
% \end{restatable}

% \subsection{The Case of Only a Few Strong Features: Free Lunch}
% We now show an instance of the problem where there is indeed phase-transition. Consider a weak-strong feature setting with
% \begin{eqnarray}
% d_1=1,\, b^2 = 1/d,\,c_k^2=1\forall k \in [d],
% \label{eq:fewstrong}
% \end{eqnarray}
% We will show that there is a catastrophic tradeoff between accuracy and robustness. Here, $u^2=1$, $v^2 \asymp d$, $b^2v^2 \asymp 1$, $b^4 v^2 = o(1/d)$.

% One easily computes $\epsilon_\star(r) \asymp \max(r, 1/r)$.




==> statistics.tex <==
\section{Classical Consistency and Robustness Are Not Compatible}
\label{sec:consequences}
In this section, we explore a selection of the statistical consequences of our results.

\subsection{Failure of Consistent Estimators to be Robust}
\begin{restatable}{df}{}
We say an estimator $\mathcal D_n \mapsto \widehat w_n \in \mathbb R^d$ of the generative model $w_0$ is standard risk-consistent if its excess standard risk vanishes in the infinite-sample limit, i.e $\Delta(\widehat w_n) = o_{n,\mathbb P}(1)$.
\end{restatable}
For such estimators, we have the following result which is a direct consequence of Corollary \ref{cor:concrete}, but is stated as a theorem due to its importance.
\begin{restatable}{thm}{}
If $\widehat w_n$ is a standard risk-consistent estimator of the generative model $w_0$, then it holds for any $r \ge 0$ that
% \begin{eqnarray}
$
E(\widehat w_n,r) \gtrsim (1-o_{n,\mathbb P}(1))\|w_0\|_\Sigma^2 r^2/r_1^2.
$
% \end{eqnarray}
\label{thm:nonrobustconsistent}
\end{restatable} 
%%\vspace{-5mm}
As a consequence, for an imperceptible attack strength $r \ll r(\Sigma)$,
Theorem \ref{thm:nonrobustconsistent} predicts a catastrophic failure of standard risk-consistent estimators, as regards robustness: the adversarial risk of such estimators explodes as the strength $r$ is increased.
% to infinity for imperceptible adversarial perturbations in high dimensions.
We shall exhibit a few special cases of this phenomenon.

\subsection{Failure of Lasso-type Estimators}
Consider the case of isotropic features where $\Sigma = I_d$, and suppose the generative model $w_0$ is exactly $s$-sparse in high-dimensions, where $s \in [d]$ and $s \gg 1$, and $w_0 = (1_s,0_{d-s})$ for simplicity. For $\ell_\infty$-norm attacks, we have the following corollary of Theorem \ref{thm:nonrobustconsistent} and Corollary \ref{cor:linfattack}.
% \begin{eqnarray}
%     \begin{split}
% r_0 &= \|w_0\|_2/\|w_0\|_1 = 1/\sqrt{s},\\
% r_1 &= \|w_0\|_\infty / \|w_0\|_2 = 1/\sqrt{s}.
%     \end{split}
% \end{eqnarray}
We deduce the following corollary from Theorem \ref{thm:nonrobustconsistent}.
\begin{restatable}{cor}{}
\label{cor:Lasso}
Let $\widehat w_n$ be  a standard risk-consistent estimator  of the $s$-sparse generative model $w_0$.
Then, for an $\ell_\infty$-norm attack of strength $r \asymp \sqrt{\log(d)/s}$, the adversarial risk of $\widehat w_n$ verifies
\begin{eqnarray}
E(\widehat w_n, r) \gtrsim (1-o_{n,\mathbb P}(1))\frac{\log d}{1+\widetilde\sigma^2} \cdot E_{opt}(r),
\label{eq:curse}
\end{eqnarray}
which is $\Omega(\log d)$ times larger than the global optimum $E_{opt}(r)$.
\end{restatable}
% We deduce from \eqref{eq:thighnflt} that, for any fixed $\epsilon \in [0,1)$, one has the following nontrivial lower-bound for $r \ge r_1c(\epsilon)$
% \begin{equation*}
% \begin{split}
%      \frac{E_{opt}(r,\epsilon)}{\|w_0\|_2^2}  & \asymp \max(\widetilde \sigma^2 + \epsilon^2, (1-\epsilon)^2 sr^2).
%     \end{split}
% \end{equation*}
% Taking $r = r_1\sqrt{\log d} \asymp \sqrt{\log d /s}$ then yields
% \begin{align}
% \frac{E_{opt}(r,\epsilon)}{\|w_0\|_2^2}  &\asymp  \max(\widetilde \sigma^2 + \epsilon^2, (1-\epsilon)^2 \log d)\label{eq:lboundL2}.
% %\\ &\gtrsim (1-\epsilon)^2\log d,
% % \label{eq:logboundL2}
% \end{align}
% Thus, if a model is accurate meaning that $1-\epsilon$ is close to $1$, it suffices a (normalized) adversarial risk of order at last $\log d$, which grows to infinity with input-dimension $d$. In particular, taking $\epsilon=0$, we deduce that for an attack strength $r \asymp \sqrt{\log(d)/s}$, the generative model $w_0$ suffers a adversarial risk
% \begin{eqnarray}
%     E(w_0,r)/\|w_0\|_2^2 \asymp \max(\widetilde\sigma^2,\log d),
% \end{eqnarray}
% that is $\log d$ times larger than that of the null model $E(0,r) \asymp \max(\|w_0\|_2^2,\sigma^2)$. 
The above result predicts non-robustness to imperceptible adversarial perturbations with $r \ll r(\Sigma)$.
An analogous result has been established in \cite{tsipras18} in the context of binary classification.

% We have the following statistical version of preceding observation, which shows that Lasso-type estimators which adapt to the sparisty of the generative model $w_0$, are doomed in the setting of adversarial robustness.

% \paragraph{Application to the Lasso.}
As a concrete example, the classical theory of sparse linear regression \cite{BickelSimultaneous2009,BellecSlopeMeets2018} tells us that amongst all linear models constructed using the finite training dataset $\mathcal D_n$, the Lasso estimator $\widehat w_n^{Lasso}$ with penalty parameter $\lambda \asymp \sigma \sqrt{s\log(ed/s)/n}$ attains minimax excess standard risk of
\begin{eqnarray}
\Delta(\widehat w_n^{Lasso}) \asymp \sigma^2 s\log(ed/s)/n.
\end{eqnarray}
w.h.p over the training dataset $\mathcal D_n$. Thus, if the sample size is scaled appropriately so that $s\log(ed/s)/n \to 0
$, then the Lasso estimator suffers the curse \eqref{eq:curse}. This phenomenon is empirically confirmed in Figure \ref{fig:Lasso}.

\begin{figure*}[!t]
    \centering
    %\includegraphics[width=1\textwidth]{Lasso.pdf}
    \includegraphics[width=.9\textwidth]{Lasso.pdf}
    %\vspace{-.5cm}
    \caption{\textbf{Failure of Lasso-type Estimators} (Empirical verification of Corollary \ref{cor:Lasso}). We consider a small experiment with $n=1500$, while the input-dimension $d$ varies in the set $\{10,20,\ldots,100\}\cup \{100, 150, 200, 250,\ldots, 750\}$. For each value of $d$, we set the sparsity level $s$ to the integer part of $\sqrt{d}$ and the attack strength to $r=\sqrt{\log(d)/s}$. See Appendix \ref{sec:expe} for detailed experimental setup. In the legend, $\widehat\epsilon_n := \Delta(\widehat w_n^{Lasso})$ is the excess standard risk of the Lasso estimator $\widehat w_n^{Lasso}$. Notice how our prediction \eqref{eq:curse} agrees with experiment.}
    \label{fig:Lasso}
\end{figure*}

% \subsection{Failure of Benignly-Overfitted Estimators}
% \lorem

% \lorem

\section{The Role of Over-Parametrization in Robustness}
Consider the so-called proportionate scaling high-dimensional regime where the sample size $n$ and the input-dimension $d$ grow to infinity at the same rate, i.e
\begin{eqnarray}
\label{eq:proportionate}
n,d \to \infty\text{ with }d/n \to \gamma \in (0,\infty).
\end{eqnarray}
The scalar $\gamma$ is the level of \emph{parametrization}: \emph{under-parametrization} corresponds to $\gamma < 1$, while \emph{over-parametrization} corresponds to $\gamma \ge 1$.

\subsection{Ordinary Least Squares}
It has been argues in \cite{min2021curious,bubeck2021universal} that over-parametrization is condusive to robustness. Let us recover this prediction from our theory.

 Let $\widehat w_n^{OLS} \in \mathbb R^d$ be the ordinary least-squares (OLS) estimator computed on the finite training iid dataset $\mathcal D_n=\{(x_1,y_1),\ldots,(x_n,y_n)\}$ from the data distribution \eqref{eq:generator}, that is
 \begin{eqnarray}
 \widehat w_n^{OLS}:=X^\dagger Y \in
 % \underset{w \in I_n}{\arg\min}\, \|w\|_2,
 \underset{w \in \mathbb R^d}{\arg\min}\, \widehat E_n(w),
 \label{eq:ols}
 \end{eqnarray}
% where $I_n := \{w \in \mathbb R^d %\mid f_w(x_i) = y_i\,\forall %i=1,\ldots,n\}$is the set of linear %interpolators of the data. Note that %$\widehat w_n^{OLS}$ is random, as it %depends on the random dataset %$\mathcal D_n$.
where $X := (x_1,\ldots,x_n) \in \mathbb R^{n \times d}$ is the design matrix with Moore-Penrose pseudo-inverse $X^\dagger \in \mathbb R^{d \times n}$; $Y=(y_1,\ldots,y_n) \in \mathbb R^n$ is the response vector; $\widehat E_n(w) := (1/n)\sum_{i=1}^n (f_w(x_i)-y_i)^2 = \|Xw-Y\|_2^2/n$ is the empirical version of the standard risk.


\begin{figure*}[!t]
    \centering
\includegraphics[width=.85\textwidth]{overparam.pdf}
    %%\vspace{-.5cm}
    \caption{
    % Empirical demonstration of
    \textbf{The role of over-parametrization for OLS} in robustness in isotropic setting. The blue curve corresponds to the adversarial error $E(\widehat w_n^{OLS}, r)$ for different values of the attack strength $r$, plotted against the parametrization rate $d/n$. The green curve is the lower-bound (and upper-bound) given in \eqref{eq:well-conditioned}. The vertical line at $\gamma=10^0=1$ corresponds to the so-called \emph{interpolation threshold}. The horizontal black line corresponds to the risk of the null predictor.
    Error bars represent 5 independent runs. See Appendix \ref{sec:expe} for experimental details. Notice how over-parametrization (large $\gamma$) appears to be bad for standard generalization (black curve), but good for adversarial generalization. Notice that predictions of Colloraries \ref{cor:underparam} and \ref{cor:overparam} are verified.}
    \label{fig:overparam}
\end{figure*}
 \begin{figure*}[!t]
    \centering
\includegraphics[width=1\textwidth]{compare.pdf}
    %\vspace{-.5cm}
    \caption{\textbf{Failure of OLS in robustness.}
    % Empirical verification of our bounds, for different attacks run on different models.
    Here the sample size and input-dimension are $n=100$ and $d=10$. respectively. See Appendix \ref{sec:expe} for experimental details.  OLS stands for the OLS estimator $\widehat w_n^{OLS}$, while OPT stands for the linear model $w_{opt}(r)$ which attains the globally optimal adversarial risk $E_{opt}(r)$. In each case, the lower-bound given in Theorem \ref{thm:NFLT}. We see that our lower-bound is verified in all cases. In the case of $\ell_\infty$-norm attack on OLS, notice how the adversarial risk is considerably larger than the lower-bound, indicative of the fact that OLS strikes a very bad tradeoff between standard and adversarial risk in this setting.} 
    \label{fig:all}
\end{figure*}


In \cite{Hastie2019} (see Theorem 1 therein), it was established that in the limit \eqref{eq:proportionate} the standard excess risk of the OLS estimator $\widehat w_n^{OLS}$ is given by
\begin{eqnarray}
\label{eq:hastie}
\Delta(\widehat w_n^{OLS}) \overset{a.s}{\to}
\begin{cases}
1-1/\gamma + \widetilde\sigma^2/(\gamma-1),&\mbox{ if }\gamma \ge 1,\\
\widetilde\sigma^2 \gamma/(1-\gamma),&\mbox{ else.}
\end{cases}
\end{eqnarray}


\paragraph{Extreme Under-Parametrization.} In the limit $\gamma \to 0^+$, \cite{Hastie2019} predicts that
\begin{eqnarray}
\label{eq:DeltaUnderparam}
\lim_{\gamma \to 0^+}\lim_{\substack{n,d \to \infty\\d/n \to \gamma}}\Delta(\widehat w_n^{OLS}) = 0,
\end{eqnarray}
This regime can be thought of as the fixed-dimensional regime, where $n \to \infty$ with the input-dimension $d$ held "fixed". 
Combining Theorem \ref{thm:lousy} with \eqref{eq:DeltaUnderparam} then gives the following corollary which predicts the failure of OLS and GD to find a robust model even when one exists.
\begin{restatable}{cor}{}
For a Euclidean-norm attack of strength $r \ge 0$,it holds that
\begin{eqnarray*}
\begin{split}
\lim_{\gamma \to 0^+}\lim_{\substack{n,d \to \infty\\d/n \to \gamma}}E(\widehat w_n^{OLS},r) &\asymp \sigma^2 + \|w_0\|_2^2H(r,0)^2 = \sigma^2 + \|w_0\|_2^2r^2.
\end{split}
\end{eqnarray*}
\label{cor:underparam}
\end{restatable}
Incidentally, up to within multiplicative absolute constants, the RHS in the above corresponds to the (normalized) adversarial risk of the generative model\footnote{To see this, apply Lemmas \ref{lm:analytic} and \ref{lm:proxy} at $w=w_0$.} $w_0$, which is far from being optimal (in particular, it is unbounded in $r$). This means that OLS and GD\footnote{Since the GD dynamics \eqref{eq:gd} converges to OLS estimator as noted earlier.} may fail to find robust models even when they exist.

 \paragraph{Extreme Over-Parametrization.} In the limit $\gamma \to +\infty$, \cite{Hastie2019} predicts that
$$
\lim_{\gamma \to +\infty}\lim_{\substack{n,d \to \infty\\d/n \to \gamma}}\Delta(\widehat w_n^{OLS})  = 1.
$$
Thus, in this regime the excess standard risk $\Delta(\widehat w_n^{OLS})$ tends to $1$ (the null predictor), and the estimate \eqref{eq:thighnflt} given in our Theorem \ref{thm:lousy} predicts that
\begin{restatable}{cor}{}
For a Euclidean-norm attack of strength $r \ge 0$, it holds that
\begin{eqnarray*}
\begin{split}
\lim_{\gamma \to \infty}\lim_{\substack{n,d \to \infty\\d/n \to \gamma}} E(\widehat w_n^{OLS},r) &\asymp \sigma^2 + \|w_0\|_2^2H(r,1)^2 = \sigma^2 + \|w_0\|_2^2.
\end{split}
\end{eqnarray*}
\label{cor:overparam}
\end{restatable}
The RHS matches (up to within absolute constants), the normalized adversarial risk of the null model\footnote{To see this, apply Lemmas \ref{lm:analytic} and \ref{lm:proxy} at $w=0$.}, i.e $E(0,r) \asymp \sigma^2 + \|w_0\|_2^2$, which is itself sub-optimal for small values of $r$.

The situation is empirically confirmed in Figures ~\ref{fig:all} and \ref{fig:overparam}.

\subsection{Optimality of Adversarial Training in the Extremely Under-Parametrized Regime}
To illustrate the analytic power of our results, let us present a simple self-contained derivation of a crucial result established in \cite{javanmard2022precise}, namely that in the infinite-data regime corresponding to \eqref{eq:proportionate} with $\gamma \to 0^+$,
adversarial training attains all points of the Pareto frontier $\mathcal C_r$, for any $r \ge 0$.
More precisely, consider adversarial training which minimizes over $w \in \mathbb R^d$, the empirical adversarial risk \begin{eqnarray}
\widehat E(w,s) = \frac{1}{n}\sum_{i=1}^n \sup_{\|\delta\| \le s}(f_w(x_i+\delta)-y_i)^2.
\end{eqnarray}
Here $s \ge 0$ is the attack strength used during training. It is easy to see that
\begin{eqnarray}
    \widehat E(w,s) \asymp \frac{1}{n}\sum_{i=1}^n (x_i^\top w - y_i)^2 + r^2\|w\|_2^2.
\end{eqnarray}
Let $\widehat w(s)$ be the minimizer of the RHS over $w \in \mathbb R^d$.
\begin{assume}
\label{assume:javanmard}
Assume that $\dfrac{\|w_0\|_2^2}{d} \to R^2 \in (0,\infty)$ and $\dfrac{\sigma_0^2}{d} \to \sigma^2 \in (0,\infty)$ in the limit \eqref{eq:proportionate}.
\end{assume}
We have the following result.
\begin{prop}
\label{prop:softjavanmard}
Take Assumption \ref{assume:javanmard} for granted. For any $r \ge 0$ and $\epsilon \in [0,1)$, it holds with $s = \epsilon/(1-\epsilon)$ that
\begin{eqnarray}
\begin{split}
    \lim_{\gamma \to 0^+}\lim_{\substack{n,d \to \infty\\d/n \to \gamma}}\Delta(\widehat w_n(s)) &= \epsilon^2,\\
        \lim_{\gamma \to 0^+}\lim_{\substack{n,d \to \infty\\d/n \to \gamma}}E(\widehat w_n(s),r) &\asymp E_{opt}(r,\epsilon).
        \end{split}
\end{eqnarray}
\end{prop}

\subsection{Failure of Adversarial Training in Low-SNR Regime}
We now consider the case where $\mathrm{SNR} := R^2/\sigma^2 \ll 1$ and show that for any fixed $\gamma \in (0,\infty)$, adversarially training fails to be robust.

Indeed, let  $m_\gamma$ be the complementary Stieltjes transform of the Marchenko-Pastur distribution $\mu_\gamma \in \mathcal P(\mathbb R)$ with shape parameter $\gamma$, defined by
\begin{eqnarray}
m_\gamma(z) := \int_0^\infty \frac{\mathrm{d}\mu_\gamma(z)}{\lambda-z},\text{ for }z \in \mathbb C\setminus \mathbb R,\\
m_\gamma(z) := \lim_{\eta \to 0} m_\gamma(z + i\eta),\mbox{ if }z \in \mathbb R.
\end{eqnarray}
We have the following result.
\begin{restatable}{thm}{}
Suppose $SNR := R^2/\sigma^2 = o(1)$ in the proportionate scaling limit \eqref{eq:proportionate}. Then, for any $r,t \ge 0$, it holds in the proportionate scaling limit \eqref{eq:proportionate} that
\begin{eqnarray}
\begin{split}
\lim_{\substack{n,d \to \infty\\d/n \to \gamma}}E(\widehat w^{AT}_n(t)) &= \overline e(t) := \gamma (m_\gamma(-t) + t m_\gamma'(-t)),\\
\lim_{\substack{n,d \to \infty\\d/n \to \gamma}} E(\widehat w^{AT}_n(t),r) &\asymp r^2 \overline e(t).
\end{split}
\end{eqnarray}
\end{restatable}


% \subsection{Euclidean Attacks on Well-Conditioned features}
% Consider Euclidean-norm attacks on isotropic features, i.e $\Sigma=I_d$. This is the setup studied in \cite{Javanmard2020PreciseTI}). In this case, note that $r_1=r_2=1$. Then, 
% we deduce from \eqref{eq:informalthight} that, for fixed $\epsilon \in [0,1)$, one has the following nontrivial lower-bound for $r \ge c(\epsilon)$ with $c(\epsilon) = \epsilon/\sqrt{\widetilde\sigma^2 + \epsilon^2} \in [0, 1]$,
% \begin{equation*}
%     \frac{E_{opt}(r,\epsilon)}{\|w_0\|_2^2}   \asymp H(r,\widetilde\sigma,\epsilon)^2   
%     \asymp  \max(\widetilde\sigma^2 + \epsilon^2, (1-\epsilon)^2r^2).
% \end{equation*}


% \input{benignO.tex}
% \lorem

% that is $r \ll \|x\|_\infty$ w.h.p, for a random test point $x$.

% \begin{figure*}
%     \centering
% \includegraphics[width=.7\textwidth]{highdim.pdf}
%     \caption{High-dimensional effects. \textbf{Right:} Results for $\ell_2$-norm attack, with attack strength $r=r_1\sqrt{\log d}$, where $d$ is the input-dimension. Blue curve is empirically computed adversarial risk of OLS estimator $\widehat w_n^{OLS}$. Broken black curve is our lower-bound in \eqref{eq:mainresult}. Broken magenta curve $(1-\epsilon)^2 \log d$, where $\widehat \epsilon$ is the excess standard risk of $\widehat w_n^{OLS}$. \textbf{Left:} Results for $\ell_\infty$-norm attack, with attack strength $r=r_1\sqrt{\log(d / s)}$, where $s \approx \sqrt{d} \ll d$ is the sparsity of the generative model $w_0$.}
%     \label{fig:highdim}
% \end{figure*}
% \lorem 


% \section{Statistical Consequences}
% \subsection{Minimax Theory}
% \textcolor{red}{TODO:}
% \begin{itemize}
% \item Consider Bayesian linear regression where $w_0 \sim N(0,I_d)$.
% \item Compute posterior distribution of $w_0$ given the training data $\mathcal D_n$.
% \item Use concentration / RMT arguments to obtain lower and upper-bounds for $H(r/r_0,\epsilon)$, as function of $n$, $d$, $\Sigma$, $r$, and $\epsilon$.
% \item Harvest the spoils!
% \end{itemize}

\subsection{Proof of Proposition \ref{prop:softjavanmard}}
    Indeed, observe $\widehat E(w,s) = \dfrac{1}{n}\sum_{i=1}^n(|x_i^\top w - y_i| + s\|w\|_\star)^2 \asymp \dfrac{1}{n}\|Xw-y\|_2^2 + s^2\|w\|_\star^2$, where the first is thanks to Lemma \ref{lm:wellknown} and the second is thanks to Lemma \ref{lm:sandwich}. In the special case of Euclidean-norm attacks, minimizing the RHS over $w \in \mathbb R^d$ gives
\begin{eqnarray}
\begin{split}
    w=\widehat w(s^2) &:= (X^\top X/n +  s^2 I_d)^{-1}X^\top y/n\\
    &= (\widehat \Sigma_n + s^2 I_d)^{-1}\widehat\Sigma_n w_0 + (\widehat \Sigma_n + s^2 I_d)^{-1}X^\top Z/n,
\end{split}
\end{eqnarray}
where $Z=(z_1,\ldots,z_n) \in \mathbb R^d$ is the label-noise vector for the dataset.
Thus, $\widehat w(s^2)$ is a ridge estimator with regularization parameter $t=s^2$. Here, $\widehat \Sigma_n := X^\top X/n$ is the empirical covariance matrix, with eigenvalues $\widehat \lambda_1 \ge \widehat \lambda_2 \ge \ldots $. In the limit $d \to \infty$, one then deduces that the standard risk of the adversarially trained model is given by
\begin{eqnarray}
\begin{split}
E(\widehat w(t)) - \sigma_0^2 &= \|\widehat w(r)-w_0\|_\Sigma^2 = t^2\frac{\|w_0\|_2^2}{d}\sum_j\frac{1}{(\widehat \lambda_j + t)^2} + \frac{\sigma_0^2}{n}\sum_j \frac{\widehat \lambda_j}{(\widehat \lambda_j+t)^2} + o_{\mathbb P}(1)\\
&= t^2R^2\sum_j\frac{1}{(\widehat \lambda_j + t)^2} + \gamma\sigma^2\sum_j \frac{\widehat \lambda_j}{(\widehat \lambda_j+t)^2} + o_{\mathbb P}(1).
\end{split}
\end{eqnarray}
Also, one deduces that the adversarial risk of the adversarially trained model is given by
\begin{eqnarray}
\begin{split}
E(\widehat w(t),r) &\asymp E(\widehat w(t)) + r^2\|\widehat w(t)\|_2^2\\
&= E(\widehat w(t)) + \frac{r^2\|w_0\|_2^2}{d}\sum_j \frac{\widehat \lambda_j^2}{(\widehat \lambda_j+t)^2} + \frac{r^2\sigma_0^2}{n}\sum_j \frac{\widehat \lambda_j}{(\widehat \lambda_j+t)^2} + o_{\mathbb P}(1)\\
&= E(\widehat w(t)) + r^2R^2\sum_j \frac{\widehat \lambda_j^2}{(\widehat \lambda_j+t)^2} + \gamma r^2\sigma^2\sum_j \frac{\widehat \lambda_j}{(\widehat \lambda_j+t)^2} + o_{\mathbb P}(1)
\end{split}
\end{eqnarray}
In the proportionate scaling regime \eqref{eq:proportionate} with $\gamma \to 0^+$, we further obtain
\begin{align}
    \frac{E(\widehat w(t))}{d} &\overset{p}{\to} \overline E(\widehat w(t)) := \frac{t^2 R^2}{(1+t)^2} + \sigma^2,\\
        \frac{E(\widehat w(t),r)}{d} \asymp \frac{E(\widehat w(t)) + r^2\|\widehat w(t)\|_2^2}{d} &\overset{p}{\to}  \overline E(\widehat w(t)) + \frac{r^2R^2}{(1+t)^2}.
\end{align}
Setting $\overline E(\widehat w(t)) = \epsilon^2 R^2 + \sigma^2$ gives $\epsilon^2 = t^2/(1+t)^2 \in [0,1]$, i.e $\epsilon = t/(1+t)$, or equivalently $1/(1+t) = 1-\epsilon$, and so
\begin{align*}
\Delta(\widehat w(t)) &:= \frac{E(\widehat w(t)) - \sigma_0^2}{\|w_0\|_2^2} \to  \frac{t^2}{(1+t)^2} = \epsilon^2,\\
\frac{E(\widehat w(t),r)}{d} &\asymp \epsilon^2R^2 + \sigma^2 +  (1-\epsilon)^2 R^2 r^2 \asymp \frac{E_{opt}(r,\epsilon)}{d},
\end{align*}
where the last step in the second line is thanks to Corollary \ref{cor:isotropic}.


==> weakstrong.tex <==
\subsection{Weak-Strong Features}
For large input-dimension $d$, let $b \asymp 1/d$, and set the spectral quantities $(\lambda_k)_k$ and $(c_k)_k$ as follows
\begin{eqnarray}
\lambda_k = 1_{k=1} + b1_{k \ge 2}\text{ and }c_k= 1,\text{ for all }k \in [d].
\end{eqnarray}
It is clear that for Euclidean-norm attacks, the imperceptibility threshold is $r(\Sigma) \asymp \sqrt{\mbox{tr}(\Sigma)} = \Theta(1)$. Also note that $\|w_0\|_\Sigma^2 = 1 + 1 = 2 = \Theta(1)$.
One computes
\begin{align}
G(\lambda) &= \frac{\lambda^2}{(1+\lambda)^2} + \frac{\lambda^2}{(b+\lambda)^2} \asymp \frac{\lambda^2}{(b+\lambda)^2},\\
F(r,\lambda) &= G(\lambda) + r^2\left(\frac{1}{(1+\lambda)^2} + \frac{b}{(b+\lambda)^2}\right).
\end{align}
For $1 \gtrsim r \gtrsim \sqrt b \asymp 1/\sqrt d$, the "free lunch" threshold is given by 
\begin{eqnarray}
\begin{split}
\epsilon_\star(r) = \frac{\sqrt{G(r^2)}}{\|w_0\|_\Sigma} \asymp \sqrt{G(r^2)} \asymp \frac{r^2}{b+r^2} \asymp \min(r^2/b,1) = \Theta(1).
\end{split}
\end{eqnarray}
For such values of $r$, 
the absolute optimal adversarial risk $E_{opt}(r)$ is given by
\begin{eqnarray}
\begin{split}
    E_{opt}(r) &\asymp \sigma^2 + F(r,r^2) \asymp \sigma^2 + G(r^2) 
+ r^2\left(\frac{1}{(1+r^2)^2} + \frac{b}{(b+r^2)^2}\right)\\
    &\asymp \sigma^2 + 1 + \min(r^2/b,b/r^2) \asymp \sigma^2 + 1,
    \end{split}
\end{eqnarray}
For $0 \le \epsilon \le \epsilon_\star(r)$, solving the equation $G(\lambda) = \epsilon^2\|w_0\|_\Sigma^2$ for $\lambda \in [0,r^2]$ gives
\begin{eqnarray}
    \lambda_{opt}(r,\epsilon) \asymp \frac{b\epsilon}{1-\epsilon}.
\end{eqnarray}

Thus, for $0 \le \epsilon \le \epsilon_\star(\epsilon)$, one has
\begin{eqnarray*}
\begin{split}
    E_{opt}(r,\epsilon) &\asymp \sigma^2 + F(r,\lambda_{opt}(r,\epsilon)) \asymp \sigma^2 + \epsilon^2 + r^2\left(\frac{1}{(1+b\epsilon/(1-\epsilon))^2} + \frac{b}{(b+b\epsilon/(1-\epsilon))^2}\right)
    \\
    &\asymp \sigma^2 + (1-\epsilon)^2 r^2 + (1-\epsilon)^2 r^2/b \asymp \sigma^2 + \epsilon^2 + (1-\epsilon)^2r^2/b.
    \end{split}
\end{eqnarray*}
Comparing with $E_{opt}(r,\epsilon)$, we deduce that
\begin{restatable}{cor}{}
Consider Euclidean-norm attack of strength $1/\sqrt d \lesssim r \lesssim 1$. Fix a tolerance level $\epsilon \in [0,1]$. The following hold:
\begin{itemize}
\item[(i)] \textbf{(Free Lunch Threshold).} $\epsilon_\star(r) \asymp \min(r^2d,1) = \Theta(1)$.
\item[(ii)] \textbf{(Free Lunch).} If $\epsilon \ge \epsilon_\star(r)$, then $E_{opt}(r,\epsilon) \asymp E_{opt}(r) \asymp \sigma^2 + 1$.
\item[(iii)] \textbf{(Accuracy / Robustness Tradeoff).} 
If $0 \le \epsilon \le \epsilon_\star(r)$, then
\begin{eqnarray}
    \frac{E_{opt}(r,\epsilon)}{E_{opt}(r)} \asymp \epsilon^2 + (1-\epsilon)^2 r^2/b \asymp (1-\epsilon)^2 r^2 d.
\end{eqnarray}
That is, the adversarial risk $E_{opt}(r,\epsilon)$ of accurate models is up to $d$ times larger than the absolute optimum value $E_{opt}(r)$ over all linear models.
\end{itemize}
\end{restatable}



